A Simulation Framework for Contention-Free Scheduling on WiGig

The latest IEEE 802.11 amendments provide support to directional communications in the Millimeter Wave spectrum and, thanks to the wide bandwidth available at such frequencies, makes it possible to wirelessly approach several emergent use cases, such as virtual and augmented reality, telepresence, and remote control of industrial facilities. However, these applications require stringent Quality of Service, that only contention-free scheduling algorithms can guarantee. In this paper, we propose an end-to-end framework for the joint admission control and scheduling of periodic traffic streams over mmWave Wireless Local Area Networks based on Network Simulator 3, a popular full-stack open-source network simulator. Moreover, we design a baseline algorithm to handle scheduling requests, and we evaluate its performance with a full-stack perspective. The algorithm is tested in three scenarios, where we investigated different configurations and features to highlight the differences and trade-offs between contention-based and contention-free access strategies.

==> img/100Mbps/numStas_10_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.89, xmax=9.89,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9,STA 10},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=180.1195776185,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,147.966055519961);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,142.421576059754);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,135.372828487911);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,141.10536885398);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,151.895846730463);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,142.730843630975);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,156.258713774316);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,133.135584696838);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,118.591841491897);
\draw[draw=none,fill=color0] (axis cs:8.6,0) rectangle (axis cs:9,142.465476046882);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,52.4664155152823);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,42.8363360342506);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,56.3801401044929);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,51.0283446713191);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,52.5879567569889);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,50.9965270888777);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,49.8054841246773);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,53.2553244999667);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,47.4296458787703);
\draw[draw=none,fill=color1] (axis cs:9,0) rectangle (axis cs:9.4,52.2691495323327);
\path [draw=black, thick]
(axis cs:-0.2,135.334955355857)
--(axis cs:-0.2,160.597155684066);

\path [draw=black, thick]
(axis cs:0.8,126.306072060371)
--(axis cs:0.8,158.537080059136);

\path [draw=black, thick]
(axis cs:1.8,124.120828846255)
--(axis cs:1.8,146.624828129568);

\path [draw=black, thick]
(axis cs:2.8,128.52500885373)
--(axis cs:2.8,153.685728854229);

\path [draw=black, thick]
(axis cs:3.8,139.711442568935)
--(axis cs:3.8,164.080250891992);

\path [draw=black, thick]
(axis cs:4.8,126.986689619037)
--(axis cs:4.8,158.474997642913);

\path [draw=black, thick]
(axis cs:5.8,140.97497267387)
--(axis cs:5.8,171.542454874762);

\path [draw=black, thick]
(axis cs:6.8,120.321979335363)
--(axis cs:6.8,145.949190058313);

\path [draw=black, thick]
(axis cs:7.8,105.966669085099)
--(axis cs:7.8,131.217013898695);

\path [draw=black, thick]
(axis cs:8.8,124.224828345904)
--(axis cs:8.8,160.706123747859);

\path [draw=black, thick]
(axis cs:0.2,43.1792008257653)
--(axis cs:0.2,61.7536302047993);

\path [draw=black, thick]
(axis cs:1.2,33.6448238907307)
--(axis cs:1.2,52.0278481777705);

\path [draw=black, thick]
(axis cs:2.2,46.9931696725232)
--(axis cs:2.2,65.7671105364627);

\path [draw=black, thick]
(axis cs:3.2,41.3172879327634)
--(axis cs:3.2,60.7394014098749);

\path [draw=black, thick]
(axis cs:4.2,41.9539565333193)
--(axis cs:4.2,63.2219569806585);

\path [draw=black, thick]
(axis cs:5.2,40.9484357081499)
--(axis cs:5.2,61.0446184696054);

\path [draw=black, thick]
(axis cs:6.2,39.1172785799565)
--(axis cs:6.2,60.4936896693982);

\path [draw=black, thick]
(axis cs:7.2,44.2754590738633)
--(axis cs:7.2,62.23518992607);

\path [draw=black, thick]
(axis cs:8.2,38.589791668685)
--(axis cs:8.2,56.2695000888557);

\path [draw=black, thick]
(axis cs:9.2,43.9539383338012)
--(axis cs:9.2,60.5843607308641);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_10_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.89, xmax=9.89,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9,STA 10},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=105,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,84.2562927631579);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,84.5675157894737);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,87.8876587719298);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,85.3770304824562);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,83.5698377192982);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,86.8896015350877);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,83.8181870614035);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,88.2484203947368);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,89.7796929824562);
\draw[draw=none,fill=color0] (axis cs:8.6,0) rectangle (axis cs:9,86.0527453947368);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,100);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,100);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,100);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,100);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,100);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,100);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,100);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,100);
\draw[draw=none,fill=color1] (axis cs:9,0) rectangle (axis cs:9.4,100);
\path [draw=black, thick]
(axis cs:-0.2,80.4128326088218)
--(axis cs:-0.2,88.099752917494);

\path [draw=black, thick]
(axis cs:0.8,81.2218623031357)
--(axis cs:0.8,87.9131692758117);

\path [draw=black, thick]
(axis cs:1.8,84.7385038759446)
--(axis cs:1.8,91.0368136679151);

\path [draw=black, thick]
(axis cs:2.8,82.5537292499714)
--(axis cs:2.8,88.2003317149409);

\path [draw=black, thick]
(axis cs:3.8,80.1631672646139)
--(axis cs:3.8,86.9765081739825);

\path [draw=black, thick]
(axis cs:4.8,83.7558654486872)
--(axis cs:4.8,90.0233376214883);

\path [draw=black, thick]
(axis cs:5.8,80.8138030869329)
--(axis cs:5.8,86.8225710358741);

\path [draw=black, thick]
(axis cs:6.8,85.5247519552222)
--(axis cs:6.8,90.9720888342515);

\path [draw=black, thick]
(axis cs:7.8,87.1172860275697)
--(axis cs:7.8,92.4420999373426);

\path [draw=black, thick]
(axis cs:8.8,81.7282350514875)
--(axis cs:8.8,90.3772557379862);

\path [draw=black, thick]
(axis cs:0.2,100)
--(axis cs:0.2,100);

\path [draw=black, thick]
(axis cs:1.2,100)
--(axis cs:1.2,100);

\path [draw=black, thick]
(axis cs:2.2,100)
--(axis cs:2.2,100);

\path [draw=black, thick]
(axis cs:3.2,100)
--(axis cs:3.2,100);

\path [draw=black, thick]
(axis cs:4.2,100)
--(axis cs:4.2,100);

\path [draw=black, thick]
(axis cs:5.2,100)
--(axis cs:5.2,100);

\path [draw=black, thick]
(axis cs:6.2,100)
--(axis cs:6.2,100);

\path [draw=black, thick]
(axis cs:7.2,100)
--(axis cs:7.2,100);

\path [draw=black, thick]
(axis cs:8.2,100)
--(axis cs:8.2,100);

\path [draw=black, thick]
(axis cs:9.2,100)
--(axis cs:9.2,100);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_10_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.87, xmax=9.47,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9,STA 10},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=180.623072112603,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,148.914119525597);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,145.229261209901);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,134.785273492066);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,140.317202747873);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,151.161850005143);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,144.9711389196);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,156.775637705928);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,135.53532674796);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,122.544853740242);
\draw[draw=none,fill=color0] (axis cs:8.6,0) rectangle (axis cs:9,140.906072785252);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,50.9829274424038);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,42.1016892512433);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,56.3966552095466);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,nan);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,55.6143511536367);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,nan);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,nan);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,nan);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,nan);
\draw[draw=none,fill=color1] (axis cs:9,0) rectangle (axis cs:9.4,nan);
\path [draw=black, thick]
(axis cs:-0.2,136.365292186151)
--(axis cs:-0.2,161.462946865044);

\path [draw=black, thick]
(axis cs:0.8,128.629441603098)
--(axis cs:0.8,161.829080816704);

\path [draw=black, thick]
(axis cs:1.8,123.50041344641)
--(axis cs:1.8,146.070133537723);

\path [draw=black, thick]
(axis cs:2.8,127.859428053774)
--(axis cs:2.8,152.774977441972);

\path [draw=black, thick]
(axis cs:3.8,138.89046703054)
--(axis cs:3.8,163.433232979746);

\path [draw=black, thick]
(axis cs:4.8,129.740019454442)
--(axis cs:4.8,160.202258384758);

\path [draw=black, thick]
(axis cs:5.8,141.529301971281)
--(axis cs:5.8,172.021973440574);

\path [draw=black, thick]
(axis cs:6.8,122.169464109016)
--(axis cs:6.8,148.901189386904);

\path [draw=black, thick]
(axis cs:7.8,108.666140514181)
--(axis cs:7.8,136.423566966303);

\path [draw=black, thick]
(axis cs:8.8,122.937538405357)
--(axis cs:8.8,158.874607165146);

\path [draw=black, thick]
(axis cs:0.2,41.923827035499)
--(axis cs:0.2,60.0420278493086);

\path [draw=black, thick]
(axis cs:1.2,32.9811276261387)
--(axis cs:1.2,51.2222508763479);

\path [draw=black, thick]
(axis cs:2.2,47.512965049495)
--(axis cs:2.2,65.2803453695983);

\path [draw=black, thick]
(axis cs:4.2,45.6013025612336)
--(axis cs:4.2,65.6273997460398);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_10_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.89, xmax=9.89,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9,STA 10},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=107.355414756479,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,84.2847932017544);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,84.4349067982456);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,88.1399403508772);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,85.3227322368421);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,83.9583826754386);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,87.173997368421);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,83.260477631579);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,88.3026401315789);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,88.8855546052632);
\draw[draw=none,fill=color0] (axis cs:8.6,0) rectangle (axis cs:9,86.5960065789474);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,99.9323673245614);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,100);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,100);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,79.9933721491228);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,99.9994046052632);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,76.5333486842105);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,93.3184096491228);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,86.6660712719298);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,79.8958903508772);
\draw[draw=none,fill=color1] (axis cs:9,0) rectangle (axis cs:9.4,76.4965120614035);
\path [draw=black, thick]
(axis cs:-0.2,80.4456200016373)
--(axis cs:-0.2,88.1239664018714);

\path [draw=black, thick]
(axis cs:0.8,81.0568252649633)
--(axis cs:0.8,87.8129883315279);

\path [draw=black, thick]
(axis cs:1.8,84.9334189376773)
--(axis cs:1.8,91.3464617640771);

\path [draw=black, thick]
(axis cs:2.8,82.4944918342941)
--(axis cs:2.8,88.1509726393901);

\path [draw=black, thick]
(axis cs:3.8,80.4396027429337)
--(axis cs:3.8,87.4771626079435);

\path [draw=black, thick]
(axis cs:4.8,83.992752160042)
--(axis cs:4.8,90.3552425768001);

\path [draw=black, thick]
(axis cs:5.8,80.2795156609283)
--(axis cs:5.8,86.2414396022296);

\path [draw=black, thick]
(axis cs:6.8,85.5629848182088)
--(axis cs:6.8,91.042295444949);

\path [draw=black, thick]
(axis cs:7.8,85.7804373773775)
--(axis cs:7.8,91.9906718331488);

\path [draw=black, thick]
(axis cs:8.8,82.3084829127003)
--(axis cs:8.8,90.8835302451945);

\path [draw=black, thick]
(axis cs:0.2,99.80243041823)
--(axis cs:0.2,100.062304230893);

\path [draw=black, thick]
(axis cs:1.2,100)
--(axis cs:1.2,100);

\path [draw=black, thick]
(axis cs:2.2,100)
--(axis cs:2.2,100);

\path [draw=black, thick]
(axis cs:3.2,65.6807365454404)
--(axis cs:3.2,94.3060077528052);

\path [draw=black, thick]
(axis cs:4.2,99.998257245979)
--(axis cs:4.2,100.000551964547);

\path [draw=black, thick]
(axis cs:5.2,61.4237545965664)
--(axis cs:5.2,91.6429427718547);

\path [draw=black, thick]
(axis cs:6.2,84.3935671492181)
--(axis cs:6.2,102.243252149028);

\path [draw=black, thick]
(axis cs:7.2,74.5017501264779)
--(axis cs:7.2,98.8303924173818);

\path [draw=black, thick]
(axis cs:8.2,65.5993500948068)
--(axis cs:8.2,94.1924306069476);

\path [draw=black, thick]
(axis cs:9.2,61.3925579508994)
--(axis cs:9.2,91.6004661719077);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_10_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.89, xmax=9.89,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9,STA 10},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=180.1195776185,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,147.966055519961);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,142.421576059754);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,135.372828487911);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,141.10536885398);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,151.895846730463);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,142.730843630975);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,156.258713774316);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,133.135584696838);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,118.591841491897);
\draw[draw=none,fill=color0] (axis cs:8.6,0) rectangle (axis cs:9,142.465476046882);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,4.65616829100044);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,4.6565988341201);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,4.65681500761256);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,4.65619564062911);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,4.65669802011157);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,4.65648532397184);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,4.65613344941656);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,4.65666350766234);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,4.65615880135701);
\draw[draw=none,fill=color1] (axis cs:9,0) rectangle (axis cs:9.4,4.65630448234424);
\path [draw=black, thick]
(axis cs:-0.2,135.334955355857)
--(axis cs:-0.2,160.597155684066);

\path [draw=black, thick]
(axis cs:0.8,126.306072060371)
--(axis cs:0.8,158.537080059136);

\path [draw=black, thick]
(axis cs:1.8,124.120828846255)
--(axis cs:1.8,146.624828129568);

\path [draw=black, thick]
(axis cs:2.8,128.52500885373)
--(axis cs:2.8,153.685728854229);

\path [draw=black, thick]
(axis cs:3.8,139.711442568935)
--(axis cs:3.8,164.080250891992);

\path [draw=black, thick]
(axis cs:4.8,126.986689619037)
--(axis cs:4.8,158.474997642913);

\path [draw=black, thick]
(axis cs:5.8,140.97497267387)
--(axis cs:5.8,171.542454874762);

\path [draw=black, thick]
(axis cs:6.8,120.321979335363)
--(axis cs:6.8,145.949190058313);

\path [draw=black, thick]
(axis cs:7.8,105.966669085099)
--(axis cs:7.8,131.217013898695);

\path [draw=black, thick]
(axis cs:8.8,124.224828345904)
--(axis cs:8.8,160.706123747859);

\path [draw=black, thick]
(axis cs:0.2,4.6559189357678)
--(axis cs:0.2,4.65641764623309);

\path [draw=black, thick]
(axis cs:1.2,4.65624434913237)
--(axis cs:1.2,4.65695331910783);

\path [draw=black, thick]
(axis cs:2.2,4.65647761158613)
--(axis cs:2.2,4.65715240363899);

\path [draw=black, thick]
(axis cs:3.2,4.6559238210044)
--(axis cs:3.2,4.65646746025381);

\path [draw=black, thick]
(axis cs:4.2,4.6563637538409)
--(axis cs:4.2,4.65703228638225);

\path [draw=black, thick]
(axis cs:5.2,4.65613799070459)
--(axis cs:5.2,4.65683265723909);

\path [draw=black, thick]
(axis cs:6.2,4.65590858605139)
--(axis cs:6.2,4.65635831278173);

\path [draw=black, thick]
(axis cs:7.2,4.65631581958106)
--(axis cs:7.2,4.65701119574362);

\path [draw=black, thick]
(axis cs:8.2,4.65594013151845)
--(axis cs:8.2,4.65637747119557);

\path [draw=black, thick]
(axis cs:9.2,4.65602341396549)
--(axis cs:9.2,4.656585550723);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_10_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.89, xmax=9.89,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9,STA 10},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=105,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,84.2562927631579);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,84.5675157894737);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,87.8876587719298);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,85.3770304824561);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,83.5698377192982);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,86.8896015350877);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,83.8181870614035);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,88.2484203947369);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,89.7796929824562);
\draw[draw=none,fill=color0] (axis cs:8.6,0) rectangle (axis cs:9,86.0527453947368);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,100);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,100);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,100);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,100);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,100);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,100);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,100);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,100);
\draw[draw=none,fill=color1] (axis cs:9,0) rectangle (axis cs:9.4,100);
\path [draw=black, thick]
(axis cs:-0.2,80.4128326088218)
--(axis cs:-0.2,88.0997529174941);

\path [draw=black, thick]
(axis cs:0.8,81.2218623031357)
--(axis cs:0.8,87.9131692758117);

\path [draw=black, thick]
(axis cs:1.8,84.7385038759446)
--(axis cs:1.8,91.0368136679151);

\path [draw=black, thick]
(axis cs:2.8,82.5537292499714)
--(axis cs:2.8,88.2003317149409);

\path [draw=black, thick]
(axis cs:3.8,80.1631672646139)
--(axis cs:3.8,86.9765081739826);

\path [draw=black, thick]
(axis cs:4.8,83.7558654486872)
--(axis cs:4.8,90.0233376214883);

\path [draw=black, thick]
(axis cs:5.8,80.8138030869329)
--(axis cs:5.8,86.8225710358741);

\path [draw=black, thick]
(axis cs:6.8,85.5247519552223)
--(axis cs:6.8,90.9720888342515);

\path [draw=black, thick]
(axis cs:7.8,87.1172860275697)
--(axis cs:7.8,92.4420999373426);

\path [draw=black, thick]
(axis cs:8.8,81.7282350514875)
--(axis cs:8.8,90.3772557379862);

\path [draw=black, thick]
(axis cs:0.2,100)
--(axis cs:0.2,100);

\path [draw=black, thick]
(axis cs:1.2,100)
--(axis cs:1.2,100);

\path [draw=black, thick]
(axis cs:2.2,100)
--(axis cs:2.2,100);

\path [draw=black, thick]
(axis cs:3.2,100)
--(axis cs:3.2,100);

\path [draw=black, thick]
(axis cs:4.2,100)
--(axis cs:4.2,100);

\path [draw=black, thick]
(axis cs:5.2,100)
--(axis cs:5.2,100);

\path [draw=black, thick]
(axis cs:6.2,100)
--(axis cs:6.2,100);

\path [draw=black, thick]
(axis cs:7.2,100)
--(axis cs:7.2,100);

\path [draw=black, thick]
(axis cs:8.2,100)
--(axis cs:8.2,100);

\path [draw=black, thick]
(axis cs:9.2,100)
--(axis cs:9.2,100);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_1_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=0, xmax=1,
xtick style={color=black},
xtick={0},
xticklabels={STA 1},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=black},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0}
]
\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_1_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=0, xmax=1,
xtick style={color=black},
xtick={0},
xticklabels={STA 1},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=black},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0}
]
\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_1_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=0, xmax=1,
xtick style={color=black},
xtick={0},
xticklabels={STA 1},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=black},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0}
]
\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_1_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=0, xmax=1,
xtick style={color=black},
xtick={0},
xticklabels={STA 1},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=black},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0}
]
\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_1_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=0, xmax=1,
xtick style={color=black},
xtick={0},
xticklabels={STA 1},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=black},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0}
]
\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_1_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=0, xmax=1,
xtick style={color=black},
xtick={0},
xticklabels={STA 1},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=black},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0}
]
\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_2_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.49, xmax=1.49,
xtick style={color=black},
xtick={0,1},
xticklabels={STA 1,STA 2},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=60.2668716152604,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,6.26890180769888);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,6.47486049856273);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,37.2654866619105);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,47.7716732257317);
\path [draw=black, thick]
(axis cs:-0.2,5.49538416850701)
--(axis cs:-0.2,7.04241944689075);

\path [draw=black, thick]
(axis cs:0.8,5.66263025027536)
--(axis cs:0.8,7.2870907468501);

\path [draw=black, thick]
(axis cs:0.2,28.0296355722501)
--(axis cs:0.2,46.5013377515709);

\path [draw=black, thick]
(axis cs:1.2,38.1463258655011)
--(axis cs:1.2,57.3970205859622);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_2_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.49, xmax=1.49,
xtick style={color=black},
xtick={0,1},
xticklabels={STA 1,STA 2},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=105,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,100);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,100);
\path [draw=black, thick]
(axis cs:-0.2,100)
--(axis cs:-0.2,100);

\path [draw=black, thick]
(axis cs:0.8,100)
--(axis cs:0.8,100);

\path [draw=black, thick]
(axis cs:0.2,100)
--(axis cs:0.2,100);

\path [draw=black, thick]
(axis cs:1.2,100)
--(axis cs:1.2,100);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_2_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.49, xmax=1.49,
xtick style={color=black},
xtick={0,1},
xticklabels={STA 1,STA 2},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=10.0948866514716,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,6.26890180769888);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,6.47486049856273);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,7.21930006769146);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,7.869360663524);
\path [draw=black, thick]
(axis cs:-0.2,5.49538416850701)
--(axis cs:-0.2,7.04241944689075);

\path [draw=black, thick]
(axis cs:0.8,5.66263025027536)
--(axis cs:0.8,7.2870907468501);

\path [draw=black, thick]
(axis cs:0.2,6.28698509442955)
--(axis cs:0.2,8.15161504095337);

\path [draw=black, thick]
(axis cs:1.2,6.1245435637417)
--(axis cs:1.2,9.61417776330631);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_2_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.49, xmax=1.49,
xtick style={color=black},
xtick={0,1},
xticklabels={STA 1,STA 2},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=105,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,100);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,100);
\path [draw=black, thick]
(axis cs:-0.2,100)
--(axis cs:-0.2,100);

\path [draw=black, thick]
(axis cs:0.8,100)
--(axis cs:0.8,100);

\path [draw=black, thick]
(axis cs:0.2,100)
--(axis cs:0.2,100);

\path [draw=black, thick]
(axis cs:1.2,100)
--(axis cs:1.2,100);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_2_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.49, xmax=1.49,
xtick style={color=black},
xtick={0,1},
xticklabels={STA 1,STA 2},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=7.6514452841926,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,6.26890180769888);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,6.47486049856273);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,4.65586568168736);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,4.65590136528578);
\path [draw=black, thick]
(axis cs:-0.2,5.49538416850701)
--(axis cs:-0.2,7.04241944689074);

\path [draw=black, thick]
(axis cs:0.8,5.66263025027536)
--(axis cs:0.8,7.2870907468501);

\path [draw=black, thick]
(axis cs:0.2,4.6557433678863)
--(axis cs:0.2,4.65598799548841);

\path [draw=black, thick]
(axis cs:1.2,4.65578267563304)
--(axis cs:1.2,4.65602005493853);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_2_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.49, xmax=1.49,
xtick style={color=black},
xtick={0,1},
xticklabels={STA 1,STA 2},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=105,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,100);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,100);
\path [draw=black, thick]
(axis cs:-0.2,100)
--(axis cs:-0.2,100);

\path [draw=black, thick]
(axis cs:0.8,100)
--(axis cs:0.8,100);

\path [draw=black, thick]
(axis cs:0.2,100)
--(axis cs:0.2,100);

\path [draw=black, thick]
(axis cs:1.2,100)
--(axis cs:1.2,100);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_3_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.54, xmax=2.54,
xtick style={color=black},
xtick={0,1,2},
xticklabels={STA 1,STA 2,STA 3},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=63.5139563977837,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,6.7198064341223);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,7.33847607305387);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,7.19918475532191);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,49.6988397055068);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,51.113420457072);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,49.3578374998085);
\path [draw=black, thick]
(axis cs:-0.2,5.6604385382126)
--(axis cs:-0.2,7.77917433003201);

\path [draw=black, thick]
(axis cs:0.8,6.1445098257589)
--(axis cs:0.8,8.53244232034884);

\path [draw=black, thick]
(axis cs:1.8,6.18954531245622)
--(axis cs:1.8,8.20882419818761);

\path [draw=black, thick]
(axis cs:0.2,38.90819712741)
--(axis cs:0.2,60.4894822836036);

\path [draw=black, thick]
(axis cs:1.2,42.4291724968462)
--(axis cs:1.2,59.7976684172979);

\path [draw=black, thick]
(axis cs:2.2,41.3105358913275)
--(axis cs:2.2,57.4051391082895);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_3_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.5,0.09)}, anchor=south, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.54, xmax=2.54,
xtick style={color=black},
xtick={0,1,2},
xticklabels={STA 1,STA 2,STA 3},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=105,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,100);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,100);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,100);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,100);
\path [draw=black, thick]
(axis cs:-0.2,100)
--(axis cs:-0.2,100);

\path [draw=black, thick]
(axis cs:0.8,100)
--(axis cs:0.8,100);

\path [draw=black, thick]
(axis cs:1.8,100)
--(axis cs:1.8,100);

\path [draw=black, thick]
(axis cs:0.2,100)
--(axis cs:0.2,100);

\path [draw=black, thick]
(axis cs:1.2,100)
--(axis cs:1.2,100);

\path [draw=black, thick]
(axis cs:2.2,100)
--(axis cs:2.2,100);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_3_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.54, xmax=2.54,
xtick style={color=black},
xtick={0,1,2},
xticklabels={STA 1,STA 2,STA 3},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=13.3526025926026,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,6.7198064341223);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,7.33847607305387);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,7.19918475532191);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,9.26829956938015);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,9.64118468010786);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,9.99457694125317);
\path [draw=black, thick]
(axis cs:-0.2,5.66043853821259)
--(axis cs:-0.2,7.77917433003201);

\path [draw=black, thick]
(axis cs:0.8,6.1445098257589)
--(axis cs:0.8,8.53244232034885);

\path [draw=black, thick]
(axis cs:1.8,6.18954531245622)
--(axis cs:1.8,8.20882419818761);

\path [draw=black, thick]
(axis cs:0.2,7.09176686805218)
--(axis cs:0.2,11.4448322707081);

\path [draw=black, thick]
(axis cs:1.2,6.80815546856691)
--(axis cs:1.2,12.4742138916488);

\path [draw=black, thick]
(axis cs:2.2,7.27238950859909)
--(axis cs:2.2,12.7167643739072);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_3_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.5,0.09)}, anchor=south, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.54, xmax=2.54,
xtick style={color=black},
xtick={0,1,2},
xticklabels={STA 1,STA 2,STA 3},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=105,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,100);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,100);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,100);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,100);
\path [draw=black, thick]
(axis cs:-0.2,100)
--(axis cs:-0.2,100);

\path [draw=black, thick]
(axis cs:0.8,100)
--(axis cs:0.8,100);

\path [draw=black, thick]
(axis cs:1.8,100)
--(axis cs:1.8,100);

\path [draw=black, thick]
(axis cs:0.2,100)
--(axis cs:0.2,100);

\path [draw=black, thick]
(axis cs:1.2,100)
--(axis cs:1.2,100);

\path [draw=black, thick]
(axis cs:2.2,100)
--(axis cs:2.2,100);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_3_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.54, xmax=2.54,
xtick style={color=black},
xtick={0,1,2},
xticklabels={STA 1,STA 2,STA 3},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=8.95906443636629,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,6.7198064341223);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,7.33847607305387);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,7.19918475532191);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,4.65602856988937);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,4.65620668705253);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,4.65605560841586);
\path [draw=black, thick]
(axis cs:-0.2,5.66043853821259)
--(axis cs:-0.2,7.77917433003201);

\path [draw=black, thick]
(axis cs:0.8,6.1445098257589)
--(axis cs:0.8,8.53244232034885);

\path [draw=black, thick]
(axis cs:1.8,6.18954531245622)
--(axis cs:1.8,8.20882419818761);

\path [draw=black, thick]
(axis cs:0.2,4.6557952638342)
--(axis cs:0.2,4.65626187594453);

\path [draw=black, thick]
(axis cs:1.2,4.65601732653039)
--(axis cs:1.2,4.65639604757468);

\path [draw=black, thick]
(axis cs:2.2,4.65589357715762)
--(axis cs:2.2,4.6562176396741);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_3_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.5,0.09)}, anchor=south, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.54, xmax=2.54,
xtick style={color=black},
xtick={0,1,2},
xticklabels={STA 1,STA 2,STA 3},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=105,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,100);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,100);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,100);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,100);
\path [draw=black, thick]
(axis cs:-0.2,100)
--(axis cs:-0.2,100);

\path [draw=black, thick]
(axis cs:0.8,100)
--(axis cs:0.8,100);

\path [draw=black, thick]
(axis cs:1.8,100)
--(axis cs:1.8,100);

\path [draw=black, thick]
(axis cs:0.2,100)
--(axis cs:0.2,100);

\path [draw=black, thick]
(axis cs:1.2,100)
--(axis cs:1.2,100);

\path [draw=black, thick]
(axis cs:2.2,100)
--(axis cs:2.2,100);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_4_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=65.8619840026842,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,8.51606216825566);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,7.17006447231536);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,7.12207491667739);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,8.07518690816623);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,52.1817322003576);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50.1437445630691);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,49.2919732672535);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,53.6880840954652);
\path [draw=black, thick]
(axis cs:-0.2,7.09267389988134)
--(axis cs:-0.2,9.93945043662997);

\path [draw=black, thick]
(axis cs:0.8,6.06317755791348)
--(axis cs:0.8,8.27695138671724);

\path [draw=black, thick]
(axis cs:1.8,6.06500258118578)
--(axis cs:1.8,8.17914725216899);

\path [draw=black, thick]
(axis cs:2.8,6.83948447820779)
--(axis cs:2.8,9.31088933812466);

\path [draw=black, thick]
(axis cs:0.2,42.9216454653002)
--(axis cs:0.2,61.441818935415);

\path [draw=black, thick]
(axis cs:1.2,40.4440556592103)
--(axis cs:1.2,59.843433466928);

\path [draw=black, thick]
(axis cs:2.2,39.525332490749)
--(axis cs:2.2,59.058614043758);

\path [draw=black, thick]
(axis cs:3.2,44.650469140755)
--(axis cs:3.2,62.7256990501755);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_4_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=105,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,100);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,100);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,100);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,100);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,100);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,100);
\path [draw=black, thick]
(axis cs:-0.2,100)
--(axis cs:-0.2,100);

\path [draw=black, thick]
(axis cs:0.8,100)
--(axis cs:0.8,100);

\path [draw=black, thick]
(axis cs:1.8,100)
--(axis cs:1.8,100);

\path [draw=black, thick]
(axis cs:2.8,100)
--(axis cs:2.8,100);

\path [draw=black, thick]
(axis cs:0.2,100)
--(axis cs:0.2,100);

\path [draw=black, thick]
(axis cs:1.2,100)
--(axis cs:1.2,100);

\path [draw=black, thick]
(axis cs:2.2,100)
--(axis cs:2.2,100);

\path [draw=black, thick]
(axis cs:3.2,100)
--(axis cs:3.2,100);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_4_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=21.7649776830028,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,8.51606216825565);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,7.17006447231536);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,7.12207491667739);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,8.07518690816623);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,11.169302944787);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,13.5410748842483);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,12.2127318039247);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,16.6567284748537);
\path [draw=black, thick]
(axis cs:-0.2,7.09267389988134)
--(axis cs:-0.2,9.93945043662997);

\path [draw=black, thick]
(axis cs:0.8,6.06317755791348)
--(axis cs:0.8,8.27695138671724);

\path [draw=black, thick]
(axis cs:1.8,6.06500258118578)
--(axis cs:1.8,8.17914725216899);

\path [draw=black, thick]
(axis cs:2.8,6.83948447820779)
--(axis cs:2.8,9.31088933812466);

\path [draw=black, thick]
(axis cs:0.2,8.41913389464427)
--(axis cs:0.2,13.9194719949297);

\path [draw=black, thick]
(axis cs:1.2,10.4727468404021)
--(axis cs:1.2,16.6094029280946);

\path [draw=black, thick]
(axis cs:2.2,9.33172046421041)
--(axis cs:2.2,15.093743143639);

\path [draw=black, thick]
(axis cs:3.2,12.5849067754191)
--(axis cs:3.2,20.7285501742884);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_4_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=105.000193187592,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,100);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,100);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,100);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,99.9998015350877);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,100);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,100);
\path [draw=black, thick]
(axis cs:-0.2,100)
--(axis cs:-0.2,100);

\path [draw=black, thick]
(axis cs:0.8,100)
--(axis cs:0.8,100);

\path [draw=black, thick]
(axis cs:1.8,100)
--(axis cs:1.8,100);

\path [draw=black, thick]
(axis cs:2.8,100)
--(axis cs:2.8,100);

\path [draw=black, thick]
(axis cs:0.2,100)
--(axis cs:0.2,100);

\path [draw=black, thick]
(axis cs:1.2,99.999419081993)
--(axis cs:1.2,100.000183988182);

\path [draw=black, thick]
(axis cs:2.2,100)
--(axis cs:2.2,100);

\path [draw=black, thick]
(axis cs:3.2,100)
--(axis cs:3.2,100);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_4_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=10.4364229584615,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,8.51606216825566);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,7.17006447231535);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,7.12207491667738);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,8.07518690816623);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,4.65622280820641);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,4.65616163140248);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,4.65646969493172);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,4.65628227886655);
\path [draw=black, thick]
(axis cs:-0.2,7.09267389988134)
--(axis cs:-0.2,9.93945043662997);

\path [draw=black, thick]
(axis cs:0.8,6.06317755791348)
--(axis cs:0.8,8.27695138671723);

\path [draw=black, thick]
(axis cs:1.8,6.06500258118578)
--(axis cs:1.8,8.17914725216899);

\path [draw=black, thick]
(axis cs:2.8,6.83948447820779)
--(axis cs:2.8,9.31088933812466);

\path [draw=black, thick]
(axis cs:0.2,4.65594136102089)
--(axis cs:0.2,4.65650425539192);

\path [draw=black, thick]
(axis cs:1.2,4.65596272233492)
--(axis cs:1.2,4.65636054047004);

\path [draw=black, thick]
(axis cs:2.2,4.65622362109822)
--(axis cs:2.2,4.65671576876522);

\path [draw=black, thick]
(axis cs:3.2,4.6559930675647)
--(axis cs:3.2,4.6565714901684);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_4_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=105,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,100);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,100);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,100);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,100);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,100);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,100);
\path [draw=black, thick]
(axis cs:-0.2,100)
--(axis cs:-0.2,100);

\path [draw=black, thick]
(axis cs:0.8,100)
--(axis cs:0.8,100);

\path [draw=black, thick]
(axis cs:1.8,100)
--(axis cs:1.8,100);

\path [draw=black, thick]
(axis cs:2.8,100)
--(axis cs:2.8,100);

\path [draw=black, thick]
(axis cs:0.2,100)
--(axis cs:0.2,100);

\path [draw=black, thick]
(axis cs:1.2,100)
--(axis cs:1.2,100);

\path [draw=black, thick]
(axis cs:2.2,100)
--(axis cs:2.2,100);

\path [draw=black, thick]
(axis cs:3.2,100)
--(axis cs:3.2,100);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_5_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.64, xmax=4.64,
xtick style={color=black},
xtick={0,1,2,3,4},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=68.7828411122635,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,8.55983077427638);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,8.20929003116155);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,7.64656534405538);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,6.89952659141443);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,7.58863349150124);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,37.5161040612788);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,49.7388613939652);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,55.8944362478938);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,44.5174734304708);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,50.747517278694);
\path [draw=black, thick]
(axis cs:-0.2,7.09010797806929)
--(axis cs:-0.2,10.0295535704835);

\path [draw=black, thick]
(axis cs:0.8,6.88333518344431)
--(axis cs:0.8,9.53524487887878);

\path [draw=black, thick]
(axis cs:1.8,6.53655484510402)
--(axis cs:1.8,8.75657584300675);

\path [draw=black, thick]
(axis cs:2.8,6.01597336141842)
--(axis cs:2.8,7.78307982141044);

\path [draw=black, thick]
(axis cs:3.8,6.44386858753246)
--(axis cs:3.8,8.73339839547003);

\path [draw=black, thick]
(axis cs:0.2,28.2544563418376)
--(axis cs:0.2,46.7777517807201);

\path [draw=black, thick]
(axis cs:1.2,40.6107074032344)
--(axis cs:1.2,58.867015384696);

\path [draw=black, thick]
(axis cs:2.2,46.2814047698224)
--(axis cs:2.2,65.5074677259652);

\path [draw=black, thick]
(axis cs:3.2,34.807276976851)
--(axis cs:3.2,54.2276698840907);

\path [draw=black, thick]
(axis cs:4.2,41.1204558494146)
--(axis cs:4.2,60.3745787079733);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_5_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.64, xmax=4.64,
xtick style={color=black},
xtick={0,1,2,3,4},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=105,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,100);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,100);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,100);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,100);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,100);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,100);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,100);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,100);
\path [draw=black, thick]
(axis cs:-0.2,100)
--(axis cs:-0.2,100);

\path [draw=black, thick]
(axis cs:0.8,100)
--(axis cs:0.8,100);

\path [draw=black, thick]
(axis cs:1.8,100)
--(axis cs:1.8,100);

\path [draw=black, thick]
(axis cs:2.8,100)
--(axis cs:2.8,100);

\path [draw=black, thick]
(axis cs:3.8,100)
--(axis cs:3.8,100);

\path [draw=black, thick]
(axis cs:0.2,100)
--(axis cs:0.2,100);

\path [draw=black, thick]
(axis cs:1.2,100)
--(axis cs:1.2,100);

\path [draw=black, thick]
(axis cs:2.2,100)
--(axis cs:2.2,100);

\path [draw=black, thick]
(axis cs:3.2,100)
--(axis cs:3.2,100);

\path [draw=black, thick]
(axis cs:4.2,100)
--(axis cs:4.2,100);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_5_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.64, xmax=4.64,
xtick style={color=black},
xtick={0,1,2,3,4},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=22.4745206921996,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,8.55983077427638);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,8.20929003116154);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,7.64656534405538);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,6.89952659141443);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,7.58863349150124);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,13.6936774521591);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,17.4152465059587);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,15.3854282520018);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,15.8582126441516);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,16.945758730563);
\path [draw=black, thick]
(axis cs:-0.2,7.09010797806929)
--(axis cs:-0.2,10.0295535704835);

\path [draw=black, thick]
(axis cs:0.8,6.88333518344431)
--(axis cs:0.8,9.53524487887878);

\path [draw=black, thick]
(axis cs:1.8,6.53655484510402)
--(axis cs:1.8,8.75657584300675);

\path [draw=black, thick]
(axis cs:2.8,6.01597336141842)
--(axis cs:2.8,7.78307982141044);

\path [draw=black, thick]
(axis cs:3.8,6.44386858753246)
--(axis cs:3.8,8.73339839547002);

\path [draw=black, thick]
(axis cs:0.2,9.7853899354376)
--(axis cs:0.2,17.6019649688806);

\path [draw=black, thick]
(axis cs:1.2,13.426187590775)
--(axis cs:1.2,21.4043054211425);

\path [draw=black, thick]
(axis cs:2.2,12.0423907987214)
--(axis cs:2.2,18.7284657052821);

\path [draw=black, thick]
(axis cs:3.2,11.5326540049163)
--(axis cs:3.2,20.1837712833868);

\path [draw=black, thick]
(axis cs:4.2,12.6120096288933)
--(axis cs:4.2,21.2795078322326);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_5_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.64, xmax=4.64,
xtick style={color=black},
xtick={0,1,2,3,4},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=105.000260314057,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,100);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,100);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,100);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,100);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,100);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,99.9994046052632);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,100);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,99.9998015350877);
\path [draw=black, thick]
(axis cs:-0.2,100)
--(axis cs:-0.2,100);

\path [draw=black, thick]
(axis cs:0.8,100)
--(axis cs:0.8,100);

\path [draw=black, thick]
(axis cs:1.8,100)
--(axis cs:1.8,100);

\path [draw=black, thick]
(axis cs:2.8,100)
--(axis cs:2.8,100);

\path [draw=black, thick]
(axis cs:3.8,100)
--(axis cs:3.8,100);

\path [draw=black, thick]
(axis cs:0.2,100)
--(axis cs:0.2,100);

\path [draw=black, thick]
(axis cs:1.2,100)
--(axis cs:1.2,100);

\path [draw=black, thick]
(axis cs:2.2,99.9985612923764)
--(axis cs:2.2,100.00024791815);

\path [draw=black, thick]
(axis cs:3.2,100)
--(axis cs:3.2,100);

\path [draw=black, thick]
(axis cs:4.2,99.999419081993)
--(axis cs:4.2,100.000183988182);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_5_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.64, xmax=4.64,
xtick style={color=black},
xtick={0,1,2,3,4},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=10.4732659993827,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,8.49738083307515);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,8.19601548303108);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,7.62119834756858);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,6.96057196449534);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,7.58735178400433);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,4.65628673804664);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,4.65646500689867);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,4.65646374311153);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,4.65609559679655);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,4.65604557512147);
\path [draw=black, thick]
(axis cs:-0.2,7.02022261911917)
--(axis cs:-0.2,9.97453904703113);

\path [draw=black, thick]
(axis cs:0.8,6.87452130064816)
--(axis cs:0.8,9.51750966541399);

\path [draw=black, thick]
(axis cs:1.8,6.52285916073667)
--(axis cs:1.8,8.71953753440049);

\path [draw=black, thick]
(axis cs:2.8,6.07552821924575)
--(axis cs:2.8,7.84561570974494);

\path [draw=black, thick]
(axis cs:3.8,6.44231464920421)
--(axis cs:3.8,8.73238891880445);

\path [draw=black, thick]
(axis cs:0.2,4.65600571425534)
--(axis cs:0.2,4.65656776183794);

\path [draw=black, thick]
(axis cs:1.2,4.65618272895639)
--(axis cs:1.2,4.65674728484094);

\path [draw=black, thick]
(axis cs:2.2,4.65618635211891)
--(axis cs:2.2,4.65674113410416);

\path [draw=black, thick]
(axis cs:3.2,4.65583893068872)
--(axis cs:3.2,4.65635226290438);

\path [draw=black, thick]
(axis cs:4.2,4.65580459464571)
--(axis cs:4.2,4.65628655559722);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_5_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.64, xmax=4.64,
xtick style={color=black},
xtick={0,1,2,3,4},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=105,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,100);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,100);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,100);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,100);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,100);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,100);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,100);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,100);
\path [draw=black, thick]
(axis cs:-0.2,100)
--(axis cs:-0.2,100);

\path [draw=black, thick]
(axis cs:0.8,100)
--(axis cs:0.8,100);

\path [draw=black, thick]
(axis cs:1.8,100)
--(axis cs:1.8,100);

\path [draw=black, thick]
(axis cs:2.8,100)
--(axis cs:2.8,100);

\path [draw=black, thick]
(axis cs:3.8,100)
--(axis cs:3.8,100);

\path [draw=black, thick]
(axis cs:0.2,100)
--(axis cs:0.2,100);

\path [draw=black, thick]
(axis cs:1.2,100)
--(axis cs:1.2,100);

\path [draw=black, thick]
(axis cs:2.2,100)
--(axis cs:2.2,100);

\path [draw=black, thick]
(axis cs:3.2,100)
--(axis cs:3.2,100);

\path [draw=black, thick]
(axis cs:4.2,100)
--(axis cs:4.2,100);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_6_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.69, xmax=5.69,
xtick style={color=black},
xtick={0,1,2,3,4,5},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=70.3865423571798,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,11.4727933729902);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,9.56327848715709);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,9.56360026882493);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,10.586102695576);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,9.22087069965738);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,8.32094520737449);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,42.4968795777195);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50.7693338181776);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,51.6355205911637);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,49.9194908405051);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,42.4954954395046);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,57.7634072939654);
\path [draw=black, thick]
(axis cs:-0.2,9.31332409224066)
--(axis cs:-0.2,13.6322626537397);

\path [draw=black, thick]
(axis cs:0.8,7.87571251457124)
--(axis cs:0.8,11.250844459743);

\path [draw=black, thick]
(axis cs:1.8,7.50364139728708)
--(axis cs:1.8,11.6235591403628);

\path [draw=black, thick]
(axis cs:2.8,8.37485647686837)
--(axis cs:2.8,12.7973489142836);

\path [draw=black, thick]
(axis cs:3.8,7.3294418489041)
--(axis cs:3.8,11.1122995504107);

\path [draw=black, thick]
(axis cs:4.8,6.34316925300768)
--(axis cs:4.8,10.2987211617413);

\path [draw=black, thick]
(axis cs:0.2,34.5839099886938)
--(axis cs:0.2,50.4098491667451);

\path [draw=black, thick]
(axis cs:1.2,43.0454037032139)
--(axis cs:1.2,58.4932639331413);

\path [draw=black, thick]
(axis cs:2.2,42.7884778689707)
--(axis cs:2.2,60.4825633133566);

\path [draw=black, thick]
(axis cs:3.2,39.24645677151)
--(axis cs:3.2,60.5925249095003);

\path [draw=black, thick]
(axis cs:4.2,35.6101438643791)
--(axis cs:4.2,49.38084701463);

\path [draw=black, thick]
(axis cs:5.2,48.4920123429977)
--(axis cs:5.2,67.0348022449332);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_6_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.69, xmax=5.69,
xtick style={color=black},
xtick={0,1,2,3,4,5},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=105.000045972228,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,99.9994046052631);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,100);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,100);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,100);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,100);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,100);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,100);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,100);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,100);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,100);
\path [draw=black, thick]
(axis cs:-0.2,100)
--(axis cs:-0.2,100);

\path [draw=black, thick]
(axis cs:0.8,99.9987654274523)
--(axis cs:0.8,100.000043783074);

\path [draw=black, thick]
(axis cs:1.8,100)
--(axis cs:1.8,100);

\path [draw=black, thick]
(axis cs:2.8,100)
--(axis cs:2.8,100);

\path [draw=black, thick]
(axis cs:3.8,100)
--(axis cs:3.8,100);

\path [draw=black, thick]
(axis cs:4.8,100)
--(axis cs:4.8,100);

\path [draw=black, thick]
(axis cs:0.2,100)
--(axis cs:0.2,100);

\path [draw=black, thick]
(axis cs:1.2,100)
--(axis cs:1.2,100);

\path [draw=black, thick]
(axis cs:2.2,100)
--(axis cs:2.2,100);

\path [draw=black, thick]
(axis cs:3.2,100)
--(axis cs:3.2,100);

\path [draw=black, thick]
(axis cs:4.2,100)
--(axis cs:4.2,100);

\path [draw=black, thick]
(axis cs:5.2,100)
--(axis cs:5.2,100);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_6_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.69, xmax=5.69,
xtick style={color=black},
xtick={0,1,2,3,4,5},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=35.3038637875705,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,11.4727933729902);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,9.5632784871571);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,9.56360026882493);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,10.586102695576);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,9.22087069965738);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,8.32094520737449);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,18.7026902925086);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,22.9949453258462);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,23.054747375594);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,19.0733294266562);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,29.4776792372182);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,23.6552694716752);
\path [draw=black, thick]
(axis cs:-0.2,9.31332409224066)
--(axis cs:-0.2,13.6322626537397);

\path [draw=black, thick]
(axis cs:0.8,7.87571251457124)
--(axis cs:0.8,11.250844459743);

\path [draw=black, thick]
(axis cs:1.8,7.50364139728707)
--(axis cs:1.8,11.6235591403628);

\path [draw=black, thick]
(axis cs:2.8,8.37485647686837)
--(axis cs:2.8,12.7973489142836);

\path [draw=black, thick]
(axis cs:3.8,7.3294418489041)
--(axis cs:3.8,11.1122995504107);

\path [draw=black, thick]
(axis cs:4.8,6.34316925300768)
--(axis cs:4.8,10.2987211617413);

\path [draw=black, thick]
(axis cs:0.2,13.9354108766102)
--(axis cs:0.2,23.4699697084069);

\path [draw=black, thick]
(axis cs:1.2,18.4473323317957)
--(axis cs:1.2,27.5425583198966);

\path [draw=black, thick]
(axis cs:2.2,17.2564725735371)
--(axis cs:2.2,28.853022177651);

\path [draw=black, thick]
(axis cs:3.2,14.8247361022445)
--(axis cs:3.2,23.3219227510679);

\path [draw=black, thick]
(axis cs:4.2,25.3326310577027)
--(axis cs:4.2,33.6227274167338);

\path [draw=black, thick]
(axis cs:5.2,18.6462322995746)
--(axis cs:5.2,28.6643066437758);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_6_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.69, xmax=5.69,
xtick style={color=black},
xtick={0,1,2,3,4,5},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=105.000600309507,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,99.9994046052631);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,100);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,100);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,100);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,100);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,99.9996030701754);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,99.9990076754386);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,99.9998015350877);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,99.9990076754386);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,100);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,99.9996030701754);
\path [draw=black, thick]
(axis cs:-0.2,100)
--(axis cs:-0.2,100);

\path [draw=black, thick]
(axis cs:0.8,99.9987654274523)
--(axis cs:0.8,100.000043783074);

\path [draw=black, thick]
(axis cs:1.8,100)
--(axis cs:1.8,100);

\path [draw=black, thick]
(axis cs:2.8,100)
--(axis cs:2.8,100);

\path [draw=black, thick]
(axis cs:3.8,100)
--(axis cs:3.8,100);

\path [draw=black, thick]
(axis cs:4.8,100)
--(axis cs:4.8,100);

\path [draw=black, thick]
(axis cs:0.2,99.9990716069805)
--(axis cs:0.2,100.00013453337);

\path [draw=black, thick]
(axis cs:1.2,99.9978960404115)
--(axis cs:1.2,100.000119310466);

\path [draw=black, thick]
(axis cs:2.2,99.999419081993)
--(axis cs:2.2,100.000183988182);

\path [draw=black, thick]
(axis cs:3.2,99.9974436275373)
--(axis cs:3.2,100.00057172334);

\path [draw=black, thick]
(axis cs:4.2,100)
--(axis cs:4.2,100);

\path [draw=black, thick]
(axis cs:5.2,99.9990716069805)
--(axis cs:5.2,100.00013453337);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_6_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.69, xmax=5.69,
xtick style={color=black},
xtick={0,1,2,3,4,5},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=14.3138757864267,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,11.4727933729902);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,9.56327848715709);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,9.56360026882493);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,10.586102695576);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,9.22087069965738);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,8.32094520737449);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,4.65652631646188);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,4.65632341419825);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,4.65632687869079);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,4.65662466208791);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,4.65618088851653);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,4.65636922811306);
\path [draw=black, thick]
(axis cs:-0.2,9.31332409224066)
--(axis cs:-0.2,13.6322626537397);

\path [draw=black, thick]
(axis cs:0.8,7.87571251457124)
--(axis cs:0.8,11.250844459743);

\path [draw=black, thick]
(axis cs:1.8,7.50364139728707)
--(axis cs:1.8,11.6235591403628);

\path [draw=black, thick]
(axis cs:2.8,8.37485647686837)
--(axis cs:2.8,12.7973489142836);

\path [draw=black, thick]
(axis cs:3.8,7.3294418489041)
--(axis cs:3.8,11.1122995504107);

\path [draw=black, thick]
(axis cs:4.8,6.34316925300768)
--(axis cs:4.8,10.2987211617413);

\path [draw=black, thick]
(axis cs:0.2,4.65610731321788)
--(axis cs:0.2,4.65694531970587);

\path [draw=black, thick]
(axis cs:1.2,4.65603194745829)
--(axis cs:1.2,4.65661488093821);

\path [draw=black, thick]
(axis cs:2.2,4.65611744645325)
--(axis cs:2.2,4.65653631092834);

\path [draw=black, thick]
(axis cs:3.2,4.65635611937237)
--(axis cs:3.2,4.65689320480345);

\path [draw=black, thick]
(axis cs:4.2,4.65593101653434)
--(axis cs:4.2,4.65643076049871);

\path [draw=black, thick]
(axis cs:5.2,4.65596153303656)
--(axis cs:5.2,4.65677692318956);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_6_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.69, xmax=5.69,
xtick style={color=black},
xtick={0,1,2,3,4,5},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=105.000045972228,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,99.9994046052631);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,100);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,100);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,100);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,100);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,100);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,100);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,100);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,100);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,100);
\path [draw=black, thick]
(axis cs:-0.2,100)
--(axis cs:-0.2,100);

\path [draw=black, thick]
(axis cs:0.8,99.9987654274523)
--(axis cs:0.8,100.000043783074);

\path [draw=black, thick]
(axis cs:1.8,100)
--(axis cs:1.8,100);

\path [draw=black, thick]
(axis cs:2.8,100)
--(axis cs:2.8,100);

\path [draw=black, thick]
(axis cs:3.8,100)
--(axis cs:3.8,100);

\path [draw=black, thick]
(axis cs:4.8,100)
--(axis cs:4.8,100);

\path [draw=black, thick]
(axis cs:0.2,100)
--(axis cs:0.2,100);

\path [draw=black, thick]
(axis cs:1.2,100)
--(axis cs:1.2,100);

\path [draw=black, thick]
(axis cs:2.2,100)
--(axis cs:2.2,100);

\path [draw=black, thick]
(axis cs:3.2,100)
--(axis cs:3.2,100);

\path [draw=black, thick]
(axis cs:4.2,100)
--(axis cs:4.2,100);

\path [draw=black, thick]
(axis cs:5.2,100)
--(axis cs:5.2,100);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_7_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.74, xmax=6.74,
xtick style={color=black},
xtick={0,1,2,3,4,5,6},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=71.7359992908983,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,12.9081199922876);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,11.9576400843062);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,12.2696308797353);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,9.25236146634636);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,11.0132677173829);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,11.5105602520378);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,10.9847517796865);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,44.7723371046562);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50.1684554420574);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,44.9549279192923);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,48.2018785503588);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,50.6883955655543);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,57.9271074740625);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,52.5670397715523);
\path [draw=black, thick]
(axis cs:-0.2,10.6836852320053)
--(axis cs:-0.2,15.1325547525698);

\path [draw=black, thick]
(axis cs:0.8,9.52159221865124)
--(axis cs:0.8,14.3936879499612);

\path [draw=black, thick]
(axis cs:1.8,9.86250330336173)
--(axis cs:1.8,14.6767584561089);

\path [draw=black, thick]
(axis cs:2.8,7.49748373254812)
--(axis cs:2.8,11.0072392001446);

\path [draw=black, thick]
(axis cs:3.8,8.40135517132303)
--(axis cs:3.8,13.6251802634428);

\path [draw=black, thick]
(axis cs:4.8,9.44843954768164)
--(axis cs:4.8,13.572680956394);

\path [draw=black, thick]
(axis cs:5.8,8.79724142390751)
--(axis cs:5.8,13.1722621354655);

\path [draw=black, thick]
(axis cs:0.2,36.1752052066637)
--(axis cs:0.2,53.3694690026486);

\path [draw=black, thick]
(axis cs:1.2,41.7470010185553)
--(axis cs:1.2,58.5899098655596);

\path [draw=black, thick]
(axis cs:2.2,35.5065844908757)
--(axis cs:2.2,54.4032713477089);

\path [draw=black, thick]
(axis cs:3.2,38.9411415501858)
--(axis cs:3.2,57.4626155505318);

\path [draw=black, thick]
(axis cs:4.2,40.7758482474665)
--(axis cs:4.2,60.6009428836422);

\path [draw=black, thick]
(axis cs:5.2,47.5342156234599)
--(axis cs:5.2,68.319999324665);

\path [draw=black, thick]
(axis cs:6.2,44.5545223669235)
--(axis cs:6.2,60.5795571761812);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_7_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.74, xmax=6.74,
xtick style={color=black},
xtick={0,1,2,3,4,5,6},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=105.000193187592,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,100);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,99.9998015350877);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,100);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,99.9998015350877);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,99.9998015350877);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,100);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,100);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,100);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,100);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,100);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,100);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,100);
\path [draw=black, thick]
(axis cs:-0.2,100)
--(axis cs:-0.2,100);

\path [draw=black, thick]
(axis cs:0.8,100)
--(axis cs:0.8,100);

\path [draw=black, thick]
(axis cs:1.8,99.999419081993)
--(axis cs:1.8,100.000183988182);

\path [draw=black, thick]
(axis cs:2.8,100)
--(axis cs:2.8,100);

\path [draw=black, thick]
(axis cs:3.8,99.999419081993)
--(axis cs:3.8,100.000183988182);

\path [draw=black, thick]
(axis cs:4.8,99.999419081993)
--(axis cs:4.8,100.000183988182);

\path [draw=black, thick]
(axis cs:5.8,100)
--(axis cs:5.8,100);

\path [draw=black, thick]
(axis cs:0.2,100)
--(axis cs:0.2,100);

\path [draw=black, thick]
(axis cs:1.2,100)
--(axis cs:1.2,100);

\path [draw=black, thick]
(axis cs:2.2,100)
--(axis cs:2.2,100);

\path [draw=black, thick]
(axis cs:3.2,100)
--(axis cs:3.2,100);

\path [draw=black, thick]
(axis cs:4.2,100)
--(axis cs:4.2,100);

\path [draw=black, thick]
(axis cs:5.2,100)
--(axis cs:5.2,100);

\path [draw=black, thick]
(axis cs:6.2,100)
--(axis cs:6.2,100);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_7_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.74, xmax=6.74,
xtick style={color=black},
xtick={0,1,2,3,4,5,6},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=44.1885346699606,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,13.1943555953422);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,11.7718769901422);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,12.4804685425606);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,9.43795591483377);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,11.2296628199396);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,11.8640575961311);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,11.0647100683392);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,31.1176778162969);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,31.1885373920992);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,31.1763420359618);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,29.8590002679543);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,28.2253090674189);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,34.6639341162371);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,35.2570883843797);
\path [draw=black, thick]
(axis cs:-0.2,10.9821350168573)
--(axis cs:-0.2,15.4065761738271);

\path [draw=black, thick]
(axis cs:0.8,9.29487309531963)
--(axis cs:0.8,14.2488808849647);

\path [draw=black, thick]
(axis cs:1.8,10.1227757194379)
--(axis cs:1.8,14.8381613656832);

\path [draw=black, thick]
(axis cs:2.8,7.64854523564077)
--(axis cs:2.8,11.2273665940268);

\path [draw=black, thick]
(axis cs:3.8,8.65003884697946)
--(axis cs:3.8,13.8092867928998);

\path [draw=black, thick]
(axis cs:4.8,9.72615362047107)
--(axis cs:4.8,14.0019615717911);

\path [draw=black, thick]
(axis cs:5.8,8.89231876998623)
--(axis cs:5.8,13.2371013666923);

\path [draw=black, thick]
(axis cs:0.2,24.4917357876912)
--(axis cs:0.2,37.7436198449026);

\path [draw=black, thick]
(axis cs:1.2,26.3690514725807)
--(axis cs:1.2,36.0080233116176);

\path [draw=black, thick]
(axis cs:2.2,25.3224985263528)
--(axis cs:2.2,37.0301855455708);

\path [draw=black, thick]
(axis cs:3.2,24.7381721002698)
--(axis cs:3.2,34.9798284356387);

\path [draw=black, thick]
(axis cs:4.2,22.7164201021679)
--(axis cs:4.2,33.7341980326698);

\path [draw=black, thick]
(axis cs:5.2,27.2435494991783)
--(axis cs:5.2,42.0843187332958);

\path [draw=black, thick]
(axis cs:6.2,30.4397781204548)
--(axis cs:6.2,40.0743986483046);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_7_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.74, xmax=6.74,
xtick style={color=black},
xtick={0,1,2,3,4,5,6},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=105.000386375183,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,100);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,99.9996030701754);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,99.9998015350877);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,99.9998015350877);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,99.9998015350877);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,100);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,99.999048245614);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,99.9998015350877);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,99.9996030701754);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,99.9988497807018);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,99.9990076754386);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,99.9996030701754);
\path [draw=black, thick]
(axis cs:-0.2,100)
--(axis cs:-0.2,100);

\path [draw=black, thick]
(axis cs:0.8,100)
--(axis cs:0.8,100);

\path [draw=black, thick]
(axis cs:1.8,99.9990716069805)
--(axis cs:1.8,100.00013453337);

\path [draw=black, thick]
(axis cs:2.8,99.999419081993)
--(axis cs:2.8,100.000183988182);

\path [draw=black, thick]
(axis cs:3.8,99.999419081993)
--(axis cs:3.8,100.000183988182);

\path [draw=black, thick]
(axis cs:4.8,99.999419081993)
--(axis cs:4.8,100.000183988182);

\path [draw=black, thick]
(axis cs:5.8,100)
--(axis cs:5.8,100);

\path [draw=black, thick]
(axis cs:0.2,100)
--(axis cs:0.2,100);

\path [draw=black, thick]
(axis cs:1.2,99.9979859703487)
--(axis cs:1.2,100.000110520879);

\path [draw=black, thick]
(axis cs:2.2,99.999419081993)
--(axis cs:2.2,100.000183988182);

\path [draw=black, thick]
(axis cs:3.2,99.9990716069805)
--(axis cs:3.2,100.00013453337);

\path [draw=black, thick]
(axis cs:4.2,99.9978886902752)
--(axis cs:4.2,99.9998108711283);

\path [draw=black, thick]
(axis cs:5.2,99.9977673687086)
--(axis cs:5.2,100.000247982169);

\path [draw=black, thick]
(axis cs:6.2,99.998838163986)
--(axis cs:6.2,100.000367976365);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_7_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.74, xmax=6.74,
xtick style={color=black},
xtick={0,1,2,3,4,5,6},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=15.8891824901983,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,12.9081199922876);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,11.9576400843062);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,12.2696308797353);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,9.25236146634637);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,11.0132677173829);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,11.5105602520378);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,10.9847517796865);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,4.65619636710242);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,4.65633738909295);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,4.65637739621377);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,4.65635800212225);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,4.65646043034144);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,4.65641287455876);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,4.65653817341001);
\path [draw=black, thick]
(axis cs:-0.2,10.6836852320053)
--(axis cs:-0.2,15.1325547525698);

\path [draw=black, thick]
(axis cs:0.8,9.52159221865123)
--(axis cs:0.8,14.3936879499612);

\path [draw=black, thick]
(axis cs:1.8,9.86250330336173)
--(axis cs:1.8,14.6767584561089);

\path [draw=black, thick]
(axis cs:2.8,7.49748373254812)
--(axis cs:2.8,11.0072392001446);

\path [draw=black, thick]
(axis cs:3.8,8.40135517132303)
--(axis cs:3.8,13.6251802634428);

\path [draw=black, thick]
(axis cs:4.8,9.44843954768165)
--(axis cs:4.8,13.572680956394);

\path [draw=black, thick]
(axis cs:5.8,8.79724142390751)
--(axis cs:5.8,13.1722621354655);

\path [draw=black, thick]
(axis cs:0.2,4.65585821349294)
--(axis cs:0.2,4.6565345207119);

\path [draw=black, thick]
(axis cs:1.2,4.6560746378298)
--(axis cs:1.2,4.6566001403561);

\path [draw=black, thick]
(axis cs:2.2,4.65607051665902)
--(axis cs:2.2,4.65668427576852);

\path [draw=black, thick]
(axis cs:3.2,4.65601953963183)
--(axis cs:3.2,4.65669646461266);

\path [draw=black, thick]
(axis cs:4.2,4.65609139124273)
--(axis cs:4.2,4.65682946944014);

\path [draw=black, thick]
(axis cs:5.2,4.65603151155407)
--(axis cs:5.2,4.65679423756346);

\path [draw=black, thick]
(axis cs:6.2,4.6562149228027)
--(axis cs:6.2,4.65686142401733);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_7_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.74, xmax=6.74,
xtick style={color=black},
xtick={0,1,2,3,4,5,6},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=105.000193187592,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,100);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,99.9998015350877);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,100);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,99.9998015350877);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,99.9998015350877);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,100);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,100);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,100);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,100);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,100);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,100);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,100);
\path [draw=black, thick]
(axis cs:-0.2,100)
--(axis cs:-0.2,100);

\path [draw=black, thick]
(axis cs:0.8,100)
--(axis cs:0.8,100);

\path [draw=black, thick]
(axis cs:1.8,99.999419081993)
--(axis cs:1.8,100.000183988182);

\path [draw=black, thick]
(axis cs:2.8,100)
--(axis cs:2.8,100);

\path [draw=black, thick]
(axis cs:3.8,99.999419081993)
--(axis cs:3.8,100.000183988182);

\path [draw=black, thick]
(axis cs:4.8,99.999419081993)
--(axis cs:4.8,100.000183988182);

\path [draw=black, thick]
(axis cs:5.8,100)
--(axis cs:5.8,100);

\path [draw=black, thick]
(axis cs:0.2,100)
--(axis cs:0.2,100);

\path [draw=black, thick]
(axis cs:1.2,100)
--(axis cs:1.2,100);

\path [draw=black, thick]
(axis cs:2.2,100)
--(axis cs:2.2,100);

\path [draw=black, thick]
(axis cs:3.2,100)
--(axis cs:3.2,100);

\path [draw=black, thick]
(axis cs:4.2,100)
--(axis cs:4.2,100);

\path [draw=black, thick]
(axis cs:5.2,100)
--(axis cs:5.2,100);

\path [draw=black, thick]
(axis cs:6.2,100)
--(axis cs:6.2,100);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_8_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.79, xmax=7.79,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=71.47751218727,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,12.5243649745759);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,15.6537440930741);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,14.9807961349512);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,12.8186997164944);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,15.8394696120999);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,14.7698362074148);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,13.1333960102206);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,14.5894177487385);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,49.976938841637);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,58.027887621482);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,44.5318753061851);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,55.7351044089536);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,51.7201919513654);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,57.6940919802661);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,58.0081127363785);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,50.46812138104);
\path [draw=black, thick]
(axis cs:-0.2,9.79698986571453)
--(axis cs:-0.2,15.2517400834373);

\path [draw=black, thick]
(axis cs:0.8,12.6399807190523)
--(axis cs:0.8,18.6675074670959);

\path [draw=black, thick]
(axis cs:1.8,12.4934079030305)
--(axis cs:1.8,17.4681843668719);

\path [draw=black, thick]
(axis cs:2.8,9.79061806448106)
--(axis cs:2.8,15.8467813685077);

\path [draw=black, thick]
(axis cs:3.8,12.7451667771796)
--(axis cs:3.8,18.9337724470202);

\path [draw=black, thick]
(axis cs:4.8,11.9838998365548)
--(axis cs:4.8,17.5557725782747);

\path [draw=black, thick]
(axis cs:5.8,10.7719540380122)
--(axis cs:5.8,15.4948379824291);

\path [draw=black, thick]
(axis cs:6.8,11.6065948665376)
--(axis cs:6.8,17.5722406309394);

\path [draw=black, thick]
(axis cs:0.2,40.5705055571223)
--(axis cs:0.2,59.3833721261517);

\path [draw=black, thick]
(axis cs:1.2,48.2596094398034)
--(axis cs:1.2,67.7961658031607);

\path [draw=black, thick]
(axis cs:2.2,34.5056969324753)
--(axis cs:2.2,54.558053679895);

\path [draw=black, thick]
(axis cs:3.2,46.9782847058459)
--(axis cs:3.2,64.4919241120612);

\path [draw=black, thick]
(axis cs:4.2,42.5848492736078)
--(axis cs:4.2,60.8555346291231);

\path [draw=black, thick]
(axis cs:5.2,48.3482582405229)
--(axis cs:5.2,67.0399257200092);

\path [draw=black, thick]
(axis cs:6.2,47.9424043420237)
--(axis cs:6.2,68.0738211307333);

\path [draw=black, thick]
(axis cs:7.2,40.1481691627878)
--(axis cs:7.2,60.7880735992922);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_8_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.79, xmax=7.79,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=105.000579562775,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,99.9994046052632);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,99.9990076754386);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,99.9998015350877);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,99.9998015350877);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,99.9996030701754);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,99.9996030701754);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,99.9998015350877);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,100);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,100);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,100);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,100);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,100);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,100);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,100);
\path [draw=black, thick]
(axis cs:-0.2,100)
--(axis cs:-0.2,100);

\path [draw=black, thick]
(axis cs:0.8,99.998257245979)
--(axis cs:0.8,100.000551964547);

\path [draw=black, thick]
(axis cs:1.8,99.9980417023115)
--(axis cs:1.8,99.9999736485657);

\path [draw=black, thick]
(axis cs:2.8,99.999419081993)
--(axis cs:2.8,100.000183988182);

\path [draw=black, thick]
(axis cs:3.8,99.999419081993)
--(axis cs:3.8,100.000183988182);

\path [draw=black, thick]
(axis cs:4.8,99.9990716069804)
--(axis cs:4.8,100.00013453337);

\path [draw=black, thick]
(axis cs:5.8,99.9990716069805)
--(axis cs:5.8,100.00013453337);

\path [draw=black, thick]
(axis cs:6.8,99.999419081993)
--(axis cs:6.8,100.000183988182);

\path [draw=black, thick]
(axis cs:0.2,100)
--(axis cs:0.2,100);

\path [draw=black, thick]
(axis cs:1.2,100)
--(axis cs:1.2,100);

\path [draw=black, thick]
(axis cs:2.2,100)
--(axis cs:2.2,100);

\path [draw=black, thick]
(axis cs:3.2,100)
--(axis cs:3.2,100);

\path [draw=black, thick]
(axis cs:4.2,100)
--(axis cs:4.2,100);

\path [draw=black, thick]
(axis cs:5.2,100)
--(axis cs:5.2,100);

\path [draw=black, thick]
(axis cs:6.2,100)
--(axis cs:6.2,100);

\path [draw=black, thick]
(axis cs:7.2,100)
--(axis cs:7.2,100);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_8_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.79, xmax=7.79,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=57.0972745825574,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,12.5243649745759);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,15.6537440930741);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,14.9807961349512);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,12.8186997164944);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,15.8394696120999);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,14.7698362074148);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,13.1333960102206);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,14.5894177487385);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,38.3253101587596);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,43.7215032172294);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,36.5233062554489);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,43.5644890249864);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,40.7178002470674);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,42.8509043798852);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,46.1183438331134);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,44.7080925898828);
\path [draw=black, thick]
(axis cs:-0.2,9.79698986571453)
--(axis cs:-0.2,15.2517400834373);

\path [draw=black, thick]
(axis cs:0.8,12.6399807190523)
--(axis cs:0.8,18.6675074670959);

\path [draw=black, thick]
(axis cs:1.8,12.4934079030305)
--(axis cs:1.8,17.4681843668719);

\path [draw=black, thick]
(axis cs:2.8,9.79061806448106)
--(axis cs:2.8,15.8467813685077);

\path [draw=black, thick]
(axis cs:3.8,12.7451667771796)
--(axis cs:3.8,18.9337724470202);

\path [draw=black, thick]
(axis cs:4.8,11.9838998365548)
--(axis cs:4.8,17.5557725782747);

\path [draw=black, thick]
(axis cs:5.8,10.7719540380122)
--(axis cs:5.8,15.4948379824291);

\path [draw=black, thick]
(axis cs:6.8,11.6065948665376)
--(axis cs:6.8,17.5722406309394);

\path [draw=black, thick]
(axis cs:0.2,31.0574960286685)
--(axis cs:0.2,45.5931242888507);

\path [draw=black, thick]
(axis cs:1.2,35.198812758713)
--(axis cs:1.2,52.2441936757458);

\path [draw=black, thick]
(axis cs:2.2,29.2061653745852)
--(axis cs:2.2,43.8404471363126);

\path [draw=black, thick]
(axis cs:3.2,37.2534345757859)
--(axis cs:3.2,49.8755434741869);

\path [draw=black, thick]
(axis cs:4.2,32.6855669539876)
--(axis cs:4.2,48.7500335401472);

\path [draw=black, thick]
(axis cs:5.2,35.5220824207008)
--(axis cs:5.2,50.1797263390695);

\path [draw=black, thick]
(axis cs:6.2,37.858330920934)
--(axis cs:6.2,54.3783567452927);

\path [draw=black, thick]
(axis cs:7.2,37.1862403964476)
--(axis cs:7.2,52.229944783318);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_8_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.79, xmax=7.79,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=105.000579562775,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,99.9994046052632);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,99.9990076754386);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,99.9998015350877);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,99.9998015350877);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,99.9996030701754);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,99.9996030701754);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,99.9998015350877);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,99.9998015350877);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,99.9996030701754);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,100);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,100);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,99.9996030701754);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,99.9998015350877);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,99.9998015350877);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,99.9994046052632);
\path [draw=black, thick]
(axis cs:-0.2,100)
--(axis cs:-0.2,100);

\path [draw=black, thick]
(axis cs:0.8,99.998257245979)
--(axis cs:0.8,100.000551964547);

\path [draw=black, thick]
(axis cs:1.8,99.9980417023115)
--(axis cs:1.8,99.9999736485657);

\path [draw=black, thick]
(axis cs:2.8,99.999419081993)
--(axis cs:2.8,100.000183988182);

\path [draw=black, thick]
(axis cs:3.8,99.999419081993)
--(axis cs:3.8,100.000183988182);

\path [draw=black, thick]
(axis cs:4.8,99.9990716069805)
--(axis cs:4.8,100.00013453337);

\path [draw=black, thick]
(axis cs:5.8,99.9990716069805)
--(axis cs:5.8,100.00013453337);

\path [draw=black, thick]
(axis cs:6.8,99.999419081993)
--(axis cs:6.8,100.000183988182);

\path [draw=black, thick]
(axis cs:0.2,99.999419081993)
--(axis cs:0.2,100.000183988182);

\path [draw=black, thick]
(axis cs:1.2,99.9990716069804)
--(axis cs:1.2,100.00013453337);

\path [draw=black, thick]
(axis cs:2.2,100)
--(axis cs:2.2,100);

\path [draw=black, thick]
(axis cs:3.2,100)
--(axis cs:3.2,100);

\path [draw=black, thick]
(axis cs:4.2,99.998838163986)
--(axis cs:4.2,100.000367976365);

\path [draw=black, thick]
(axis cs:5.2,99.999419081993)
--(axis cs:5.2,100.000183988182);

\path [draw=black, thick]
(axis cs:6.2,99.999419081993)
--(axis cs:6.2,100.000183988182);

\path [draw=black, thick]
(axis cs:7.2,99.9987654274523)
--(axis cs:7.2,100.000043783074);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_8_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.79, xmax=7.79,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=19.8804610693712,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,12.5243649745759);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,15.6537440930741);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,14.9807961349512);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,12.8186997164944);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,15.8394696120999);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,14.7698362074148);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,13.1333960102206);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,14.5894177487385);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,4.65649869613348);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,4.65643935008436);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,4.65657011791457);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,4.65629491591417);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,4.65668843140273);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,4.65630344950312);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,4.65667780351779);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,4.65627337265607);
\path [draw=black, thick]
(axis cs:-0.2,9.79698986571452)
--(axis cs:-0.2,15.2517400834373);

\path [draw=black, thick]
(axis cs:0.8,12.6399807190523)
--(axis cs:0.8,18.6675074670959);

\path [draw=black, thick]
(axis cs:1.8,12.4934079030305)
--(axis cs:1.8,17.4681843668719);

\path [draw=black, thick]
(axis cs:2.8,9.79061806448107)
--(axis cs:2.8,15.8467813685077);

\path [draw=black, thick]
(axis cs:3.8,12.7451667771796)
--(axis cs:3.8,18.9337724470202);

\path [draw=black, thick]
(axis cs:4.8,11.9838998365548)
--(axis cs:4.8,17.5557725782747);

\path [draw=black, thick]
(axis cs:5.8,10.7719540380122)
--(axis cs:5.8,15.4948379824291);

\path [draw=black, thick]
(axis cs:6.8,11.6065948665376)
--(axis cs:6.8,17.5722406309394);

\path [draw=black, thick]
(axis cs:0.2,4.65610878115212)
--(axis cs:0.2,4.65688861111484);

\path [draw=black, thick]
(axis cs:1.2,4.65608828961195)
--(axis cs:1.2,4.65679041055677);

\path [draw=black, thick]
(axis cs:2.2,4.65622470197477)
--(axis cs:2.2,4.65691553385437);

\path [draw=black, thick]
(axis cs:3.2,4.65600032028249)
--(axis cs:3.2,4.65658951154585);

\path [draw=black, thick]
(axis cs:4.2,4.6562144867158)
--(axis cs:4.2,4.65716237608966);

\path [draw=black, thick]
(axis cs:5.2,4.6560592913274)
--(axis cs:5.2,4.65654760767885);

\path [draw=black, thick]
(axis cs:6.2,4.65637445083288)
--(axis cs:6.2,4.6569811562027);

\path [draw=black, thick]
(axis cs:7.2,4.65597031374491)
--(axis cs:7.2,4.65657643156722);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_8_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.79, xmax=7.79,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=105.000579562775,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,99.9994046052632);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,99.9990076754386);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,99.9998015350877);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,99.9998015350877);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,99.9996030701754);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,99.9996030701754);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,99.9998015350877);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,100);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,100);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,100);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,100);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,100);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,100);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,100);
\path [draw=black, thick]
(axis cs:-0.2,100)
--(axis cs:-0.2,100);

\path [draw=black, thick]
(axis cs:0.8,99.998257245979)
--(axis cs:0.8,100.000551964547);

\path [draw=black, thick]
(axis cs:1.8,99.9980417023115)
--(axis cs:1.8,99.9999736485657);

\path [draw=black, thick]
(axis cs:2.8,99.999419081993)
--(axis cs:2.8,100.000183988182);

\path [draw=black, thick]
(axis cs:3.8,99.999419081993)
--(axis cs:3.8,100.000183988182);

\path [draw=black, thick]
(axis cs:4.8,99.9990716069804)
--(axis cs:4.8,100.00013453337);

\path [draw=black, thick]
(axis cs:5.8,99.9990716069804)
--(axis cs:5.8,100.00013453337);

\path [draw=black, thick]
(axis cs:6.8,99.999419081993)
--(axis cs:6.8,100.000183988182);

\path [draw=black, thick]
(axis cs:0.2,100)
--(axis cs:0.2,100);

\path [draw=black, thick]
(axis cs:1.2,100)
--(axis cs:1.2,100);

\path [draw=black, thick]
(axis cs:2.2,100)
--(axis cs:2.2,100);

\path [draw=black, thick]
(axis cs:3.2,100)
--(axis cs:3.2,100);

\path [draw=black, thick]
(axis cs:4.2,100)
--(axis cs:4.2,100);

\path [draw=black, thick]
(axis cs:5.2,100)
--(axis cs:5.2,100);

\path [draw=black, thick]
(axis cs:6.2,100)
--(axis cs:6.2,100);

\path [draw=black, thick]
(axis cs:7.2,100)
--(axis cs:7.2,100);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_9_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.84, xmax=8.84,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=70.6821201505168,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,44.7890344476867);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,41.0581621032978);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,42.8806155046843);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,42.8073786417772);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,43.128376216986);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,43.5587410141043);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,40.8439948738825);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,45.1819988487461);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,42.0231631486039);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,44.9134981216289);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,58.0316396532508);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,44.1960256768578);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,46.3395508152704);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,55.0894525146127);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,52.1808221863735);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,50.6392024727514);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,59.4901201056432);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,44.460674212962);
\path [draw=black, thick]
(axis cs:-0.2,31.5655682696016)
--(axis cs:-0.2,58.0125006257717);

\path [draw=black, thick]
(axis cs:0.8,28.265113691027)
--(axis cs:0.8,53.8512105155685);

\path [draw=black, thick]
(axis cs:1.8,30.3959028256661)
--(axis cs:1.8,55.3653281837025);

\path [draw=black, thick]
(axis cs:2.8,31.0727919435485)
--(axis cs:2.8,54.5419653400059);

\path [draw=black, thick]
(axis cs:3.8,31.3620490912515)
--(axis cs:3.8,54.8947033427205);

\path [draw=black, thick]
(axis cs:4.8,30.045266373914)
--(axis cs:4.8,57.0722156542947);

\path [draw=black, thick]
(axis cs:5.8,28.7715798215633)
--(axis cs:5.8,52.9164099262016);

\path [draw=black, thick]
(axis cs:6.8,31.751937976464)
--(axis cs:6.8,58.6120597210283);

\path [draw=black, thick]
(axis cs:7.8,29.74810831126)
--(axis cs:7.8,54.2982179859479);

\path [draw=black, thick]
(axis cs:0.2,34.4467788996935)
--(axis cs:0.2,55.3802173435643);

\path [draw=black, thick]
(axis cs:1.2,49.606401875512)
--(axis cs:1.2,66.4568774309896);

\path [draw=black, thick]
(axis cs:2.2,33.622571015038)
--(axis cs:2.2,54.7694803386775);

\path [draw=black, thick]
(axis cs:3.2,35.8785325890786)
--(axis cs:3.2,56.8005690414623);

\path [draw=black, thick]
(axis cs:4.2,44.7411903018525)
--(axis cs:4.2,65.4377147273729);

\path [draw=black, thick]
(axis cs:5.2,43.3285181056645)
--(axis cs:5.2,61.0331262670825);

\path [draw=black, thick]
(axis cs:6.2,41.6796048766148)
--(axis cs:6.2,59.598800068888);

\path [draw=black, thick]
(axis cs:7.2,51.6639353060323)
--(axis cs:7.2,67.3163049052541);

\path [draw=black, thick]
(axis cs:8.2,33.9669294937625)
--(axis cs:8.2,54.9544189321614);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_9_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.84, xmax=8.84,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=105,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,99.073084868421);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,98.8935605263158);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,98.5469666666667);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,97.9667530701754);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,99.1328951754386);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,98.3745879385965);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,99.1742543859649);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,99.2485967105263);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,99.1229754385965);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,100);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,100);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,100);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,100);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,100);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,100);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,100);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,100);
\path [draw=black, thick]
(axis cs:-0.2,98.5318295820157)
--(axis cs:-0.2,99.6143401548264);

\path [draw=black, thick]
(axis cs:0.8,98.111888939429)
--(axis cs:0.8,99.6752321132025);

\path [draw=black, thick]
(axis cs:1.8,97.4247536432332)
--(axis cs:1.8,99.6691796901002);

\path [draw=black, thick]
(axis cs:2.8,96.9288099339216)
--(axis cs:2.8,99.0046962064293);

\path [draw=black, thick]
(axis cs:3.8,98.4209994173156)
--(axis cs:3.8,99.8447909335616);

\path [draw=black, thick]
(axis cs:4.8,97.3045460454562)
--(axis cs:4.8,99.4446298317368);

\path [draw=black, thick]
(axis cs:5.8,98.6422272797135)
--(axis cs:5.8,99.7062814922163);

\path [draw=black, thick]
(axis cs:6.8,98.6407688307033)
--(axis cs:6.8,99.8564245903493);

\path [draw=black, thick]
(axis cs:7.8,98.4060420675402)
--(axis cs:7.8,99.8399088096528);

\path [draw=black, thick]
(axis cs:0.2,100)
--(axis cs:0.2,100);

\path [draw=black, thick]
(axis cs:1.2,100)
--(axis cs:1.2,100);

\path [draw=black, thick]
(axis cs:2.2,100)
--(axis cs:2.2,100);

\path [draw=black, thick]
(axis cs:3.2,100)
--(axis cs:3.2,100);

\path [draw=black, thick]
(axis cs:4.2,100)
--(axis cs:4.2,100);

\path [draw=black, thick]
(axis cs:5.2,100)
--(axis cs:5.2,100);

\path [draw=black, thick]
(axis cs:6.2,100)
--(axis cs:6.2,100);

\path [draw=black, thick]
(axis cs:7.2,100)
--(axis cs:7.2,100);

\path [draw=black, thick]
(axis cs:8.2,100)
--(axis cs:8.2,100);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_9_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.84, xmax=8.84,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=66.8751281703979,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,44.7890344476867);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,41.0581621032978);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,42.8806155046843);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,42.8073786417772);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,43.128376216986);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,43.5587410141043);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,40.8439948738825);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,45.1819988487461);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,42.0231631486039);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,41.6686563790108);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,55.7096454860151);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,39.1525987419059);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,nan);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,49.6927427071468);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,41.678121858481);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,51.6583743842359);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,48.4322718100665);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,48.4781754745403);
\path [draw=black, thick]
(axis cs:-0.2,31.5655682696016)
--(axis cs:-0.2,58.0125006257717);

\path [draw=black, thick]
(axis cs:0.8,28.265113691027)
--(axis cs:0.8,53.8512105155686);

\path [draw=black, thick]
(axis cs:1.8,30.3959028256661)
--(axis cs:1.8,55.3653281837025);

\path [draw=black, thick]
(axis cs:2.8,31.0727919435485)
--(axis cs:2.8,54.5419653400058);

\path [draw=black, thick]
(axis cs:3.8,31.3620490912515)
--(axis cs:3.8,54.8947033427205);

\path [draw=black, thick]
(axis cs:4.8,30.045266373914)
--(axis cs:4.8,57.0722156542947);

\path [draw=black, thick]
(axis cs:5.8,28.7715798215633)
--(axis cs:5.8,52.9164099262016);

\path [draw=black, thick]
(axis cs:6.8,31.7519379764639)
--(axis cs:6.8,58.6120597210282);

\path [draw=black, thick]
(axis cs:7.8,29.74810831126)
--(axis cs:7.8,54.2982179859479);

\path [draw=black, thick]
(axis cs:0.2,32.5934967128586)
--(axis cs:0.2,50.7438160451631);

\path [draw=black, thick]
(axis cs:1.2,47.7286927145084)
--(axis cs:1.2,63.6905982575218);

\path [draw=black, thick]
(axis cs:2.2,30.1118288244141)
--(axis cs:2.2,48.1933686593977);

\path [draw=black, thick]
(axis cs:4.2,40.0379565360579)
--(axis cs:4.2,59.3475288782356);

\path [draw=black, thick]
(axis cs:5.2,33.7196128408476)
--(axis cs:5.2,49.6366308761145);

\path [draw=black, thick]
(axis cs:6.2,43.3224615616113)
--(axis cs:6.2,59.9942872068605);

\path [draw=black, thick]
(axis cs:7.2,40.4327267964589)
--(axis cs:7.2,56.4318168236741);

\path [draw=black, thick]
(axis cs:8.2,39.1154157113922)
--(axis cs:8.2,57.8409352376884);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_9_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.84, xmax=8.84,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=108.243808770771,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,99.073084868421);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,98.8935605263158);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,98.5469666666667);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,97.9667530701755);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,99.1328951754386);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,98.3745879385965);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,99.1742543859649);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,99.2485967105263);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,99.1229754385965);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,99.9674550438596);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,100);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,99.9994046052632);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,96.6658728070175);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,100);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,99.9994046052632);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,99.9998015350877);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,100);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,99.9676535087719);
\path [draw=black, thick]
(axis cs:-0.2,98.5318295820157)
--(axis cs:-0.2,99.6143401548264);

\path [draw=black, thick]
(axis cs:0.8,98.111888939429)
--(axis cs:0.8,99.6752321132026);

\path [draw=black, thick]
(axis cs:1.8,97.4247536432332)
--(axis cs:1.8,99.6691796901002);

\path [draw=black, thick]
(axis cs:2.8,96.9288099339216)
--(axis cs:2.8,99.0046962064293);

\path [draw=black, thick]
(axis cs:3.8,98.4209994173156)
--(axis cs:3.8,99.8447909335616);

\path [draw=black, thick]
(axis cs:4.8,97.3045460454562)
--(axis cs:4.8,99.4446298317368);

\path [draw=black, thick]
(axis cs:5.8,98.6422272797135)
--(axis cs:5.8,99.7062814922163);

\path [draw=black, thick]
(axis cs:6.8,98.6407688307033)
--(axis cs:6.8,99.8564245903493);

\path [draw=black, thick]
(axis cs:7.8,98.4060420675402)
--(axis cs:7.8,99.8399088096528);

\path [draw=black, thick]
(axis cs:0.2,99.9051335443286)
--(axis cs:0.2,100.029776543391);

\path [draw=black, thick]
(axis cs:1.2,100)
--(axis cs:1.2,100);

\path [draw=black, thick]
(axis cs:2.2,99.9987654274523)
--(axis cs:2.2,100.000043783074);

\path [draw=black, thick]
(axis cs:3.2,90.2424039275862)
--(axis cs:3.2,103.089341686449);

\path [draw=black, thick]
(axis cs:4.2,100)
--(axis cs:4.2,100);

\path [draw=black, thick]
(axis cs:5.2,99.998257245979)
--(axis cs:5.2,100.000551964547);

\path [draw=black, thick]
(axis cs:6.2,99.999419081993)
--(axis cs:6.2,100.000183988182);

\path [draw=black, thick]
(axis cs:7.2,100)
--(axis cs:7.2,100);

\path [draw=black, thick]
(axis cs:8.2,99.9053199933333)
--(axis cs:8.2,100.029987024211);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_9_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.84, xmax=8.84,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=61.5426627070797,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,44.7890344476867);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,41.0581621032978);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,42.8806155046843);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,42.8073786417772);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,43.128376216986);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,43.5587410141043);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,40.8439948738825);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,45.1819988487461);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,42.0231631486039);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,4.65640519569973);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,4.65657752549539);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,4.65649248210137);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,4.65636107851532);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,4.65631685343743);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,4.65659410507375);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,4.65639719264715);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,4.65646190571931);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,4.6562900990344);
\path [draw=black, thick]
(axis cs:-0.2,31.5655682696016)
--(axis cs:-0.2,58.0125006257717);

\path [draw=black, thick]
(axis cs:0.8,28.265113691027)
--(axis cs:0.8,53.8512105155685);

\path [draw=black, thick]
(axis cs:1.8,30.3959028256661)
--(axis cs:1.8,55.3653281837025);

\path [draw=black, thick]
(axis cs:2.8,31.0727919435485)
--(axis cs:2.8,54.5419653400059);

\path [draw=black, thick]
(axis cs:3.8,31.3620490912515)
--(axis cs:3.8,54.8947033427205);

\path [draw=black, thick]
(axis cs:4.8,30.045266373914)
--(axis cs:4.8,57.0722156542947);

\path [draw=black, thick]
(axis cs:5.8,28.7715798215633)
--(axis cs:5.8,52.9164099262016);

\path [draw=black, thick]
(axis cs:6.8,31.751937976464)
--(axis cs:6.8,58.6120597210283);

\path [draw=black, thick]
(axis cs:7.8,29.74810831126)
--(axis cs:7.8,54.2982179859478);

\path [draw=black, thick]
(axis cs:0.2,4.65593825150918)
--(axis cs:0.2,4.65687213989028);

\path [draw=black, thick]
(axis cs:1.2,4.65612987323851)
--(axis cs:1.2,4.65702517775228);

\path [draw=black, thick]
(axis cs:2.2,4.65617241670396)
--(axis cs:2.2,4.65681254749879);

\path [draw=black, thick]
(axis cs:3.2,4.65595081380881)
--(axis cs:3.2,4.65677134322184);

\path [draw=black, thick]
(axis cs:4.2,4.65606370264101)
--(axis cs:4.2,4.65657000423385);

\path [draw=black, thick]
(axis cs:5.2,4.6562555875773)
--(axis cs:5.2,4.6569326225702);

\path [draw=black, thick]
(axis cs:6.2,4.65608386318749)
--(axis cs:6.2,4.65671052210681);

\path [draw=black, thick]
(axis cs:7.2,4.65612512667987)
--(axis cs:7.2,4.65679868475874);

\path [draw=black, thick]
(axis cs:8.2,4.65591547282829)
--(axis cs:8.2,4.65666472524051);

\end{axis}

\end{tikzpicture}


==> img/100Mbps/numStas_9_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.84, xmax=8.84,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=105,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,99.0730848684211);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,98.8935605263158);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,98.5469666666667);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,97.9667530701754);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,99.1328951754386);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,98.3745879385965);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,99.1742543859649);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,99.2485967105263);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,99.1229754385965);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,100);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,100);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,100);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,100);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,100);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,100);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,100);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,100);
\path [draw=black, thick]
(axis cs:-0.2,98.5318295820157)
--(axis cs:-0.2,99.6143401548264);

\path [draw=black, thick]
(axis cs:0.8,98.111888939429)
--(axis cs:0.8,99.6752321132026);

\path [draw=black, thick]
(axis cs:1.8,97.4247536432332)
--(axis cs:1.8,99.6691796901002);

\path [draw=black, thick]
(axis cs:2.8,96.9288099339216)
--(axis cs:2.8,99.0046962064293);

\path [draw=black, thick]
(axis cs:3.8,98.4209994173156)
--(axis cs:3.8,99.8447909335616);

\path [draw=black, thick]
(axis cs:4.8,97.3045460454562)
--(axis cs:4.8,99.4446298317368);

\path [draw=black, thick]
(axis cs:5.8,98.6422272797135)
--(axis cs:5.8,99.7062814922163);

\path [draw=black, thick]
(axis cs:6.8,98.6407688307033)
--(axis cs:6.8,99.8564245903493);

\path [draw=black, thick]
(axis cs:7.8,98.4060420675402)
--(axis cs:7.8,99.8399088096528);

\path [draw=black, thick]
(axis cs:0.2,100)
--(axis cs:0.2,100);

\path [draw=black, thick]
(axis cs:1.2,100)
--(axis cs:1.2,100);

\path [draw=black, thick]
(axis cs:2.2,100)
--(axis cs:2.2,100);

\path [draw=black, thick]
(axis cs:3.2,100)
--(axis cs:3.2,100);

\path [draw=black, thick]
(axis cs:4.2,100)
--(axis cs:4.2,100);

\path [draw=black, thick]
(axis cs:5.2,100)
--(axis cs:5.2,100);

\path [draw=black, thick]
(axis cs:6.2,100)
--(axis cs:6.2,100);

\path [draw=black, thick]
(axis cs:7.2,100)
--(axis cs:7.2,100);

\path [draw=black, thick]
(axis cs:8.2,100)
--(axis cs:8.2,100);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_10_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.87, xmax=9.47,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9,STA 10},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=455.688841597977,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,421.063407110915);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,422.494417830849);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,414.26580568154);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,419.951825070117);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,416.12182476649);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,422.406998779714);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,417.253715237922);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,422.496957745437);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,416.548644016064);
\draw[draw=none,fill=color0] (axis cs:8.6,0) rectangle (axis cs:9,425.954929266011);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,nan);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,nan);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,nan);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,nan);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,nan);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,nan);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,nan);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,nan);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,nan);
\draw[draw=none,fill=color1] (axis cs:9,0) rectangle (axis cs:9.4,nan);
\path [draw=black, thick]
(axis cs:-0.2,408.137441271376)
--(axis cs:-0.2,433.989372950454);

\path [draw=black, thick]
(axis cs:0.8,417.717205182492)
--(axis cs:0.8,427.271630479207);

\path [draw=black, thick]
(axis cs:1.8,404.590732478915)
--(axis cs:1.8,423.940878884166);

\path [draw=black, thick]
(axis cs:2.8,411.313079808991)
--(axis cs:2.8,428.590570331242);

\path [draw=black, thick]
(axis cs:3.8,409.413329739598)
--(axis cs:3.8,422.830319793382);

\path [draw=black, thick]
(axis cs:4.8,416.041952165528)
--(axis cs:4.8,428.772045393901);

\path [draw=black, thick]
(axis cs:5.8,409.699242467147)
--(axis cs:5.8,424.808188008698);

\path [draw=black, thick]
(axis cs:6.8,413.855036822407)
--(axis cs:6.8,431.138878668467);

\path [draw=black, thick]
(axis cs:7.8,408.576799956969)
--(axis cs:7.8,424.520488075158);

\path [draw=black, thick]
(axis cs:8.8,420.484128112153)
--(axis cs:8.8,431.425730419869);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_10_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.89, xmax=9.89,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9,STA 10},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=216.489395341032,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,79.726098245614);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,86.6512002192982);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,87.4149276315789);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,88.3577164473684);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,84.4686822368421);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,81.632025);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,83.5959456140351);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,77.5601129385965);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,82.2502864035088);
\draw[draw=none,fill=color0] (axis cs:8.6,0) rectangle (axis cs:9,81.6705138157895);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,153.333333333333);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,180);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,193.333333333333);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,73.3333333333333);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,106.666666666667);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,33.3333333333333);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,80);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,93.3333333333333);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,40);
\draw[draw=none,fill=color1] (axis cs:9,0) rectangle (axis cs:9.4,46.6666666666667);
\path [draw=black, thick]
(axis cs:-0.2,71.9937459090918)
--(axis cs:-0.2,87.4584505821363);

\path [draw=black, thick]
(axis cs:0.8,79.3208584047666)
--(axis cs:0.8,93.9815420338299);

\path [draw=black, thick]
(axis cs:1.8,80.4631144371284)
--(axis cs:1.8,94.3667408260295);

\path [draw=black, thick]
(axis cs:2.8,82.8073812445812)
--(axis cs:2.8,93.9080516501557);

\path [draw=black, thick]
(axis cs:3.8,78.181378412945)
--(axis cs:3.8,90.7559860607392);

\path [draw=black, thick]
(axis cs:4.8,75.3740167024051)
--(axis cs:4.8,87.8900332975949);

\path [draw=black, thick]
(axis cs:5.8,76.5950870652297)
--(axis cs:5.8,90.5968041628405);

\path [draw=black, thick]
(axis cs:6.8,71.3954844762114)
--(axis cs:6.8,83.7247414009816);

\path [draw=black, thick]
(axis cs:7.8,75.7390178777756)
--(axis cs:7.8,88.761554929242);

\path [draw=black, thick]
(axis cs:8.8,75.2084783194045)
--(axis cs:8.8,88.1325493121744);

\path [draw=black, thick]
(axis cs:0.2,123.06300560566)
--(axis cs:0.2,183.603661061007);

\path [draw=black, thick]
(axis cs:1.2,158.529275745797)
--(axis cs:1.2,201.470724254203);

\path [draw=black, thick]
(axis cs:2.2,180.486290151398)
--(axis cs:2.2,206.180376515269);

\path [draw=black, thick]
(axis cs:3.2,38.8445933565643)
--(axis cs:3.2,107.822073310102);

\path [draw=black, thick]
(axis cs:4.2,70.961735997723)
--(axis cs:4.2,142.37159733561);

\path [draw=black, thick]
(axis cs:5.2,6.66111168969428)
--(axis cs:5.2,60.0055549769724);

\path [draw=black, thick]
(axis cs:6.2,44.9384541128033)
--(axis cs:6.2,115.061545887197);

\path [draw=black, thick]
(axis cs:7.2,57.6284026643897)
--(axis cs:7.2,129.038264002277);

\path [draw=black, thick]
(axis cs:8.2,11.3723676610633)
--(axis cs:8.2,68.6276323389367);

\path [draw=black, thick]
(axis cs:9.2,16.3963389389935)
--(axis cs:9.2,76.9369943943399);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_10_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.87, xmax=9.47,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9,STA 10},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=456.221971905932,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,421.538648925347);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,422.018753369816);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,414.380028609175);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,419.847587659287);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,415.999638535182);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,424.504563339294);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,417.652167695686);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,421.936271544343);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,416.503497130686);
\draw[draw=none,fill=color0] (axis cs:8.6,0) rectangle (axis cs:9,424.358455296054);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,nan);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,nan);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,nan);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,nan);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,nan);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,nan);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,nan);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,nan);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,nan);
\draw[draw=none,fill=color1] (axis cs:9,0) rectangle (axis cs:9.4,nan);
\path [draw=black, thick]
(axis cs:-0.2,408.580181749807)
--(axis cs:-0.2,434.497116100888);

\path [draw=black, thick]
(axis cs:0.8,417.216858599044)
--(axis cs:0.8,426.820648140588);

\path [draw=black, thick]
(axis cs:1.8,404.685104818747)
--(axis cs:1.8,424.074952399602);

\path [draw=black, thick]
(axis cs:2.8,411.196423780524)
--(axis cs:2.8,428.498751538049);

\path [draw=black, thick]
(axis cs:3.8,409.288276548112)
--(axis cs:3.8,422.711000522253);

\path [draw=black, thick]
(axis cs:4.8,418.476253045669)
--(axis cs:4.8,430.532873632918);

\path [draw=black, thick]
(axis cs:5.8,409.986751832382)
--(axis cs:5.8,425.31758355899);

\path [draw=black, thick]
(axis cs:6.8,413.447376643268)
--(axis cs:6.8,430.425166445418);

\path [draw=black, thick]
(axis cs:7.8,408.556018632515)
--(axis cs:7.8,424.450975628856);

\path [draw=black, thick]
(axis cs:8.8,418.639394002642)
--(axis cs:8.8,430.077516589466);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_10_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.89, xmax=9.89,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9,STA 10},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=214.744860287459,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,81.1520078947368);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,85.937209868421);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,88.3727899122807);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,87.800435745614);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,83.4851765350877);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,81.1548896929824);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,83.1905734649123);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,79.2633434210526);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,82.4380377192983);
\draw[draw=none,fill=color0] (axis cs:8.6,0) rectangle (axis cs:9,80.9391379385965);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,153.333333333333);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,180);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,186.666468201754);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,66.2132660087719);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,113.333333333333);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,33.3333333333333);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,80);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,86.6666666666667);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,33.3333333333333);
\draw[draw=none,fill=color1] (axis cs:9,0) rectangle (axis cs:9.4,46.6666666666667);
\path [draw=black, thick]
(axis cs:-0.2,73.3928405680358)
--(axis cs:-0.2,88.9111752214379);

\path [draw=black, thick]
(axis cs:0.8,78.4422425070555)
--(axis cs:0.8,93.4321772297866);

\path [draw=black, thick]
(axis cs:1.8,81.4271768666591)
--(axis cs:1.8,95.3184029579024);

\path [draw=black, thick]
(axis cs:2.8,82.3641110413912)
--(axis cs:2.8,93.2367604498369);

\path [draw=black, thick]
(axis cs:3.8,77.4198071771235)
--(axis cs:3.8,89.550545893052);

\path [draw=black, thick]
(axis cs:4.8,74.9539021279164)
--(axis cs:4.8,87.3558772580485);

\path [draw=black, thick]
(axis cs:5.8,76.1117524365608)
--(axis cs:5.8,90.2693944932638);

\path [draw=black, thick]
(axis cs:6.8,72.763290968514)
--(axis cs:6.8,85.7633958735913);

\path [draw=black, thick]
(axis cs:7.8,75.9721687096311)
--(axis cs:7.8,88.9039067289654);

\path [draw=black, thick]
(axis cs:8.8,74.3591028641202)
--(axis cs:8.8,87.5191730130728);

\path [draw=black, thick]
(axis cs:0.2,123.06300560566)
--(axis cs:0.2,183.603661061007);

\path [draw=black, thick]
(axis cs:1.2,158.529275745797)
--(axis cs:1.2,201.470724254203);

\path [draw=black, thick]
(axis cs:2.2,168.814021844024)
--(axis cs:2.2,204.518914559484);

\path [draw=black, thick]
(axis cs:3.2,32.6941262600509)
--(axis cs:3.2,99.732405757493);

\path [draw=black, thick]
(axis cs:4.2,77.8683041313674)
--(axis cs:4.2,148.798362535299);

\path [draw=black, thick]
(axis cs:5.2,6.66111168969428)
--(axis cs:5.2,60.0055549769724);

\path [draw=black, thick]
(axis cs:6.2,44.9384541128033)
--(axis cs:6.2,115.061545887197);

\path [draw=black, thick]
(axis cs:7.2,51.2016374647007)
--(axis cs:7.2,122.131695868633);

\path [draw=black, thick]
(axis cs:8.2,6.66111168969428)
--(axis cs:8.2,60.0055549769724);

\path [draw=black, thick]
(axis cs:9.2,16.3963389389935)
--(axis cs:9.2,76.9369943943399);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_10_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.87, xmax=9.47,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9,STA 10},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=456.221971905932,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,421.538648925347);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,422.018753369816);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,414.380028609175);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,419.847587659287);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,415.999638535182);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,424.504563339294);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,417.652167695686);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,421.936271544343);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,416.503497130686);
\draw[draw=none,fill=color0] (axis cs:8.6,0) rectangle (axis cs:9,424.358455296054);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,nan);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,nan);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,nan);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,nan);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,nan);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,nan);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,nan);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,nan);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,nan);
\draw[draw=none,fill=color1] (axis cs:9,0) rectangle (axis cs:9.4,nan);
\path [draw=black, thick]
(axis cs:-0.2,408.580181749807)
--(axis cs:-0.2,434.497116100888);

\path [draw=black, thick]
(axis cs:0.8,417.216858599044)
--(axis cs:0.8,426.820648140588);

\path [draw=black, thick]
(axis cs:1.8,404.685104818747)
--(axis cs:1.8,424.074952399602);

\path [draw=black, thick]
(axis cs:2.8,411.196423780524)
--(axis cs:2.8,428.498751538049);

\path [draw=black, thick]
(axis cs:3.8,409.288276548112)
--(axis cs:3.8,422.711000522253);

\path [draw=black, thick]
(axis cs:4.8,418.476253045669)
--(axis cs:4.8,430.532873632918);

\path [draw=black, thick]
(axis cs:5.8,409.986751832382)
--(axis cs:5.8,425.31758355899);

\path [draw=black, thick]
(axis cs:6.8,413.447376643268)
--(axis cs:6.8,430.425166445418);

\path [draw=black, thick]
(axis cs:7.8,408.556018632515)
--(axis cs:7.8,424.450975628856);

\path [draw=black, thick]
(axis cs:8.8,418.639394002642)
--(axis cs:8.8,430.077516589466);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_10_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.89, xmax=9.89,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9,STA 10},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=216.489395341032,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,81.1520078947369);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,85.9372098684211);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,88.3727899122807);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,87.800435745614);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,83.4851765350877);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,81.1548896929825);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,83.1905734649123);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,79.2633434210527);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,82.4380377192983);
\draw[draw=none,fill=color0] (axis cs:8.6,0) rectangle (axis cs:9,80.9391379385965);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,153.333333333333);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,180);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,193.333333333333);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,80);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,106.666666666667);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,33.3333333333333);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,80);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,93.3333333333333);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,33.3333333333333);
\draw[draw=none,fill=color1] (axis cs:9,0) rectangle (axis cs:9.4,46.6666666666667);
\path [draw=black, thick]
(axis cs:-0.2,73.3928405680358)
--(axis cs:-0.2,88.9111752214379);

\path [draw=black, thick]
(axis cs:0.8,78.4422425070555)
--(axis cs:0.8,93.4321772297867);

\path [draw=black, thick]
(axis cs:1.8,81.4271768666591)
--(axis cs:1.8,95.3184029579024);

\path [draw=black, thick]
(axis cs:2.8,82.3641110413911)
--(axis cs:2.8,93.2367604498369);

\path [draw=black, thick]
(axis cs:3.8,77.4198071771235)
--(axis cs:3.8,89.5505458930519);

\path [draw=black, thick]
(axis cs:4.8,74.9539021279164)
--(axis cs:4.8,87.3558772580485);

\path [draw=black, thick]
(axis cs:5.8,76.1117524365608)
--(axis cs:5.8,90.2693944932638);

\path [draw=black, thick]
(axis cs:6.8,72.763290968514)
--(axis cs:6.8,85.7633958735913);

\path [draw=black, thick]
(axis cs:7.8,75.9721687096311)
--(axis cs:7.8,88.9039067289654);

\path [draw=black, thick]
(axis cs:8.8,74.3591028641202)
--(axis cs:8.8,87.5191730130728);

\path [draw=black, thick]
(axis cs:0.2,123.06300560566)
--(axis cs:0.2,183.603661061007);

\path [draw=black, thick]
(axis cs:1.2,158.529275745797)
--(axis cs:1.2,201.470724254203);

\path [draw=black, thick]
(axis cs:2.2,180.486290151398)
--(axis cs:2.2,206.180376515269);

\path [draw=black, thick]
(axis cs:3.2,44.9384541128033)
--(axis cs:3.2,115.061545887197);

\path [draw=black, thick]
(axis cs:4.2,70.961735997723)
--(axis cs:4.2,142.37159733561);

\path [draw=black, thick]
(axis cs:5.2,6.66111168969428)
--(axis cs:5.2,60.0055549769724);

\path [draw=black, thick]
(axis cs:6.2,44.9384541128033)
--(axis cs:6.2,115.061545887197);

\path [draw=black, thick]
(axis cs:7.2,57.6284026643897)
--(axis cs:7.2,129.038264002277);

\path [draw=black, thick]
(axis cs:8.2,6.66111168969428)
--(axis cs:8.2,60.0055549769724);

\path [draw=black, thick]
(axis cs:9.2,16.3963389389935)
--(axis cs:9.2,76.9369943943399);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_1_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=0, xmax=1,
xtick style={color=black},
xtick={0},
xticklabels={STA 1},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=black},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0}
]
\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_1_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=0, xmax=1,
xtick style={color=black},
xtick={0},
xticklabels={STA 1},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=black},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0}
]
\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_1_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=0, xmax=1,
xtick style={color=black},
xtick={0},
xticklabels={STA 1},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=black},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0}
]
\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_1_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=0, xmax=1,
xtick style={color=black},
xtick={0},
xticklabels={STA 1},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=black},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0}
]
\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_1_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=0, xmax=1,
xtick style={color=black},
xtick={0},
xticklabels={STA 1},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=black},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0}
]
\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_1_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=0, xmax=1,
xtick style={color=black},
xtick={0},
xticklabels={STA 1},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=black},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0}
]
\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_2_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.49, xmax=1.49,
xtick style={color=black},
xtick={0,1},
xticklabels={STA 1,STA 2},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=59.0083551470317,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,12.7889582359593);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,13.1900843035156);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,38.7179743569026);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,48.2821618478923);
\path [draw=black, thick]
(axis cs:-0.2,11.5936642773577)
--(axis cs:-0.2,13.9842521945609);

\path [draw=black, thick]
(axis cs:0.8,11.9435273658691)
--(axis cs:0.8,14.436641241162);

\path [draw=black, thick]
(axis cs:0.2,30.2814681696312)
--(axis cs:0.2,47.154480544174);

\path [draw=black, thick]
(axis cs:1.2,40.3658902224211)
--(axis cs:1.2,56.1984334733635);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_2_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.49, xmax=1.49,
xtick style={color=black},
xtick={0,1},
xticklabels={STA 1,STA 2},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=210,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,200);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,200);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,200);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,200);
\path [draw=black, thick]
(axis cs:-0.2,200)
--(axis cs:-0.2,200);

\path [draw=black, thick]
(axis cs:0.8,200)
--(axis cs:0.8,200);

\path [draw=black, thick]
(axis cs:0.2,200)
--(axis cs:0.2,200);

\path [draw=black, thick]
(axis cs:1.2,200)
--(axis cs:1.2,200);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_2_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.49, xmax=1.49,
xtick style={color=black},
xtick={0,1},
xticklabels={STA 1,STA 2},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=21.532903387498,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,12.7889582359593);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,13.1900843035156);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,14.6749425112556);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,17.4460637581554);
\path [draw=black, thick]
(axis cs:-0.2,11.5936642773577)
--(axis cs:-0.2,13.9842521945609);

\path [draw=black, thick]
(axis cs:0.8,11.9435273658691)
--(axis cs:0.8,14.436641241162);

\path [draw=black, thick]
(axis cs:0.2,12.9891316429359)
--(axis cs:0.2,16.3607533795753);

\path [draw=black, thick]
(axis cs:1.2,14.3846004805983)
--(axis cs:1.2,20.5075270357124);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_2_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.49, xmax=1.49,
xtick style={color=black},
xtick={0,1},
xticklabels={STA 1,STA 2},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=210,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,200);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,200);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,200);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,200);
\path [draw=black, thick]
(axis cs:-0.2,200)
--(axis cs:-0.2,200);

\path [draw=black, thick]
(axis cs:0.8,200)
--(axis cs:0.8,200);

\path [draw=black, thick]
(axis cs:0.2,200)
--(axis cs:0.2,200);

\path [draw=black, thick]
(axis cs:1.2,200)
--(axis cs:1.2,200);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_2_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.49, xmax=1.49,
xtick style={color=black},
xtick={0,1},
xticklabels={STA 1,STA 2},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=15.1584733032201,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,12.7889582359593);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,13.1900843035156);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,9.29007759056414);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,9.29009543942311);
\path [draw=black, thick]
(axis cs:-0.2,11.5936642773577)
--(axis cs:-0.2,13.9842521945609);

\path [draw=black, thick]
(axis cs:0.8,11.9435273658691)
--(axis cs:0.8,14.436641241162);

\path [draw=black, thick]
(axis cs:0.2,9.29001664198312)
--(axis cs:0.2,9.29013853914516);

\path [draw=black, thick]
(axis cs:1.2,9.29003553582907)
--(axis cs:1.2,9.29015534301714);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_2_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.49, xmax=1.49,
xtick style={color=black},
xtick={0,1},
xticklabels={STA 1,STA 2},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=210,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,200);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,200);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,200);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,200);
\path [draw=black, thick]
(axis cs:-0.2,200)
--(axis cs:-0.2,200);

\path [draw=black, thick]
(axis cs:0.8,200)
--(axis cs:0.8,200);

\path [draw=black, thick]
(axis cs:0.2,200)
--(axis cs:0.2,200);

\path [draw=black, thick]
(axis cs:1.2,200)
--(axis cs:1.2,200);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_3_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.54, xmax=2.54,
xtick style={color=black},
xtick={0,1,2},
xticklabels={STA 1,STA 2,STA 3},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=64.7045855738975,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,16.0535017200852);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,16.8348961258177);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,16.7671787562518);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,45.79645137757);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,52.4734298647895);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,49.6542211837077);
\path [draw=black, thick]
(axis cs:-0.2,13.5920619878556)
--(axis cs:-0.2,18.5149414523149);

\path [draw=black, thick]
(axis cs:0.8,14.416083649481)
--(axis cs:0.8,19.2537086021545);

\path [draw=black, thick]
(axis cs:1.8,14.0994608167041)
--(axis cs:1.8,19.4348966957995);

\path [draw=black, thick]
(axis cs:0.2,37.9296168507014)
--(axis cs:0.2,53.6632859044387);

\path [draw=black, thick]
(axis cs:1.2,43.3234448972956)
--(axis cs:1.2,61.6234148322834);

\path [draw=black, thick]
(axis cs:2.2,41.9230986118415)
--(axis cs:2.2,57.3853437555739);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_3_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.5,0.09)}, anchor=south, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.54, xmax=2.54,
xtick style={color=black},
xtick={0,1,2},
xticklabels={STA 1,STA 2,STA 3},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=210.000579562775,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,199.999404605263);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,199.999801535088);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,200);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,200);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,200);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,200);
\path [draw=black, thick]
(axis cs:-0.2,199.998257245979)
--(axis cs:-0.2,200.000551964547);

\path [draw=black, thick]
(axis cs:0.8,199.999419081993)
--(axis cs:0.8,200.000183988182);

\path [draw=black, thick]
(axis cs:1.8,200)
--(axis cs:1.8,200);

\path [draw=black, thick]
(axis cs:0.2,200)
--(axis cs:0.2,200);

\path [draw=black, thick]
(axis cs:1.2,200)
--(axis cs:1.2,200);

\path [draw=black, thick]
(axis cs:2.2,200)
--(axis cs:2.2,200);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_3_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.54, xmax=2.54,
xtick style={color=black},
xtick={0,1,2},
xticklabels={STA 1,STA 2,STA 3},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=32.9586433966763,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,16.0535017200852);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,16.8348961258177);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,16.7671787562518);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,23.3287656566544);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,26.5170071405625);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,25.1519593083455);
\path [draw=black, thick]
(axis cs:-0.2,13.5920619878556)
--(axis cs:-0.2,18.5149414523149);

\path [draw=black, thick]
(axis cs:0.8,14.416083649481)
--(axis cs:0.8,19.2537086021545);

\path [draw=black, thick]
(axis cs:1.8,14.0994608167041)
--(axis cs:1.8,19.4348966957995);

\path [draw=black, thick]
(axis cs:0.2,18.1844529572335)
--(axis cs:0.2,28.4730783560754);

\path [draw=black, thick]
(axis cs:1.2,21.6448300938142)
--(axis cs:1.2,31.3891841873108);

\path [draw=black, thick]
(axis cs:2.2,20.102702191055)
--(axis cs:2.2,30.201216425636);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_3_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.5,0.09)}, anchor=south, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.54, xmax=2.54,
xtick style={color=black},
xtick={0,1,2},
xticklabels={STA 1,STA 2,STA 3},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=210.000579562775,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,199.999404605263);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,199.999801535088);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,200);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,200);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,199.999603070175);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,199.999603070175);
\path [draw=black, thick]
(axis cs:-0.2,199.998257245979)
--(axis cs:-0.2,200.000551964547);

\path [draw=black, thick]
(axis cs:0.8,199.999419081993)
--(axis cs:0.8,200.000183988182);

\path [draw=black, thick]
(axis cs:1.8,200)
--(axis cs:1.8,200);

\path [draw=black, thick]
(axis cs:0.2,200)
--(axis cs:0.2,200);

\path [draw=black, thick]
(axis cs:1.2,199.99907160698)
--(axis cs:1.2,200.00013453337);

\path [draw=black, thick]
(axis cs:2.2,199.99907160698)
--(axis cs:2.2,200.00013453337);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_3_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.54, xmax=2.54,
xtick style={color=black},
xtick={0,1,2},
xticklabels={STA 1,STA 2,STA 3},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=20.4066415305894,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,16.0535017200852);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,16.8348961258177);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,16.7671787562518);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,9.29015906717484);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,9.29024816137916);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,9.29017322198067);
\path [draw=black, thick]
(axis cs:-0.2,13.5920619878556)
--(axis cs:-0.2,18.5149414523149);

\path [draw=black, thick]
(axis cs:0.8,14.416083649481)
--(axis cs:0.8,19.2537086021545);

\path [draw=black, thick]
(axis cs:1.8,14.0994608167041)
--(axis cs:1.8,19.4348966957994);

\path [draw=black, thick]
(axis cs:0.2,9.29004212768135)
--(axis cs:0.2,9.29027600666833);

\path [draw=black, thick]
(axis cs:1.2,9.29015312199696)
--(axis cs:1.2,9.29034320076137);

\path [draw=black, thick]
(axis cs:2.2,9.29009192449957)
--(axis cs:2.2,9.29025451946178);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_3_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.5,0.09)}, anchor=south, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.54, xmax=2.54,
xtick style={color=black},
xtick={0,1,2},
xticklabels={STA 1,STA 2,STA 3},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=210.000579562775,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,199.999404605263);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,199.999801535088);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,200);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,200);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,200);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,200);
\path [draw=black, thick]
(axis cs:-0.2,199.998257245979)
--(axis cs:-0.2,200.000551964547);

\path [draw=black, thick]
(axis cs:0.8,199.999419081993)
--(axis cs:0.8,200.000183988182);

\path [draw=black, thick]
(axis cs:1.8,200)
--(axis cs:1.8,200);

\path [draw=black, thick]
(axis cs:0.2,200)
--(axis cs:0.2,200);

\path [draw=black, thick]
(axis cs:1.2,200)
--(axis cs:1.2,200);

\path [draw=black, thick]
(axis cs:2.2,200)
--(axis cs:2.2,200);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_4_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=66.3315936687761,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,22.5069840393894);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,19.7658003449586);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,20.008516099718);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,22.3507209266639);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,53.3957455837704);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,51.9256905192761);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,54.0636667840204);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,45.1831545575098);
\path [draw=black, thick]
(axis cs:-0.2,19.36250233359)
--(axis cs:-0.2,25.6514657451887);

\path [draw=black, thick]
(axis cs:0.8,16.7247679983343)
--(axis cs:0.8,22.806832691583);

\path [draw=black, thick]
(axis cs:1.8,17.2382853278594)
--(axis cs:1.8,22.7787468715766);

\path [draw=black, thick]
(axis cs:2.8,19.3238249661091)
--(axis cs:2.8,25.3776168872187);

\path [draw=black, thick]
(axis cs:0.2,45.034579374909)
--(axis cs:0.2,61.7569117926319);

\path [draw=black, thick]
(axis cs:1.2,43.4100752236231)
--(axis cs:1.2,60.4413058149291);

\path [draw=black, thick]
(axis cs:2.2,44.9543872168254)
--(axis cs:2.2,63.1729463512154);

\path [draw=black, thick]
(axis cs:3.2,37.5728404221522)
--(axis cs:3.2,52.7934686928675);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_4_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=210.000193187592,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,200);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,199.999801535088);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,200);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,200);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,200);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,200);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,200);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,200);
\path [draw=black, thick]
(axis cs:-0.2,200)
--(axis cs:-0.2,200);

\path [draw=black, thick]
(axis cs:0.8,199.999419081993)
--(axis cs:0.8,200.000183988182);

\path [draw=black, thick]
(axis cs:1.8,200)
--(axis cs:1.8,200);

\path [draw=black, thick]
(axis cs:2.8,200)
--(axis cs:2.8,200);

\path [draw=black, thick]
(axis cs:0.2,200)
--(axis cs:0.2,200);

\path [draw=black, thick]
(axis cs:1.2,200)
--(axis cs:1.2,200);

\path [draw=black, thick]
(axis cs:2.2,200)
--(axis cs:2.2,200);

\path [draw=black, thick]
(axis cs:3.2,200)
--(axis cs:3.2,200);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_4_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=51.5523149881823,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,22.5069840393894);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,19.7658003449586);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,20.008516099718);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,22.3507209266639);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,39.4079066628949);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,41.9023956089627);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,41.677015987086);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,37.7150854057071);
\path [draw=black, thick]
(axis cs:-0.2,19.36250233359)
--(axis cs:-0.2,25.6514657451887);

\path [draw=black, thick]
(axis cs:0.8,16.7247679983343)
--(axis cs:0.8,22.8068326915829);

\path [draw=black, thick]
(axis cs:1.8,17.2382853278594)
--(axis cs:1.8,22.7787468715766);

\path [draw=black, thick]
(axis cs:2.8,19.3238249661091)
--(axis cs:2.8,25.3776168872187);

\path [draw=black, thick]
(axis cs:0.2,33.0333251563455)
--(axis cs:0.2,45.7824881694443);

\path [draw=black, thick]
(axis cs:1.2,34.7073483720376)
--(axis cs:1.2,49.0974428458879);

\path [draw=black, thick]
(axis cs:2.2,34.678180790396)
--(axis cs:2.2,48.6758511837761);

\path [draw=black, thick]
(axis cs:3.2,30.8985471117403)
--(axis cs:3.2,44.5316236996738);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_4_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=210.000193187592,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,200);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,199.999801535088);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,200);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,200);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,199.999801535088);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,199.999801535088);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,200);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,200);
\path [draw=black, thick]
(axis cs:-0.2,200)
--(axis cs:-0.2,200);

\path [draw=black, thick]
(axis cs:0.8,199.999419081993)
--(axis cs:0.8,200.000183988182);

\path [draw=black, thick]
(axis cs:1.8,200)
--(axis cs:1.8,200);

\path [draw=black, thick]
(axis cs:2.8,200)
--(axis cs:2.8,200);

\path [draw=black, thick]
(axis cs:0.2,199.999419081993)
--(axis cs:0.2,200.000183988182);

\path [draw=black, thick]
(axis cs:1.2,199.999419081993)
--(axis cs:1.2,200.000183988182);

\path [draw=black, thick]
(axis cs:2.2,200)
--(axis cs:2.2,200);

\path [draw=black, thick]
(axis cs:3.2,200)
--(axis cs:3.2,200);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_4_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=26.9340390324482,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,22.5069840393894);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,19.7658003449586);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,20.008516099718);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,22.3507209266639);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,9.2902562251531);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,9.29022562450381);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,9.29037971784936);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,9.29028282157731);
\path [draw=black, thick]
(axis cs:-0.2,19.36250233359)
--(axis cs:-0.2,25.6514657451887);

\path [draw=black, thick]
(axis cs:0.8,16.7247679983343)
--(axis cs:0.8,22.8068326915829);

\path [draw=black, thick]
(axis cs:1.8,17.2382853278594)
--(axis cs:1.8,22.7787468715766);

\path [draw=black, thick]
(axis cs:2.8,19.3238249661091)
--(axis cs:2.8,25.3776168872187);

\path [draw=black, thick]
(axis cs:0.2,9.2901151129632)
--(axis cs:0.2,9.29039733734301);

\path [draw=black, thick]
(axis cs:1.2,9.29012559649581)
--(axis cs:1.2,9.2903256525118);

\path [draw=black, thick]
(axis cs:2.2,9.29025601851297)
--(axis cs:2.2,9.29050341718575);

\path [draw=black, thick]
(axis cs:3.2,9.29013673083698)
--(axis cs:3.2,9.29042891231764);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_4_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=210.000193187592,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,200);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,199.999801535088);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,200);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,200);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,200);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,200);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,200);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,200);
\path [draw=black, thick]
(axis cs:-0.2,200)
--(axis cs:-0.2,200);

\path [draw=black, thick]
(axis cs:0.8,199.999419081993)
--(axis cs:0.8,200.000183988182);

\path [draw=black, thick]
(axis cs:1.8,200)
--(axis cs:1.8,200);

\path [draw=black, thick]
(axis cs:2.8,200)
--(axis cs:2.8,200);

\path [draw=black, thick]
(axis cs:0.2,200)
--(axis cs:0.2,200);

\path [draw=black, thick]
(axis cs:1.2,200)
--(axis cs:1.2,200);

\path [draw=black, thick]
(axis cs:2.2,200)
--(axis cs:2.2,200);

\path [draw=black, thick]
(axis cs:3.2,200)
--(axis cs:3.2,200);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_5_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.64, xmax=4.64,
xtick style={color=black},
xtick={0,1,2,3,4},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=245.858983743961,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,195.958451063131);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,189.595825187763);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,179.64225401329);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,177.517809337308);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,210.677775302356);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,39.3913374639533);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,47.4514330267402);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,44.1286211794399);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,46.4347722467934);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,53.5316733022183);
\path [draw=black, thick]
(axis cs:-0.2,170.716347397747)
--(axis cs:-0.2,221.200554728516);

\path [draw=black, thick]
(axis cs:0.8,160.402828200261)
--(axis cs:0.8,218.788822175264);

\path [draw=black, thick]
(axis cs:1.8,159.625909725883)
--(axis cs:1.8,199.658598300696);

\path [draw=black, thick]
(axis cs:2.8,156.143160521605)
--(axis cs:2.8,198.89245815301);

\path [draw=black, thick]
(axis cs:3.8,187.204137515225)
--(axis cs:3.8,234.151413089486);

\path [draw=black, thick]
(axis cs:0.2,31.2578144166514)
--(axis cs:0.2,47.5248605112553);

\path [draw=black, thick]
(axis cs:1.2,39.8667485668129)
--(axis cs:1.2,55.0361174866674);

\path [draw=black, thick]
(axis cs:2.2,35.9118531648434)
--(axis cs:2.2,52.3453891940364);

\path [draw=black, thick]
(axis cs:3.2,37.5870745656029)
--(axis cs:3.2,55.2824699279839);

\path [draw=black, thick]
(axis cs:4.2,45.0517171800493)
--(axis cs:4.2,62.0116294243872);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_5_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.64, xmax=4.64,
xtick style={color=black},
xtick={0,1,2,3,4},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=210,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,182.038874780702);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,180.38996995614);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,183.932939692983);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,187.577775);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,178.396424561403);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,200);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,200);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,200);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,200);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,200);
\path [draw=black, thick]
(axis cs:-0.2,176.922375471057)
--(axis cs:-0.2,187.155374090347);

\path [draw=black, thick]
(axis cs:0.8,173.861234111193)
--(axis cs:0.8,186.918705801088);

\path [draw=black, thick]
(axis cs:1.8,179.890772653897)
--(axis cs:1.8,187.975106732068);

\path [draw=black, thick]
(axis cs:2.8,182.991555394996)
--(axis cs:2.8,192.163994605004);

\path [draw=black, thick]
(axis cs:3.8,172.703835900622)
--(axis cs:3.8,184.089013222185);

\path [draw=black, thick]
(axis cs:0.2,200)
--(axis cs:0.2,200);

\path [draw=black, thick]
(axis cs:1.2,200)
--(axis cs:1.2,200);

\path [draw=black, thick]
(axis cs:2.2,200)
--(axis cs:2.2,200);

\path [draw=black, thick]
(axis cs:3.2,200)
--(axis cs:3.2,200);

\path [draw=black, thick]
(axis cs:4.2,200)
--(axis cs:4.2,200);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_5_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.62, xmax=4.22,
xtick style={color=black},
xtick={0,1,2,3,4},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=240.903057990258,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,193.592550117918);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,189.268414936451);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,179.85952753554);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,172.892336381672);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,206.330252871281);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,38.7721779866008);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,46.0379325047365);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,43.2153509845538);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,50.0568679467296);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,nan);
\path [draw=black, thick]
(axis cs:-0.2,169.362217801091)
--(axis cs:-0.2,217.822882434745);

\path [draw=black, thick]
(axis cs:0.8,160.179713277565)
--(axis cs:0.8,218.357116595337);

\path [draw=black, thick]
(axis cs:1.8,159.935228269778)
--(axis cs:1.8,199.783826801302);

\path [draw=black, thick]
(axis cs:2.8,152.107147773691)
--(axis cs:2.8,193.677524989653);

\path [draw=black, thick]
(axis cs:3.8,183.229021942315)
--(axis cs:3.8,229.431483800246);

\path [draw=black, thick]
(axis cs:0.2,30.7258501062575)
--(axis cs:0.2,46.8185058669441);

\path [draw=black, thick]
(axis cs:1.2,38.4099580340572)
--(axis cs:1.2,53.6659069754159);

\path [draw=black, thick]
(axis cs:2.2,35.2364320131112)
--(axis cs:2.2,51.1942699559963);

\path [draw=black, thick]
(axis cs:3.2,41.5407692085596)
--(axis cs:3.2,58.5729666848995);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_5_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.64, xmax=4.64,
xtick style={color=black},
xtick={0,1,2,3,4},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=216.489395341032,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,181.492814912281);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,180.736793201754);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,184.0166125);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,187.702239912281);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,178.791938815789);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,200);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,200);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,199.999801535088);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,200);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,193.333333333333);
\path [draw=black, thick]
(axis cs:-0.2,176.21828368082)
--(axis cs:-0.2,186.767346143741);

\path [draw=black, thick]
(axis cs:0.8,174.202720721312)
--(axis cs:0.8,187.270865682197);

\path [draw=black, thick]
(axis cs:1.8,179.936769985982)
--(axis cs:1.8,188.096455014018);

\path [draw=black, thick]
(axis cs:2.8,183.166380197569)
--(axis cs:2.8,192.238099626993);

\path [draw=black, thick]
(axis cs:3.8,173.034413681731)
--(axis cs:3.8,184.549463949848);

\path [draw=black, thick]
(axis cs:0.2,200)
--(axis cs:0.2,200);

\path [draw=black, thick]
(axis cs:1.2,200)
--(axis cs:1.2,200);

\path [draw=black, thick]
(axis cs:2.2,199.999419081993)
--(axis cs:2.2,200.000183988182);

\path [draw=black, thick]
(axis cs:3.2,200)
--(axis cs:3.2,200);

\path [draw=black, thick]
(axis cs:4.2,180.486290151398)
--(axis cs:4.2,206.180376515269);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_5_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.64, xmax=4.64,
xtick style={color=black},
xtick={0,1,2,3,4},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=245.85898374396,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,195.958451063131);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,189.595825187762);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,179.642254013289);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,177.517809337308);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,210.677775302356);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,9.29028568230629);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,9.29037800309495);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,9.29037800106319);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,9.29018564949275);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,9.29015872515697);
\path [draw=black, thick]
(axis cs:-0.2,170.716347397747)
--(axis cs:-0.2,221.200554728516);

\path [draw=black, thick]
(axis cs:0.8,160.402828200261)
--(axis cs:0.8,218.788822175264);

\path [draw=black, thick]
(axis cs:1.8,159.625909725883)
--(axis cs:1.8,199.658598300696);

\path [draw=black, thick]
(axis cs:2.8,156.143160521605)
--(axis cs:2.8,198.89245815301);

\path [draw=black, thick]
(axis cs:3.8,187.204137515225)
--(axis cs:3.8,234.151413089486);

\path [draw=black, thick]
(axis cs:0.2,9.29014423036002)
--(axis cs:0.2,9.29042713425257);

\path [draw=black, thick]
(axis cs:1.2,9.29023671919638)
--(axis cs:1.2,9.29051928699352);

\path [draw=black, thick]
(axis cs:2.2,9.29023925012099)
--(axis cs:2.2,9.29051675200538);

\path [draw=black, thick]
(axis cs:3.2,9.2900559052428)
--(axis cs:3.2,9.2903153937427);

\path [draw=black, thick]
(axis cs:4.2,9.29003624398051)
--(axis cs:4.2,9.29028120633344);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_5_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.64, xmax=4.64,
xtick style={color=black},
xtick={0,1,2,3,4},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=210,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,182.038874780702);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,180.38996995614);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,183.932939692982);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,187.577775);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,178.396424561403);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,200);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,200);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,200);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,200);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,200);
\path [draw=black, thick]
(axis cs:-0.2,176.922375471057)
--(axis cs:-0.2,187.155374090347);

\path [draw=black, thick]
(axis cs:0.8,173.861234111193)
--(axis cs:0.8,186.918705801088);

\path [draw=black, thick]
(axis cs:1.8,179.890772653897)
--(axis cs:1.8,187.975106732068);

\path [draw=black, thick]
(axis cs:2.8,182.991555394996)
--(axis cs:2.8,192.163994605004);

\path [draw=black, thick]
(axis cs:3.8,172.703835900622)
--(axis cs:3.8,184.089013222185);

\path [draw=black, thick]
(axis cs:0.2,200)
--(axis cs:0.2,200);

\path [draw=black, thick]
(axis cs:1.2,200)
--(axis cs:1.2,200);

\path [draw=black, thick]
(axis cs:2.2,200)
--(axis cs:2.2,200);

\path [draw=black, thick]
(axis cs:3.2,200)
--(axis cs:3.2,200);

\path [draw=black, thick]
(axis cs:4.2,200)
--(axis cs:4.2,200);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_6_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.67, xmax=5.27,
xtick style={color=black},
xtick={0,1,2,3,4,5},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=375.89660007051,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,342.718957475538);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,314.273084273768);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,309.641536587981);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,311.635623411791);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,316.258056038941);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,329.059094254826);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,nan);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,51.3658838303705);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,nan);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,nan);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,nan);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,nan);
\path [draw=black, thick]
(axis cs:-0.2,327.441152979162)
--(axis cs:-0.2,357.996761971914);

\path [draw=black, thick]
(axis cs:0.8,302.265791303661)
--(axis cs:0.8,326.280377243875);

\path [draw=black, thick]
(axis cs:1.8,288.671918928603)
--(axis cs:1.8,330.611154247359);

\path [draw=black, thick]
(axis cs:2.8,293.754219532992)
--(axis cs:2.8,329.51702729059);

\path [draw=black, thick]
(axis cs:3.8,301.057541745536)
--(axis cs:3.8,331.458570332346);

\path [draw=black, thick]
(axis cs:4.8,307.088453299886)
--(axis cs:4.8,351.029735209766);

\path [draw=black, thick]
(axis cs:1.2,43.2388726558378)
--(axis cs:1.2,59.4928950049032);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_6_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.69, xmax=5.69,
xtick style={color=black},
xtick={0,1,2,3,4,5},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=214.745088601195,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,140.579383552632);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,150.64986381579);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,152.508764912281);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,152.674364473684);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,143.800691666667);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,145.002404385965);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,186.666666666667);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,200);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,180);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,173.333333333333);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,146.666666666667);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,113.333333333333);
\path [draw=black, thick]
(axis cs:-0.2,133.629686605392)
--(axis cs:-0.2,147.529080499871);

\path [draw=black, thick]
(axis cs:0.8,144.612794924802)
--(axis cs:0.8,156.686932706777);

\path [draw=black, thick]
(axis cs:1.8,145.769806907006)
--(axis cs:1.8,159.247722917556);

\path [draw=black, thick]
(axis cs:2.8,145.627821531486)
--(axis cs:2.8,159.720907415883);

\path [draw=black, thick]
(axis cs:3.8,136.998351864393)
--(axis cs:3.8,150.60303146894);

\path [draw=black, thick]
(axis cs:4.8,136.158725197157)
--(axis cs:4.8,153.846083574773);

\path [draw=black, thick]
(axis cs:0.2,168.814201332195)
--(axis cs:0.2,204.519132001139);

\path [draw=black, thick]
(axis cs:1.2,200)
--(axis cs:1.2,200);

\path [draw=black, thick]
(axis cs:2.2,158.529275745797)
--(axis cs:2.2,201.470724254203);

\path [draw=black, thick]
(axis cs:3.2,149.004524012634)
--(axis cs:3.2,197.662142654033);

\path [draw=black, thick]
(axis cs:4.2,115.017628298501)
--(axis cs:4.2,178.315705034832);

\path [draw=black, thick]
(axis cs:5.2,77.8683041313674)
--(axis cs:5.2,148.798362535299);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_6_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.67, xmax=5.27,
xtick style={color=black},
xtick={0,1,2,3,4,5},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=374.212401656819,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,341.664890036359);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,314.921566321677);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,311.075530606773);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,311.242638306027);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,316.648452432467);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,330.751732643548);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,44.1275576233499);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,nan);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,nan);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,nan);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,nan);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,nan);
\path [draw=black, thick]
(axis cs:-0.2,326.937016590034)
--(axis cs:-0.2,356.392763482685);

\path [draw=black, thick]
(axis cs:0.8,303.140282676157)
--(axis cs:0.8,326.702849967197);

\path [draw=black, thick]
(axis cs:1.8,290.190614934822)
--(axis cs:1.8,331.960446278725);

\path [draw=black, thick]
(axis cs:2.8,293.382289790207)
--(axis cs:2.8,329.102986821847);

\path [draw=black, thick]
(axis cs:3.8,301.259496929902)
--(axis cs:3.8,332.037407935032);

\path [draw=black, thick]
(axis cs:4.8,308.880342278898)
--(axis cs:4.8,352.623123008198);

\path [draw=black, thick]
(axis cs:0.2,36.9679717544205)
--(axis cs:0.2,51.2871434922792);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_6_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.69, xmax=5.69,
xtick style={color=black},
xtick={0,1,2,3,4,5},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=216.489173111405,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,140.460672368421);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,152.07293245614);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,151.938665131579);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,152.935766666667);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,142.813755482456);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,144.761539254386);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,200);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,193.333134868421);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,166.666666666667);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,153.333333333333);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,153.332936403509);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,133.333333333333);
\path [draw=black, thick]
(axis cs:-0.2,133.485115079326)
--(axis cs:-0.2,147.436229657516);

\path [draw=black, thick]
(axis cs:0.8,146.369924774256)
--(axis cs:0.8,157.775940138024);

\path [draw=black, thick]
(axis cs:1.8,145.370740785787)
--(axis cs:1.8,158.50658947737);

\path [draw=black, thick]
(axis cs:2.8,145.853857025736)
--(axis cs:2.8,160.017676307597);

\path [draw=black, thick]
(axis cs:3.8,136.056540826915)
--(axis cs:3.8,149.570970137997);

\path [draw=black, thick]
(axis cs:4.8,135.895961151608)
--(axis cs:4.8,153.627117357164);

\path [draw=black, thick]
(axis cs:0.2,200)
--(axis cs:0.2,200);

\path [draw=black, thick]
(axis cs:1.2,180.486104868837)
--(axis cs:1.2,206.180164868005);

\path [draw=black, thick]
(axis cs:2.2,139.994445023028)
--(axis cs:2.2,193.338888310306);

\path [draw=black, thick]
(axis cs:3.2,123.06300560566)
--(axis cs:3.2,183.603661061007);

\path [draw=black, thick]
(axis cs:4.2,123.062687026246)
--(axis cs:4.2,183.603185780772);

\path [draw=black, thick]
(axis cs:5.2,99.5953450730376)
--(axis cs:5.2,167.071321593629);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_6_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.67, xmax=5.27,
xtick style={color=black},
xtick={0,1,2,3,4,5},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=375.027487844322,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,341.962014070548);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,309.697901570786);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,308.730631966217);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,314.046671111218);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,319.582048348902);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,336.760694599683);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,nan);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,9.29029419246982);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,nan);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,nan);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,nan);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,nan);
\path [draw=black, thick]
(axis cs:-0.2,327.304543862446)
--(axis cs:-0.2,356.619484278649);

\path [draw=black, thick]
(axis cs:0.8,299.50047129934)
--(axis cs:0.8,319.895331842233);

\path [draw=black, thick]
(axis cs:1.8,287.254898599505)
--(axis cs:1.8,330.206365332928);

\path [draw=black, thick]
(axis cs:2.8,296.565585659865)
--(axis cs:2.8,331.527756562571);

\path [draw=black, thick]
(axis cs:3.8,303.18426894929)
--(axis cs:3.8,335.979827748514);

\path [draw=black, thick]
(axis cs:4.8,316.352353157155)
--(axis cs:4.8,357.169036042212);

\path [draw=black, thick]
(axis cs:1.2,9.29016472585681)
--(axis cs:1.2,9.29042365908282);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_6_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.69, xmax=5.69,
xtick style={color=black},
xtick={0,1,2,3,4,5},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=214.745088601195,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,139.774006578947);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,154.120053508772);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,153.065542982456);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,152.414782894737);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,142.178188596491);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,143.575838157895);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,186.666666666667);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,200);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,180);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,173.333333333333);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,146.666666666667);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,113.333333333333);
\path [draw=black, thick]
(axis cs:-0.2,132.783155973365)
--(axis cs:-0.2,146.76485718453);

\path [draw=black, thick]
(axis cs:0.8,148.642153892488)
--(axis cs:0.8,159.597953125056);

\path [draw=black, thick]
(axis cs:1.8,146.158412654239)
--(axis cs:1.8,159.972673310673);

\path [draw=black, thick]
(axis cs:2.8,145.473644136214)
--(axis cs:2.8,159.355921653259);

\path [draw=black, thick]
(axis cs:3.8,135.2201308973)
--(axis cs:3.8,149.136246295683);

\path [draw=black, thick]
(axis cs:4.8,134.679113205556)
--(axis cs:4.8,152.472563110234);

\path [draw=black, thick]
(axis cs:0.2,168.814201332195)
--(axis cs:0.2,204.519132001139);

\path [draw=black, thick]
(axis cs:1.2,200)
--(axis cs:1.2,200);

\path [draw=black, thick]
(axis cs:2.2,158.529275745797)
--(axis cs:2.2,201.470724254203);

\path [draw=black, thick]
(axis cs:3.2,149.004524012634)
--(axis cs:3.2,197.662142654033);

\path [draw=black, thick]
(axis cs:4.2,115.017628298501)
--(axis cs:4.2,178.315705034832);

\path [draw=black, thick]
(axis cs:5.2,77.8683041313674)
--(axis cs:5.2,148.798362535299);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_7_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.72, xmax=6.32,
xtick style={color=black},
xtick={0,1,2,3,4,5,6},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=415.771833914296,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,385.136404121021);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,358.903823362604);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,357.937506681722);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,368.765262954385);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,351.835244335643);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,366.216885491233);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,375.462038714706);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,nan);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,nan);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,nan);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,nan);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,nan);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,nan);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,nan);
\path [draw=black, thick]
(axis cs:-0.2,374.29963308557)
--(axis cs:-0.2,395.973175156473);

\path [draw=black, thick]
(axis cs:0.8,343.512353233327)
--(axis cs:0.8,374.295293491882);

\path [draw=black, thick]
(axis cs:1.8,341.574308258055)
--(axis cs:1.8,374.300705105389);

\path [draw=black, thick]
(axis cs:2.8,355.232774854059)
--(axis cs:2.8,382.297751054712);

\path [draw=black, thick]
(axis cs:3.8,333.409458754317)
--(axis cs:3.8,370.261029916969);

\path [draw=black, thick]
(axis cs:4.8,350.536224446749)
--(axis cs:4.8,381.897546535717);

\path [draw=black, thick]
(axis cs:5.8,364.347987818052)
--(axis cs:5.8,386.576089611359);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_7_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.74, xmax=6.74,
xtick style={color=black},
xtick={0,1,2,3,4,5,6},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=211.544260466913,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,107.278823464912);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,124.863973684211);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,134.945768859649);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,121.656647149123);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,133.336608991228);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,128.100964254386);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,119.027646929825);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,153.333333333333);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,180);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,173.333333333333);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,126.666666666667);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,160);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,86.6666666666667);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,120);
\path [draw=black, thick]
(axis cs:-0.2,98.512335725931)
--(axis cs:-0.2,116.045311203894);

\path [draw=black, thick]
(axis cs:0.8,117.367787930333)
--(axis cs:0.8,132.360159438088);

\path [draw=black, thick]
(axis cs:1.8,127.039902471147)
--(axis cs:1.8,142.851635248151);

\path [draw=black, thick]
(axis cs:2.8,113.801442944193)
--(axis cs:2.8,129.511851354053);

\path [draw=black, thick]
(axis cs:3.8,126.104543928551)
--(axis cs:3.8,140.568674053906);

\path [draw=black, thick]
(axis cs:4.8,119.724246792482)
--(axis cs:4.8,136.47768171629);

\path [draw=black, thick]
(axis cs:5.8,113.596004200543)
--(axis cs:5.8,124.459289659106);

\path [draw=black, thick]
(axis cs:0.2,123.06300560566)
--(axis cs:0.2,183.603661061007);

\path [draw=black, thick]
(axis cs:1.2,158.529275745797)
--(axis cs:1.2,201.470724254203);

\path [draw=black, thick]
(axis cs:2.2,149.004524012634)
--(axis cs:2.2,197.662142654033);

\path [draw=black, thick]
(axis cs:3.2,92.1779266898977)
--(axis cs:3.2,161.155406643436);

\path [draw=black, thick]
(axis cs:4.2,131.372367661063)
--(axis cs:4.2,188.627632338937);

\path [draw=black, thick]
(axis cs:5.2,51.2016374647007)
--(axis cs:5.2,122.131695868633);

\path [draw=black, thick]
(axis cs:6.2,84.9384541128033)
--(axis cs:6.2,155.061545887197);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_7_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.72, xmax=6.32,
xtick style={color=black},
xtick={0,1,2,3,4,5,6},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=415.771833914296,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,385.136404121021);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,358.903823362604);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,357.937506681722);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,368.765262954385);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,351.835244335643);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,366.216885491233);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,375.462038714706);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,nan);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,nan);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,nan);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,nan);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,nan);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,nan);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,nan);
\path [draw=black, thick]
(axis cs:-0.2,374.29963308557)
--(axis cs:-0.2,395.973175156473);

\path [draw=black, thick]
(axis cs:0.8,343.512353233327)
--(axis cs:0.8,374.295293491881);

\path [draw=black, thick]
(axis cs:1.8,341.574308258055)
--(axis cs:1.8,374.300705105389);

\path [draw=black, thick]
(axis cs:2.8,355.232774854059)
--(axis cs:2.8,382.297751054712);

\path [draw=black, thick]
(axis cs:3.8,333.409458754317)
--(axis cs:3.8,370.261029916969);

\path [draw=black, thick]
(axis cs:4.8,350.536224446749)
--(axis cs:4.8,381.897546535717);

\path [draw=black, thick]
(axis cs:5.8,364.347987818052)
--(axis cs:5.8,386.576089611359);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_7_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.74, xmax=6.74,
xtick style={color=black},
xtick={0,1,2,3,4,5,6},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=211.544260466913,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,107.278823464912);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,124.863973684211);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,134.945768859649);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,121.656647149123);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,133.336608991228);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,128.100964254386);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,119.027646929825);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,160);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,180);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,166.666666666667);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,126.666666666667);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,153.333333333333);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,86.6666666666667);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,126.646941008772);
\path [draw=black, thick]
(axis cs:-0.2,98.512335725931)
--(axis cs:-0.2,116.045311203894);

\path [draw=black, thick]
(axis cs:0.8,117.367787930333)
--(axis cs:0.8,132.360159438088);

\path [draw=black, thick]
(axis cs:1.8,127.039902471147)
--(axis cs:1.8,142.851635248151);

\path [draw=black, thick]
(axis cs:2.8,113.801442944193)
--(axis cs:2.8,129.511851354053);

\path [draw=black, thick]
(axis cs:3.8,126.104543928551)
--(axis cs:3.8,140.568674053906);

\path [draw=black, thick]
(axis cs:4.8,119.724246792482)
--(axis cs:4.8,136.47768171629);

\path [draw=black, thick]
(axis cs:5.8,113.596004200543)
--(axis cs:5.8,124.459289659106);

\path [draw=black, thick]
(axis cs:0.2,131.372367661063)
--(axis cs:0.2,188.627632338937);

\path [draw=black, thick]
(axis cs:1.2,158.529275745797)
--(axis cs:1.2,201.470724254203);

\path [draw=black, thick]
(axis cs:2.2,139.994445023028)
--(axis cs:2.2,193.338888310306);

\path [draw=black, thick]
(axis cs:3.2,92.1779266898977)
--(axis cs:3.2,161.155406643436);

\path [draw=black, thick]
(axis cs:4.2,123.06300560566)
--(axis cs:4.2,183.603661061007);

\path [draw=black, thick]
(axis cs:5.2,51.2016374647007)
--(axis cs:5.2,122.131695868633);

\path [draw=black, thick]
(axis cs:6.2,92.1635513917012)
--(axis cs:6.2,161.130330625843);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_7_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.72, xmax=6.32,
xtick style={color=black},
xtick={0,1,2,3,4,5,6},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=415.771833914296,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,385.136404121021);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,358.903823362604);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,357.937506681722);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,368.765262954385);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,351.835244335643);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,366.216885491233);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,375.462038714706);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,nan);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,nan);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,nan);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,nan);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,nan);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,nan);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,nan);
\path [draw=black, thick]
(axis cs:-0.2,374.29963308557)
--(axis cs:-0.2,395.973175156473);

\path [draw=black, thick]
(axis cs:0.8,343.512353233327)
--(axis cs:0.8,374.295293491881);

\path [draw=black, thick]
(axis cs:1.8,341.574308258055)
--(axis cs:1.8,374.300705105389);

\path [draw=black, thick]
(axis cs:2.8,355.232774854059)
--(axis cs:2.8,382.297751054712);

\path [draw=black, thick]
(axis cs:3.8,333.409458754317)
--(axis cs:3.8,370.261029916969);

\path [draw=black, thick]
(axis cs:4.8,350.536224446749)
--(axis cs:4.8,381.897546535717);

\path [draw=black, thick]
(axis cs:5.8,364.347987818052)
--(axis cs:5.8,386.576089611359);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_7_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.74, xmax=6.74,
xtick style={color=black},
xtick={0,1,2,3,4,5,6},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=211.544260466913,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,107.278823464912);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,124.863973684211);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,134.945768859649);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,121.656647149123);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,133.336608991228);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,128.100964254386);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,119.027646929825);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,153.333333333333);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,180);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,173.333333333333);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,126.666666666667);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,160);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,93.3333333333333);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,113.333333333333);
\path [draw=black, thick]
(axis cs:-0.2,98.512335725931)
--(axis cs:-0.2,116.045311203894);

\path [draw=black, thick]
(axis cs:0.8,117.367787930333)
--(axis cs:0.8,132.360159438088);

\path [draw=black, thick]
(axis cs:1.8,127.039902471147)
--(axis cs:1.8,142.851635248151);

\path [draw=black, thick]
(axis cs:2.8,113.801442944193)
--(axis cs:2.8,129.511851354053);

\path [draw=black, thick]
(axis cs:3.8,126.104543928551)
--(axis cs:3.8,140.568674053906);

\path [draw=black, thick]
(axis cs:4.8,119.724246792482)
--(axis cs:4.8,136.47768171629);

\path [draw=black, thick]
(axis cs:5.8,113.596004200543)
--(axis cs:5.8,124.459289659106);

\path [draw=black, thick]
(axis cs:0.2,123.06300560566)
--(axis cs:0.2,183.603661061007);

\path [draw=black, thick]
(axis cs:1.2,158.529275745797)
--(axis cs:1.2,201.470724254203);

\path [draw=black, thick]
(axis cs:2.2,149.004524012634)
--(axis cs:2.2,197.662142654033);

\path [draw=black, thick]
(axis cs:3.2,92.1779266898977)
--(axis cs:3.2,161.155406643436);

\path [draw=black, thick]
(axis cs:4.2,131.372367661063)
--(axis cs:4.2,188.627632338937);

\path [draw=black, thick]
(axis cs:5.2,57.6284026643897)
--(axis cs:5.2,129.038264002277);

\path [draw=black, thick]
(axis cs:6.2,77.8683041313674)
--(axis cs:6.2,148.798362535299);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_8_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.77, xmax=7.37,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=431.207767233121,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,395.330875905368);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,395.430936080682);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,391.198503124567);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,390.227186815451);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,392.049228625501);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,396.110446520544);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,380.285045850483);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,395.641276238176);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,nan);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,nan);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,nan);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,nan);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,nan);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,nan);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,nan);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,nan);
\path [draw=black, thick]
(axis cs:-0.2,387.346590083787)
--(axis cs:-0.2,403.315161726949);

\path [draw=black, thick]
(axis cs:0.8,384.273735576639)
--(axis cs:0.8,406.588136584725);

\path [draw=black, thick]
(axis cs:1.8,375.001910596615)
--(axis cs:1.8,407.395095652518);

\path [draw=black, thick]
(axis cs:2.8,379.317416858661)
--(axis cs:2.8,401.136956772242);

\path [draw=black, thick]
(axis cs:3.8,380.191187288839)
--(axis cs:3.8,403.907269962164);

\path [draw=black, thick]
(axis cs:4.8,381.546829009544)
--(axis cs:4.8,410.674064031544);

\path [draw=black, thick]
(axis cs:5.8,366.688127944321)
--(axis cs:5.8,393.881963756645);

\path [draw=black, thick]
(axis cs:6.8,385.222330818765)
--(axis cs:6.8,406.060221657588);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_8_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.79, xmax=7.79,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=203.005832725821,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,100.211647807018);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,104.954720394737);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,103.338448903509);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,109.325323684211);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,112.173349342105);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,106.085132675439);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,115.579783991228);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,104.511798026316);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,146.666666666667);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,166.666666666667);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,166.666666666667);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,93.3333333333333);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,146.666666666667);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,80);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,106.666666666667);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,93.3333333333333);
\path [draw=black, thick]
(axis cs:-0.2,92.8601062443642)
--(axis cs:-0.2,107.563189369671);

\path [draw=black, thick]
(axis cs:0.8,97.2196049008702)
--(axis cs:0.8,112.689835888603);

\path [draw=black, thick]
(axis cs:1.8,94.6139485411872)
--(axis cs:1.8,112.06294926583);

\path [draw=black, thick]
(axis cs:2.8,102.152489143252)
--(axis cs:2.8,116.498158225169);

\path [draw=black, thick]
(axis cs:3.8,104.802479053002)
--(axis cs:3.8,119.544219631209);

\path [draw=black, thick]
(axis cs:4.8,99.8714495593103)
--(axis cs:4.8,112.298815791567);

\path [draw=black, thick]
(axis cs:5.8,107.538978707558)
--(axis cs:5.8,123.620589274898);

\path [draw=black, thick]
(axis cs:6.8,96.3621425193188)
--(axis cs:6.8,112.661453533313);

\path [draw=black, thick]
(axis cs:0.2,115.017628298501)
--(axis cs:0.2,178.315705034832);

\path [draw=black, thick]
(axis cs:1.2,139.994445023028)
--(axis cs:1.2,193.338888310306);

\path [draw=black, thick]
(axis cs:2.2,139.994445023028)
--(axis cs:2.2,193.338888310306);

\path [draw=black, thick]
(axis cs:3.2,57.6284026643897)
--(axis cs:3.2,129.038264002277);

\path [draw=black, thick]
(axis cs:4.2,115.017628298501)
--(axis cs:4.2,178.315705034832);

\path [draw=black, thick]
(axis cs:5.2,44.9384541128033)
--(axis cs:5.2,115.061545887197);

\path [draw=black, thick]
(axis cs:6.2,70.961735997723)
--(axis cs:6.2,142.37159733561);

\path [draw=black, thick]
(axis cs:7.2,57.6284026643897)
--(axis cs:7.2,129.038264002277);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_8_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.77, xmax=7.37,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=431.207767233121,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,395.330875905368);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,395.430936080682);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,391.198503124567);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,390.227186815451);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,392.049228625501);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,396.110446520544);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,380.285045850483);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,395.641276238177);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,nan);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,nan);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,nan);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,nan);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,nan);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,nan);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,nan);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,nan);
\path [draw=black, thick]
(axis cs:-0.2,387.346590083787)
--(axis cs:-0.2,403.315161726949);

\path [draw=black, thick]
(axis cs:0.8,384.273735576639)
--(axis cs:0.8,406.588136584725);

\path [draw=black, thick]
(axis cs:1.8,375.001910596615)
--(axis cs:1.8,407.395095652518);

\path [draw=black, thick]
(axis cs:2.8,379.317416858661)
--(axis cs:2.8,401.136956772242);

\path [draw=black, thick]
(axis cs:3.8,380.191187288839)
--(axis cs:3.8,403.907269962164);

\path [draw=black, thick]
(axis cs:4.8,381.546829009544)
--(axis cs:4.8,410.674064031544);

\path [draw=black, thick]
(axis cs:5.8,366.688127944321)
--(axis cs:5.8,393.881963756645);

\path [draw=black, thick]
(axis cs:6.8,385.222330818765)
--(axis cs:6.8,406.060221657588);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_8_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.79, xmax=7.79,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=203.005832725821,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,100.211647807018);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,104.954720394737);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,103.338448903509);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,109.325323684211);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,112.173349342105);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,106.085132675439);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,115.579783991228);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,104.511798026316);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,146.666666666667);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,153.333134868421);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,166.666666666667);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,93.3333333333333);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,146.666666666667);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,86.6664682017544);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,113.333333333333);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,93.3333333333333);
\path [draw=black, thick]
(axis cs:-0.2,92.8601062443642)
--(axis cs:-0.2,107.563189369671);

\path [draw=black, thick]
(axis cs:0.8,97.2196049008703)
--(axis cs:0.8,112.689835888603);

\path [draw=black, thick]
(axis cs:1.8,94.6139485411872)
--(axis cs:1.8,112.06294926583);

\path [draw=black, thick]
(axis cs:2.8,102.152489143252)
--(axis cs:2.8,116.498158225169);

\path [draw=black, thick]
(axis cs:3.8,104.802479053002)
--(axis cs:3.8,119.544219631209);

\path [draw=black, thick]
(axis cs:4.8,99.8714495593103)
--(axis cs:4.8,112.298815791567);

\path [draw=black, thick]
(axis cs:5.8,107.538978707558)
--(axis cs:5.8,123.620589274898);

\path [draw=black, thick]
(axis cs:6.8,96.3621425193188)
--(axis cs:6.8,112.661453533313);

\path [draw=black, thick]
(axis cs:0.2,115.017628298501)
--(axis cs:0.2,178.315705034832);

\path [draw=black, thick]
(axis cs:1.2,123.062846318344)
--(axis cs:1.2,183.603423418498);

\path [draw=black, thick]
(axis cs:2.2,139.994445023028)
--(axis cs:2.2,193.338888310306);

\path [draw=black, thick]
(axis cs:3.2,57.6284026643897)
--(axis cs:3.2,129.038264002277);

\path [draw=black, thick]
(axis cs:4.2,115.017628298501)
--(axis cs:4.2,178.315705034832);

\path [draw=black, thick]
(axis cs:5.2,51.2015202120182)
--(axis cs:5.2,122.131416191491);

\path [draw=black, thick]
(axis cs:6.2,77.8683041313674)
--(axis cs:6.2,148.798362535299);

\path [draw=black, thick]
(axis cs:7.2,57.6284026643897)
--(axis cs:7.2,129.038264002277);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_8_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.77, xmax=7.37,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=431.207767233121,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,395.330875905368);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,395.430936080682);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,391.198503124567);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,390.227186815451);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,392.049228625501);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,396.110446520544);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,380.285045850483);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,395.641276238176);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,nan);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,nan);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,nan);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,nan);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,nan);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,nan);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,nan);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,nan);
\path [draw=black, thick]
(axis cs:-0.2,387.346590083787)
--(axis cs:-0.2,403.315161726949);

\path [draw=black, thick]
(axis cs:0.8,384.273735576639)
--(axis cs:0.8,406.588136584725);

\path [draw=black, thick]
(axis cs:1.8,375.001910596615)
--(axis cs:1.8,407.395095652518);

\path [draw=black, thick]
(axis cs:2.8,379.317416858661)
--(axis cs:2.8,401.136956772242);

\path [draw=black, thick]
(axis cs:3.8,380.191187288839)
--(axis cs:3.8,403.907269962164);

\path [draw=black, thick]
(axis cs:4.8,381.546829009544)
--(axis cs:4.8,410.674064031544);

\path [draw=black, thick]
(axis cs:5.8,366.68812794432)
--(axis cs:5.8,393.881963756645);

\path [draw=black, thick]
(axis cs:6.8,385.222330818765)
--(axis cs:6.8,406.060221657588);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_8_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.79, xmax=7.79,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=198.059013955884,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,100.211647807018);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,104.954720394737);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,103.338448903509);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,109.325323684211);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,112.173349342105);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,106.085132675439);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,115.579783991228);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,104.511798026316);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,160);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,153.333333333333);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,160);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,93.3333333333333);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,146.666666666667);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,80);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,113.333333333333);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,93.3333333333333);
\path [draw=black, thick]
(axis cs:-0.2,92.8601062443642)
--(axis cs:-0.2,107.563189369671);

\path [draw=black, thick]
(axis cs:0.8,97.2196049008702)
--(axis cs:0.8,112.689835888603);

\path [draw=black, thick]
(axis cs:1.8,94.6139485411872)
--(axis cs:1.8,112.06294926583);

\path [draw=black, thick]
(axis cs:2.8,102.152489143252)
--(axis cs:2.8,116.498158225169);

\path [draw=black, thick]
(axis cs:3.8,104.802479053002)
--(axis cs:3.8,119.544219631209);

\path [draw=black, thick]
(axis cs:4.8,99.8714495593103)
--(axis cs:4.8,112.298815791567);

\path [draw=black, thick]
(axis cs:5.8,107.538978707558)
--(axis cs:5.8,123.620589274898);

\path [draw=black, thick]
(axis cs:6.8,96.3621425193188)
--(axis cs:6.8,112.661453533313);

\path [draw=black, thick]
(axis cs:0.2,131.372367661063)
--(axis cs:0.2,188.627632338937);

\path [draw=black, thick]
(axis cs:1.2,123.06300560566)
--(axis cs:1.2,183.603661061007);

\path [draw=black, thick]
(axis cs:2.2,131.372367661063)
--(axis cs:2.2,188.627632338937);

\path [draw=black, thick]
(axis cs:3.2,57.6284026643897)
--(axis cs:3.2,129.038264002277);

\path [draw=black, thick]
(axis cs:4.2,115.017628298501)
--(axis cs:4.2,178.315705034832);

\path [draw=black, thick]
(axis cs:5.2,44.9384541128033)
--(axis cs:5.2,115.061545887197);

\path [draw=black, thick]
(axis cs:6.2,77.8683041313674)
--(axis cs:6.2,148.798362535299);

\path [draw=black, thick]
(axis cs:7.2,57.6284026643897)
--(axis cs:7.2,129.038264002277);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_9_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.82, xmax=8.42,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=445.455773378405,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,411.106220509766);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,413.813529379057);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,405.960052746498);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,414.344744481369);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,407.664535063296);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,409.918006802485);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,405.446181299816);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,407.834614390088);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,417.239298097495);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,nan);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,nan);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,nan);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,nan);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,nan);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,nan);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,nan);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,nan);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,nan);
\path [draw=black, thick]
(axis cs:-0.2,402.994594420072)
--(axis cs:-0.2,419.21784659946);

\path [draw=black, thick]
(axis cs:0.8,406.068976660008)
--(axis cs:0.8,421.558082098106);

\path [draw=black, thick]
(axis cs:1.8,397.129267206125)
--(axis cs:1.8,414.79083828687);

\path [draw=black, thick]
(axis cs:2.8,405.300868213837)
--(axis cs:2.8,423.388620748901);

\path [draw=black, thick]
(axis cs:3.8,397.845634542751)
--(axis cs:3.8,417.483435583841);

\path [draw=black, thick]
(axis cs:4.8,401.619079419647)
--(axis cs:4.8,418.216934185323);

\path [draw=black, thick]
(axis cs:5.8,396.917729142865)
--(axis cs:5.8,413.974633456767);

\path [draw=black, thick]
(axis cs:6.8,397.827119999288)
--(axis cs:6.8,417.842108780887);

\path [draw=black, thick]
(axis cs:7.8,410.23500250127)
--(axis cs:7.8,424.243593693719);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_9_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.84, xmax=8.84,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=211.544260466913,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,91.7255526315789);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,91.950863377193);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,89.7872432017544);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,93.9573563596491);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,97.3467423245614);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,94.5667328947368);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,99.3053877192982);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,93.5158949561404);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,91.7089824561403);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,133.333333333333);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,180);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,173.333333333333);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,53.3333333333333);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,140);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,86.6666666666667);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,86.6666666666667);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,80);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,66.6666666666667);
\path [draw=black, thick]
(axis cs:-0.2,86.9320048920504)
--(axis cs:-0.2,96.5191003711074);

\path [draw=black, thick]
(axis cs:0.8,85.6632080301693)
--(axis cs:0.8,98.2385187242166);

\path [draw=black, thick]
(axis cs:1.8,82.8077820087686)
--(axis cs:1.8,96.7667043947401);

\path [draw=black, thick]
(axis cs:2.8,87.8650663310107)
--(axis cs:2.8,100.049646388288);

\path [draw=black, thick]
(axis cs:3.8,91.3831338046634)
--(axis cs:3.8,103.310350844459);

\path [draw=black, thick]
(axis cs:4.8,88.3231292106203)
--(axis cs:4.8,100.810336578853);

\path [draw=black, thick]
(axis cs:5.8,92.8338681144188)
--(axis cs:5.8,105.776907324178);

\path [draw=black, thick]
(axis cs:6.8,85.0688030542233)
--(axis cs:6.8,101.962986858057);

\path [draw=black, thick]
(axis cs:7.8,84.9927087487573)
--(axis cs:7.8,98.4252561635234);

\path [draw=black, thick]
(axis cs:0.2,99.5953450730376)
--(axis cs:0.2,167.071321593629);

\path [draw=black, thick]
(axis cs:1.2,158.529275745797)
--(axis cs:1.2,201.470724254203);

\path [draw=black, thick]
(axis cs:2.2,149.004524012634)
--(axis cs:2.2,197.662142654033);

\path [draw=black, thick]
(axis cs:3.2,21.6842949651676)
--(axis cs:3.2,84.9823717014991);

\path [draw=black, thick]
(axis cs:4.2,107.202926959864)
--(axis cs:4.2,172.797073040136);

\path [draw=black, thick]
(axis cs:5.2,51.2016374647007)
--(axis cs:5.2,122.131695868633);

\path [draw=black, thick]
(axis cs:6.2,51.2016374647007)
--(axis cs:6.2,122.131695868633);

\path [draw=black, thick]
(axis cs:7.2,44.9384541128033)
--(axis cs:7.2,115.061545887197);

\path [draw=black, thick]
(axis cs:8.2,32.928678406371)
--(axis cs:8.2,100.404654926962);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_9_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.82, xmax=8.42,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=445.455773378405,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,411.106220509766);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,413.813529379057);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,405.960052746498);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,414.344744481369);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,407.664535063296);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,409.918006802485);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,405.446181299816);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,407.834614390088);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,417.239298097495);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,nan);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,nan);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,nan);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,nan);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,nan);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,nan);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,nan);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,nan);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,nan);
\path [draw=black, thick]
(axis cs:-0.2,402.994594420072)
--(axis cs:-0.2,419.21784659946);

\path [draw=black, thick]
(axis cs:0.8,406.068976660008)
--(axis cs:0.8,421.558082098106);

\path [draw=black, thick]
(axis cs:1.8,397.129267206125)
--(axis cs:1.8,414.79083828687);

\path [draw=black, thick]
(axis cs:2.8,405.300868213837)
--(axis cs:2.8,423.388620748901);

\path [draw=black, thick]
(axis cs:3.8,397.845634542751)
--(axis cs:3.8,417.483435583841);

\path [draw=black, thick]
(axis cs:4.8,401.619079419646)
--(axis cs:4.8,418.216934185323);

\path [draw=black, thick]
(axis cs:5.8,396.917729142865)
--(axis cs:5.8,413.974633456767);

\path [draw=black, thick]
(axis cs:6.8,397.827119999288)
--(axis cs:6.8,417.842108780887);

\path [draw=black, thick]
(axis cs:7.8,410.23500250127)
--(axis cs:7.8,424.243593693719);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_9_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.84, xmax=8.84,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=211.544260466913,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,91.7255526315789);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,91.950863377193);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,89.7872432017544);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,93.9573563596491);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,97.3467423245614);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,94.5667328947368);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,99.3053877192983);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,93.5158949561404);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,91.7089824561403);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,126.666666666667);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,180);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,173.333333333333);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,53.3333333333333);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,146.666666666667);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,80);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,86.6666666666667);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,79.9994046052632);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,73.3333333333333);
\path [draw=black, thick]
(axis cs:-0.2,86.9320048920504)
--(axis cs:-0.2,96.5191003711075);

\path [draw=black, thick]
(axis cs:0.8,85.6632080301693)
--(axis cs:0.8,98.2385187242166);

\path [draw=black, thick]
(axis cs:1.8,82.8077820087686)
--(axis cs:1.8,96.7667043947401);

\path [draw=black, thick]
(axis cs:2.8,87.8650663310106)
--(axis cs:2.8,100.049646388288);

\path [draw=black, thick]
(axis cs:3.8,91.3831338046634)
--(axis cs:3.8,103.310350844459);

\path [draw=black, thick]
(axis cs:4.8,88.3231292106203)
--(axis cs:4.8,100.810336578853);

\path [draw=black, thick]
(axis cs:5.8,92.8338681144188)
--(axis cs:5.8,105.776907324178);

\path [draw=black, thick]
(axis cs:6.8,85.0688030542233)
--(axis cs:6.8,101.962986858057);

\path [draw=black, thick]
(axis cs:7.8,84.9927087487572)
--(axis cs:7.8,98.4252561635234);

\path [draw=black, thick]
(axis cs:0.2,92.1779266898977)
--(axis cs:0.2,161.155406643436);

\path [draw=black, thick]
(axis cs:1.2,158.529275745797)
--(axis cs:1.2,201.470724254203);

\path [draw=black, thick]
(axis cs:2.2,149.004524012634)
--(axis cs:2.2,197.662142654033);

\path [draw=black, thick]
(axis cs:3.2,21.6842949651676)
--(axis cs:3.2,84.9823717014991);

\path [draw=black, thick]
(axis cs:4.2,115.017628298501)
--(axis cs:4.2,178.315705034832);

\path [draw=black, thick]
(axis cs:5.2,44.9384541128033)
--(axis cs:5.2,115.061545887197);

\path [draw=black, thick]
(axis cs:6.2,51.2016374647007)
--(axis cs:6.2,122.131695868633);

\path [draw=black, thick]
(axis cs:7.2,44.9381196435128)
--(axis cs:7.2,115.060689567014);

\path [draw=black, thick]
(axis cs:8.2,38.8445933565643)
--(axis cs:8.2,107.822073310102);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_9_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.82, xmax=8.42,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=445.455773378405,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,411.106220509766);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,413.813529379057);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,405.960052746498);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,414.344744481369);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,407.664535063296);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,409.918006802485);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,405.446181299816);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,407.834614390088);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,417.239298097495);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,nan);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,nan);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,nan);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,nan);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,nan);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,nan);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,nan);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,nan);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,nan);
\path [draw=black, thick]
(axis cs:-0.2,402.994594420072)
--(axis cs:-0.2,419.21784659946);

\path [draw=black, thick]
(axis cs:0.8,406.068976660008)
--(axis cs:0.8,421.558082098106);

\path [draw=black, thick]
(axis cs:1.8,397.129267206125)
--(axis cs:1.8,414.79083828687);

\path [draw=black, thick]
(axis cs:2.8,405.300868213837)
--(axis cs:2.8,423.388620748901);

\path [draw=black, thick]
(axis cs:3.8,397.845634542751)
--(axis cs:3.8,417.483435583841);

\path [draw=black, thick]
(axis cs:4.8,401.619079419647)
--(axis cs:4.8,418.216934185323);

\path [draw=black, thick]
(axis cs:5.8,396.917729142865)
--(axis cs:5.8,413.974633456767);

\path [draw=black, thick]
(axis cs:6.8,397.827119999288)
--(axis cs:6.8,417.842108780887);

\path [draw=black, thick]
(axis cs:7.8,410.23500250127)
--(axis cs:7.8,424.243593693719);

\end{axis}

\end{tikzpicture}


==> img/200Mbps/numStas_9_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.84, xmax=8.84,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=207.545249786735,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,91.725552631579);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,91.950863377193);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,89.7872432017544);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,93.9573563596491);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,97.3467423245614);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,94.5667328947368);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,99.3053877192983);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,93.5158949561404);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,91.7089824561403);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,140);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,173.333333333333);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,173.333333333333);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,53.3333333333333);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,140);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,86.6666666666667);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,86.6666666666667);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,80);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,66.6666666666667);
\path [draw=black, thick]
(axis cs:-0.2,86.9320048920505)
--(axis cs:-0.2,96.5191003711075);

\path [draw=black, thick]
(axis cs:0.8,85.6632080301694)
--(axis cs:0.8,98.2385187242166);

\path [draw=black, thick]
(axis cs:1.8,82.8077820087686)
--(axis cs:1.8,96.7667043947401);

\path [draw=black, thick]
(axis cs:2.8,87.8650663310106)
--(axis cs:2.8,100.049646388288);

\path [draw=black, thick]
(axis cs:3.8,91.3831338046634)
--(axis cs:3.8,103.310350844459);

\path [draw=black, thick]
(axis cs:4.8,88.3231292106203)
--(axis cs:4.8,100.810336578853);

\path [draw=black, thick]
(axis cs:5.8,92.8338681144188)
--(axis cs:5.8,105.776907324178);

\path [draw=black, thick]
(axis cs:6.8,85.0688030542233)
--(axis cs:6.8,101.962986858057);

\path [draw=black, thick]
(axis cs:7.8,84.9927087487573)
--(axis cs:7.8,98.4252561635234);

\path [draw=black, thick]
(axis cs:0.2,107.202926959864)
--(axis cs:0.2,172.797073040136);

\path [draw=black, thick]
(axis cs:1.2,149.004524012634)
--(axis cs:1.2,197.662142654033);

\path [draw=black, thick]
(axis cs:2.2,149.004524012634)
--(axis cs:2.2,197.662142654033);

\path [draw=black, thick]
(axis cs:3.2,21.6842949651676)
--(axis cs:3.2,84.9823717014991);

\path [draw=black, thick]
(axis cs:4.2,107.202926959864)
--(axis cs:4.2,172.797073040136);

\path [draw=black, thick]
(axis cs:5.2,51.2016374647007)
--(axis cs:5.2,122.131695868633);

\path [draw=black, thick]
(axis cs:6.2,51.2016374647007)
--(axis cs:6.2,122.131695868633);

\path [draw=black, thick]
(axis cs:7.2,44.9384541128033)
--(axis cs:7.2,115.061545887197);

\path [draw=black, thick]
(axis cs:8.2,32.928678406371)
--(axis cs:8.2,100.404654926962);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_10_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.89, xmax=9.89,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9,STA 10},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=69.6610160635311,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,4.79490629712673);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,4.58197981150703);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,7.19512100402028);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,5.95575902110914);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,5.32693296114119);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,5.37869920589446);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,5.98662245720033);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,7.21472394296554);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,4.96401280288894);
\draw[draw=none,fill=color0] (axis cs:8.6,0) rectangle (axis cs:9,5.57183404171567);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,52.0869295835592);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,41.5915118468755);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,49.2880345101598);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,48.1817215043255);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,54.2070291359014);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,55.8359069676792);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,52.8161444117758);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,52.2782079602907);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,51.0024151056529);
\draw[draw=none,fill=color1] (axis cs:9,0) rectangle (axis cs:9.4,49.7949071021321);
\path [draw=black, thick]
(axis cs:-0.2,3.73631117045944)
--(axis cs:-0.2,5.85350142379402);

\path [draw=black, thick]
(axis cs:0.8,3.3526958697514)
--(axis cs:0.8,5.81126375326266);

\path [draw=black, thick]
(axis cs:1.8,5.54202778878562)
--(axis cs:1.8,8.84821421925494);

\path [draw=black, thick]
(axis cs:2.8,4.27525144328938)
--(axis cs:2.8,7.6362665989289);

\path [draw=black, thick]
(axis cs:3.8,4.1038198435279)
--(axis cs:3.8,6.55004607875449);

\path [draw=black, thick]
(axis cs:4.8,3.87443044112143)
--(axis cs:4.8,6.8829679706675);

\path [draw=black, thick]
(axis cs:5.8,4.78007748901187)
--(axis cs:5.8,7.19316742538878);

\path [draw=black, thick]
(axis cs:6.8,5.77804489235825)
--(axis cs:6.8,8.65140299357282);

\path [draw=black, thick]
(axis cs:7.8,3.79908680541409)
--(axis cs:7.8,6.12893880036378);

\path [draw=black, thick]
(axis cs:8.8,4.64339789278395)
--(axis cs:8.8,6.50027019064739);

\path [draw=black, thick]
(axis cs:0.2,41.4632179865696)
--(axis cs:0.2,62.7106411805489);

\path [draw=black, thick]
(axis cs:1.2,31.3438938972213)
--(axis cs:1.2,51.8391297965298);

\path [draw=black, thick]
(axis cs:2.2,40.3007054847172)
--(axis cs:2.2,58.2753635356024);

\path [draw=black, thick]
(axis cs:3.2,38.7084900066743)
--(axis cs:3.2,57.6549530019766);

\path [draw=black, thick]
(axis cs:4.2,43.1690480998908)
--(axis cs:4.2,65.2450101719119);

\path [draw=black, thick]
(axis cs:5.2,45.3279891129478)
--(axis cs:5.2,66.3438248224106);

\path [draw=black, thick]
(axis cs:6.2,42.6508112113464)
--(axis cs:6.2,62.9814776122052);

\path [draw=black, thick]
(axis cs:7.2,42.7446232317618)
--(axis cs:7.2,61.8117926888197);

\path [draw=black, thick]
(axis cs:8.2,41.1112828389664)
--(axis cs:8.2,60.8935473723395);

\path [draw=black, thick]
(axis cs:9.2,40.914528399765)
--(axis cs:9.2,58.6752858044991);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_10_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.89, xmax=9.89,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9,STA 10},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=52.5,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,50);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,50);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,50);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,50);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,50);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,50);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,50);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,50);
\draw[draw=none,fill=color0] (axis cs:8.6,0) rectangle (axis cs:9,50);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,50);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,50);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,50);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,50);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,50);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,50);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,50);
\draw[draw=none,fill=color1] (axis cs:9,0) rectangle (axis cs:9.4,50);
\path [draw=black, thick]
(axis cs:-0.2,50)
--(axis cs:-0.2,50);

\path [draw=black, thick]
(axis cs:0.8,50)
--(axis cs:0.8,50);

\path [draw=black, thick]
(axis cs:1.8,50)
--(axis cs:1.8,50);

\path [draw=black, thick]
(axis cs:2.8,50)
--(axis cs:2.8,50);

\path [draw=black, thick]
(axis cs:3.8,50)
--(axis cs:3.8,50);

\path [draw=black, thick]
(axis cs:4.8,50)
--(axis cs:4.8,50);

\path [draw=black, thick]
(axis cs:5.8,50)
--(axis cs:5.8,50);

\path [draw=black, thick]
(axis cs:6.8,50)
--(axis cs:6.8,50);

\path [draw=black, thick]
(axis cs:7.8,50)
--(axis cs:7.8,50);

\path [draw=black, thick]
(axis cs:8.8,50)
--(axis cs:8.8,50);

\path [draw=black, thick]
(axis cs:0.2,50)
--(axis cs:0.2,50);

\path [draw=black, thick]
(axis cs:1.2,50)
--(axis cs:1.2,50);

\path [draw=black, thick]
(axis cs:2.2,50)
--(axis cs:2.2,50);

\path [draw=black, thick]
(axis cs:3.2,50)
--(axis cs:3.2,50);

\path [draw=black, thick]
(axis cs:4.2,50)
--(axis cs:4.2,50);

\path [draw=black, thick]
(axis cs:5.2,50)
--(axis cs:5.2,50);

\path [draw=black, thick]
(axis cs:6.2,50)
--(axis cs:6.2,50);

\path [draw=black, thick]
(axis cs:7.2,50)
--(axis cs:7.2,50);

\path [draw=black, thick]
(axis cs:8.2,50)
--(axis cs:8.2,50);

\path [draw=black, thick]
(axis cs:9.2,50)
--(axis cs:9.2,50);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_10_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.89, xmax=9.89,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9,STA 10},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=27.6295631927538,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,4.79490629712673);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,4.58197981150703);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,7.19512100402028);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,5.95575902110914);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,5.3269329611412);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,5.37869920589446);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,5.98662245720033);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,7.21472394296554);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,4.96401280288894);
\draw[draw=none,fill=color0] (axis cs:8.6,0) rectangle (axis cs:9,5.57183404171567);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,20.7332269128068);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,13.7386899614497);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,12.593045178398);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,15.488171457925);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,17.8021968222187);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,11.7890683083067);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,16.0482238734992);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,16.2717956819044);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,12.5197156708154);
\draw[draw=none,fill=color1] (axis cs:9,0) rectangle (axis cs:9.4,16.4685927098339);
\path [draw=black, thick]
(axis cs:-0.2,3.73631117045944)
--(axis cs:-0.2,5.85350142379402);

\path [draw=black, thick]
(axis cs:0.8,3.3526958697514)
--(axis cs:0.8,5.81126375326266);

\path [draw=black, thick]
(axis cs:1.8,5.54202778878562)
--(axis cs:1.8,8.84821421925494);

\path [draw=black, thick]
(axis cs:2.8,4.27525144328938)
--(axis cs:2.8,7.6362665989289);

\path [draw=black, thick]
(axis cs:3.8,4.1038198435279)
--(axis cs:3.8,6.55004607875449);

\path [draw=black, thick]
(axis cs:4.8,3.87443044112143)
--(axis cs:4.8,6.8829679706675);

\path [draw=black, thick]
(axis cs:5.8,4.78007748901187)
--(axis cs:5.8,7.19316742538878);

\path [draw=black, thick]
(axis cs:6.8,5.77804489235825)
--(axis cs:6.8,8.65140299357282);

\path [draw=black, thick]
(axis cs:7.8,3.79908680541409)
--(axis cs:7.8,6.12893880036378);

\path [draw=black, thick]
(axis cs:8.8,4.64339789278395)
--(axis cs:8.8,6.50027019064739);

\path [draw=black, thick]
(axis cs:0.2,15.1525841182291)
--(axis cs:0.2,26.3138697073845);

\path [draw=black, thick]
(axis cs:1.2,10.5185882265598)
--(axis cs:1.2,16.9587916963396);

\path [draw=black, thick]
(axis cs:2.2,8.25004423503452)
--(axis cs:2.2,16.9360461217615);

\path [draw=black, thick]
(axis cs:3.2,11.4345626489922)
--(axis cs:3.2,19.5417802668578);

\path [draw=black, thick]
(axis cs:4.2,13.987060810122)
--(axis cs:4.2,21.6173328343154);

\path [draw=black, thick]
(axis cs:5.2,8.67562522774397)
--(axis cs:5.2,14.9025113888694);

\path [draw=black, thick]
(axis cs:6.2,11.3426458359349)
--(axis cs:6.2,20.7538019110634);

\path [draw=black, thick]
(axis cs:7.2,11.9565440350721)
--(axis cs:7.2,20.5870473287367);

\path [draw=black, thick]
(axis cs:8.2,9.24999226659106)
--(axis cs:8.2,15.7894390750398);

\path [draw=black, thick]
(axis cs:9.2,10.9189250281546)
--(axis cs:9.2,22.0182603915133);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_10_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.89, xmax=9.89,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9,STA 10},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=52.5003863751831,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,50);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,50);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,50);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,50);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,50);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,50);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,50);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,50);
\draw[draw=none,fill=color0] (axis cs:8.6,0) rectangle (axis cs:9,50);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,49.9996030701754);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,49.9998015350877);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,50);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,49.9998015350877);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,49.9998015350877);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,50);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,50);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,50);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,50);
\draw[draw=none,fill=color1] (axis cs:9,0) rectangle (axis cs:9.4,50);
\path [draw=black, thick]
(axis cs:-0.2,50)
--(axis cs:-0.2,50);

\path [draw=black, thick]
(axis cs:0.8,50)
--(axis cs:0.8,50);

\path [draw=black, thick]
(axis cs:1.8,50)
--(axis cs:1.8,50);

\path [draw=black, thick]
(axis cs:2.8,50)
--(axis cs:2.8,50);

\path [draw=black, thick]
(axis cs:3.8,50)
--(axis cs:3.8,50);

\path [draw=black, thick]
(axis cs:4.8,50)
--(axis cs:4.8,50);

\path [draw=black, thick]
(axis cs:5.8,50)
--(axis cs:5.8,50);

\path [draw=black, thick]
(axis cs:6.8,50)
--(axis cs:6.8,50);

\path [draw=black, thick]
(axis cs:7.8,50)
--(axis cs:7.8,50);

\path [draw=black, thick]
(axis cs:8.8,50)
--(axis cs:8.8,50);

\path [draw=black, thick]
(axis cs:0.2,49.998838163986)
--(axis cs:0.2,50.0003679763649);

\path [draw=black, thick]
(axis cs:1.2,49.999419081993)
--(axis cs:1.2,50.0001839881824);

\path [draw=black, thick]
(axis cs:2.2,50)
--(axis cs:2.2,50);

\path [draw=black, thick]
(axis cs:3.2,49.999419081993)
--(axis cs:3.2,50.0001839881824);

\path [draw=black, thick]
(axis cs:4.2,49.999419081993)
--(axis cs:4.2,50.0001839881824);

\path [draw=black, thick]
(axis cs:5.2,50)
--(axis cs:5.2,50);

\path [draw=black, thick]
(axis cs:6.2,50)
--(axis cs:6.2,50);

\path [draw=black, thick]
(axis cs:7.2,50)
--(axis cs:7.2,50);

\path [draw=black, thick]
(axis cs:8.2,50)
--(axis cs:8.2,50);

\path [draw=black, thick]
(axis cs:9.2,50)
--(axis cs:9.2,50);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_10_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.89, xmax=9.89,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9,STA 10},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=9.29062493021769,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,4.79490629712673);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,4.58197981150703);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,7.19512100402028);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,5.95575902110914);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,5.32693296114119);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,5.37869920589446);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,5.98662245720033);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,7.21472394296554);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,4.96401280288894);
\draw[draw=none,fill=color0] (axis cs:8.6,0) rectangle (axis cs:9,5.57183404171567);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,2.34033394673746);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,2.34117791111919);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,2.34161242842957);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,2.34041143037319);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,2.34139121808761);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,2.34099156163);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,2.34027443659999);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,2.34133246931591);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,2.3403390699645);
\draw[draw=none,fill=color1] (axis cs:9,0) rectangle (axis cs:9.4,2.34062768031222);
\path [draw=black, thick]
(axis cs:-0.2,3.73631117045944)
--(axis cs:-0.2,5.85350142379402);

\path [draw=black, thick]
(axis cs:0.8,3.3526958697514)
--(axis cs:0.8,5.81126375326266);

\path [draw=black, thick]
(axis cs:1.8,5.54202778878562)
--(axis cs:1.8,8.84821421925494);

\path [draw=black, thick]
(axis cs:2.8,4.27525144328939)
--(axis cs:2.8,7.6362665989289);

\path [draw=black, thick]
(axis cs:3.8,4.1038198435279)
--(axis cs:3.8,6.55004607875449);

\path [draw=black, thick]
(axis cs:4.8,3.87443044112143)
--(axis cs:4.8,6.8829679706675);

\path [draw=black, thick]
(axis cs:5.8,4.78007748901188)
--(axis cs:5.8,7.19316742538878);

\path [draw=black, thick]
(axis cs:6.8,5.77804489235825)
--(axis cs:6.8,8.65140299357282);

\path [draw=black, thick]
(axis cs:7.8,3.79908680541409)
--(axis cs:7.8,6.12893880036378);

\path [draw=black, thick]
(axis cs:8.8,4.64339789278395)
--(axis cs:8.8,6.50027019064739);

\path [draw=black, thick]
(axis cs:0.2,2.33983780919383)
--(axis cs:0.2,2.34083008428109);

\path [draw=black, thick]
(axis cs:1.2,2.34046986823287)
--(axis cs:1.2,2.34188595400551);

\path [draw=black, thick]
(axis cs:2.2,2.34093879174978)
--(axis cs:2.2,2.34228606510936);

\path [draw=black, thick]
(axis cs:3.2,2.33987072905793)
--(axis cs:3.2,2.34095213168844);

\path [draw=black, thick]
(axis cs:4.2,2.34072369185705)
--(axis cs:4.2,2.34205874431817);

\path [draw=black, thick]
(axis cs:5.2,2.3403003751732)
--(axis cs:5.2,2.34168274808681);

\path [draw=black, thick]
(axis cs:6.2,2.33982834075551)
--(axis cs:6.2,2.34072053244448);

\path [draw=black, thick]
(axis cs:7.2,2.34063997129306)
--(axis cs:7.2,2.34202496733875);

\path [draw=black, thick]
(axis cs:8.2,2.33990711414761)
--(axis cs:8.2,2.34077102578139);

\path [draw=black, thick]
(axis cs:9.2,2.3400695186585)
--(axis cs:9.2,2.34118584196594);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_10_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.89, xmax=9.89,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9,STA 10},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=52.5,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,50);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,50);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,50);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,50);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,50);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,50);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,50);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,50);
\draw[draw=none,fill=color0] (axis cs:8.6,0) rectangle (axis cs:9,50);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,50);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,50);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,50);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,50);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,50);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,50);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,50);
\draw[draw=none,fill=color1] (axis cs:9,0) rectangle (axis cs:9.4,50);
\path [draw=black, thick]
(axis cs:-0.2,50)
--(axis cs:-0.2,50);

\path [draw=black, thick]
(axis cs:0.8,50)
--(axis cs:0.8,50);

\path [draw=black, thick]
(axis cs:1.8,50)
--(axis cs:1.8,50);

\path [draw=black, thick]
(axis cs:2.8,50)
--(axis cs:2.8,50);

\path [draw=black, thick]
(axis cs:3.8,50)
--(axis cs:3.8,50);

\path [draw=black, thick]
(axis cs:4.8,50)
--(axis cs:4.8,50);

\path [draw=black, thick]
(axis cs:5.8,50)
--(axis cs:5.8,50);

\path [draw=black, thick]
(axis cs:6.8,50)
--(axis cs:6.8,50);

\path [draw=black, thick]
(axis cs:7.8,50)
--(axis cs:7.8,50);

\path [draw=black, thick]
(axis cs:8.8,50)
--(axis cs:8.8,50);

\path [draw=black, thick]
(axis cs:0.2,50)
--(axis cs:0.2,50);

\path [draw=black, thick]
(axis cs:1.2,50)
--(axis cs:1.2,50);

\path [draw=black, thick]
(axis cs:2.2,50)
--(axis cs:2.2,50);

\path [draw=black, thick]
(axis cs:3.2,50)
--(axis cs:3.2,50);

\path [draw=black, thick]
(axis cs:4.2,50)
--(axis cs:4.2,50);

\path [draw=black, thick]
(axis cs:5.2,50)
--(axis cs:5.2,50);

\path [draw=black, thick]
(axis cs:6.2,50)
--(axis cs:6.2,50);

\path [draw=black, thick]
(axis cs:7.2,50)
--(axis cs:7.2,50);

\path [draw=black, thick]
(axis cs:8.2,50)
--(axis cs:8.2,50);

\path [draw=black, thick]
(axis cs:9.2,50)
--(axis cs:9.2,50);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_1_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=0, xmax=1,
xtick style={color=black},
xtick={0},
xticklabels={STA 1},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=black},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0}
]
\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_1_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=0, xmax=1,
xtick style={color=black},
xtick={0},
xticklabels={STA 1},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=black},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0}
]
\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_1_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=0, xmax=1,
xtick style={color=black},
xtick={0},
xticklabels={STA 1},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=black},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0}
]
\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_1_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=0, xmax=1,
xtick style={color=black},
xtick={0},
xticklabels={STA 1},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=black},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0}
]
\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_1_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=0, xmax=1,
xtick style={color=black},
xtick={0},
xticklabels={STA 1},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=black},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0}
]
\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_1_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=0, xmax=1,
xtick style={color=black},
xtick={0},
xticklabels={STA 1},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=black},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0}
]
\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_2_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.49, xmax=1.49,
xtick style={color=black},
xtick={0,1},
xticklabels={STA 1,STA 2},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=57.7406129912208,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,3.4472165520793);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,3.74777078013208);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,38.6034707205301);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,44.9381172445061);
\path [draw=black, thick]
(axis cs:-0.2,2.81522942521755)
--(axis cs:-0.2,4.07920367894105);

\path [draw=black, thick]
(axis cs:0.8,2.97695676029092)
--(axis cs:0.8,4.51858479997324);

\path [draw=black, thick]
(axis cs:0.2,28.13663154087)
--(axis cs:0.2,49.0703099001902);

\path [draw=black, thick]
(axis cs:1.2,34.8851744973733)
--(axis cs:1.2,54.9910599916389);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_2_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.49, xmax=1.49,
xtick style={color=black},
xtick={0,1},
xticklabels={STA 1,STA 2},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=52.5,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,50);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50);
\path [draw=black, thick]
(axis cs:-0.2,50)
--(axis cs:-0.2,50);

\path [draw=black, thick]
(axis cs:0.8,50)
--(axis cs:0.8,50);

\path [draw=black, thick]
(axis cs:0.2,50)
--(axis cs:0.2,50);

\path [draw=black, thick]
(axis cs:1.2,50)
--(axis cs:1.2,50);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_2_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.49, xmax=1.49,
xtick style={color=black},
xtick={0,1},
xticklabels={STA 1,STA 2},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=5.12755463823951,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,3.4472165520793);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,3.74777078013208);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,4.03149987227844);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,3.83486050897792);
\path [draw=black, thick]
(axis cs:-0.2,2.81522942521755)
--(axis cs:-0.2,4.07920367894105);

\path [draw=black, thick]
(axis cs:0.8,2.97695676029092)
--(axis cs:0.8,4.51858479997324);

\path [draw=black, thick]
(axis cs:0.2,3.24606738805445)
--(axis cs:0.2,4.81693235650244);

\path [draw=black, thick]
(axis cs:1.2,2.78633564820393)
--(axis cs:1.2,4.88338536975191);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_2_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.49, xmax=1.49,
xtick style={color=black},
xtick={0,1},
xticklabels={STA 1,STA 2},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=52.5,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,50);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50);
\path [draw=black, thick]
(axis cs:-0.2,50)
--(axis cs:-0.2,50);

\path [draw=black, thick]
(axis cs:0.8,50)
--(axis cs:0.8,50);

\path [draw=black, thick]
(axis cs:0.2,50)
--(axis cs:0.2,50);

\path [draw=black, thick]
(axis cs:1.2,50)
--(axis cs:1.2,50);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_2_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.49, xmax=1.49,
xtick style={color=black},
xtick={0,1},
xticklabels={STA 1,STA 2},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=4.7445140399719,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,3.4472165520793);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,3.74777078013208);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,2.33971403519019);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,2.33978534597597);
\path [draw=black, thick]
(axis cs:-0.2,2.81522942521755)
--(axis cs:-0.2,4.07920367894105);

\path [draw=black, thick]
(axis cs:0.8,2.97695676029092)
--(axis cs:0.8,4.51858479997324);

\path [draw=black, thick]
(axis cs:0.2,2.33946907014856)
--(axis cs:0.2,2.33995900023182);

\path [draw=black, thick]
(axis cs:1.2,2.33954915981448)
--(axis cs:1.2,2.34002153213746);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_2_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.49, xmax=1.49,
xtick style={color=black},
xtick={0,1},
xticklabels={STA 1,STA 2},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=52.5,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,50);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50);
\path [draw=black, thick]
(axis cs:-0.2,50)
--(axis cs:-0.2,50);

\path [draw=black, thick]
(axis cs:0.8,50)
--(axis cs:0.8,50);

\path [draw=black, thick]
(axis cs:0.2,50)
--(axis cs:0.2,50);

\path [draw=black, thick]
(axis cs:1.2,50)
--(axis cs:1.2,50);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_3_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.54, xmax=2.54,
xtick style={color=black},
xtick={0,1,2},
xticklabels={STA 1,STA 2,STA 3},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=68.5327590529892,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,3.49753216314627);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,3.48567840476925);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,3.64271465651559);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,54.7063566694564);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,51.268344209296);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,44.8082328902098);
\path [draw=black, thick]
(axis cs:-0.2,2.77037221029406)
--(axis cs:-0.2,4.22469211599847);

\path [draw=black, thick]
(axis cs:0.8,2.77745167578429)
--(axis cs:0.8,4.19390513375421);

\path [draw=black, thick]
(axis cs:1.8,2.99012372938727)
--(axis cs:1.8,4.2953055836439);

\path [draw=black, thick]
(axis cs:0.2,44.1434190027325)
--(axis cs:0.2,65.2692943361802);

\path [draw=black, thick]
(axis cs:1.2,41.4973738321401)
--(axis cs:1.2,61.0393145864519);

\path [draw=black, thick]
(axis cs:2.2,36.0369227707146)
--(axis cs:2.2,53.5795430097051);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_3_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.5,0.09)}, anchor=south, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.54, xmax=2.54,
xtick style={color=black},
xtick={0,1,2},
xticklabels={STA 1,STA 2,STA 3},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=52.5,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,50);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,50);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,50);
\path [draw=black, thick]
(axis cs:-0.2,50)
--(axis cs:-0.2,50);

\path [draw=black, thick]
(axis cs:0.8,50)
--(axis cs:0.8,50);

\path [draw=black, thick]
(axis cs:1.8,50)
--(axis cs:1.8,50);

\path [draw=black, thick]
(axis cs:0.2,50)
--(axis cs:0.2,50);

\path [draw=black, thick]
(axis cs:1.2,50)
--(axis cs:1.2,50);

\path [draw=black, thick]
(axis cs:2.2,50)
--(axis cs:2.2,50);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_3_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.54, xmax=2.54,
xtick style={color=black},
xtick={0,1,2},
xticklabels={STA 1,STA 2,STA 3},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=6.44160480803018,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,3.49753216314627);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,3.48567840476925);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,3.64271465651559);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,3.97191727718916);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,4.38403359030741);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,4.62779333173164);
\path [draw=black, thick]
(axis cs:-0.2,2.77037221029406)
--(axis cs:-0.2,4.22469211599847);

\path [draw=black, thick]
(axis cs:0.8,2.77745167578429)
--(axis cs:0.8,4.19390513375421);

\path [draw=black, thick]
(axis cs:1.8,2.99012372938727)
--(axis cs:1.8,4.2953055836439);

\path [draw=black, thick]
(axis cs:0.2,3.18537239270433)
--(axis cs:0.2,4.75846216167398);

\path [draw=black, thick]
(axis cs:1.2,2.8863197681184)
--(axis cs:1.2,5.88174741249643);

\path [draw=black, thick]
(axis cs:2.2,3.12072494152978)
--(axis cs:2.2,6.1348617219335);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_3_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.5,0.09)}, anchor=south, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.54, xmax=2.54,
xtick style={color=black},
xtick={0,1,2},
xticklabels={STA 1,STA 2,STA 3},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=52.5,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,50);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,50);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,50);
\path [draw=black, thick]
(axis cs:-0.2,50)
--(axis cs:-0.2,50);

\path [draw=black, thick]
(axis cs:0.8,50)
--(axis cs:0.8,50);

\path [draw=black, thick]
(axis cs:1.8,50)
--(axis cs:1.8,50);

\path [draw=black, thick]
(axis cs:0.2,50)
--(axis cs:0.2,50);

\path [draw=black, thick]
(axis cs:1.2,50)
--(axis cs:1.2,50);

\path [draw=black, thick]
(axis cs:2.2,50)
--(axis cs:2.2,50);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_3_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.54, xmax=2.54,
xtick style={color=black},
xtick={0,1,2},
xticklabels={STA 1,STA 2,STA 3},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=4.51007086282609,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,3.49753216314627);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,3.48567840476925);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,3.64271465651559);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,2.34003955182773);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,2.3403955015137);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,2.34009232744632);
\path [draw=black, thick]
(axis cs:-0.2,2.77037221029406)
--(axis cs:-0.2,4.22469211599847);

\path [draw=black, thick]
(axis cs:0.8,2.77745167578429)
--(axis cs:0.8,4.19390513375421);

\path [draw=black, thick]
(axis cs:1.8,2.99012372938727)
--(axis cs:1.8,4.2953055836439);

\path [draw=black, thick]
(axis cs:0.2,2.33957375542596)
--(axis cs:0.2,2.34050534822951);

\path [draw=black, thick]
(axis cs:1.2,2.3400176810027)
--(axis cs:1.2,2.34077332202469);

\path [draw=black, thick]
(axis cs:2.2,2.3397689957499)
--(axis cs:2.2,2.34041565914274);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_3_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.5,0.09)}, anchor=south, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.54, xmax=2.54,
xtick style={color=black},
xtick={0,1,2},
xticklabels={STA 1,STA 2,STA 3},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=52.5,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,50);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,50);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,50);
\path [draw=black, thick]
(axis cs:-0.2,50)
--(axis cs:-0.2,50);

\path [draw=black, thick]
(axis cs:0.8,50)
--(axis cs:0.8,50);

\path [draw=black, thick]
(axis cs:1.8,50)
--(axis cs:1.8,50);

\path [draw=black, thick]
(axis cs:0.2,50)
--(axis cs:0.2,50);

\path [draw=black, thick]
(axis cs:1.2,50)
--(axis cs:1.2,50);

\path [draw=black, thick]
(axis cs:2.2,50)
--(axis cs:2.2,50);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_4_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=73.361572988889,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,3.36014486625553);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,3.17791780074691);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,3.07855089915369);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,3.45356708539573);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,53.7818558320064);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,48.2051972682594);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,51.7663138008411);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,59.7421016124859);
\path [draw=black, thick]
(axis cs:-0.2,2.92176708341157)
--(axis cs:-0.2,3.79852264909948);

\path [draw=black, thick]
(axis cs:0.8,2.62632603895128)
--(axis cs:0.8,3.72950956254254);

\path [draw=black, thick]
(axis cs:1.8,2.63435790095709)
--(axis cs:1.8,3.52274389735028);

\path [draw=black, thick]
(axis cs:2.8,2.77222155410035)
--(axis cs:2.8,4.1349126166911);

\path [draw=black, thick]
(axis cs:0.2,44.2841556334402)
--(axis cs:0.2,63.2795560305726);

\path [draw=black, thick]
(axis cs:1.2,38.4385098534948)
--(axis cs:1.2,57.9718846830239);

\path [draw=black, thick]
(axis cs:2.2,41.6486120311121)
--(axis cs:2.2,61.8840155705701);

\path [draw=black, thick]
(axis cs:3.2,49.616038473649)
--(axis cs:3.2,69.8681647513228);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_4_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=52.5,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,50);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,50);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,50);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,50);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,50);
\path [draw=black, thick]
(axis cs:-0.2,50)
--(axis cs:-0.2,50);

\path [draw=black, thick]
(axis cs:0.8,50)
--(axis cs:0.8,50);

\path [draw=black, thick]
(axis cs:1.8,50)
--(axis cs:1.8,50);

\path [draw=black, thick]
(axis cs:2.8,50)
--(axis cs:2.8,50);

\path [draw=black, thick]
(axis cs:0.2,50)
--(axis cs:0.2,50);

\path [draw=black, thick]
(axis cs:1.2,50)
--(axis cs:1.2,50);

\path [draw=black, thick]
(axis cs:2.2,50)
--(axis cs:2.2,50);

\path [draw=black, thick]
(axis cs:3.2,50)
--(axis cs:3.2,50);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_4_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=7.24699649415536,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,3.36014486625553);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,3.17791780074691);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,3.07855089915369);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,3.45356708539573);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,3.93919282141519);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,5.10569578217961);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,5.05903377775548);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,5.24197634189122);
\path [draw=black, thick]
(axis cs:-0.2,2.92176708341157)
--(axis cs:-0.2,3.79852264909948);

\path [draw=black, thick]
(axis cs:0.8,2.62632603895128)
--(axis cs:0.8,3.72950956254254);

\path [draw=black, thick]
(axis cs:1.8,2.63435790095709)
--(axis cs:1.8,3.52274389735028);

\path [draw=black, thick]
(axis cs:2.8,2.77222155410035)
--(axis cs:2.8,4.1349126166911);

\path [draw=black, thick]
(axis cs:0.2,2.9101197433509)
--(axis cs:0.2,4.96826589947949);

\path [draw=black, thick]
(axis cs:1.2,3.40195022131303)
--(axis cs:1.2,6.8094413430462);

\path [draw=black, thick]
(axis cs:2.2,3.55800040141684)
--(axis cs:2.2,6.56006715409411);

\path [draw=black, thick]
(axis cs:3.2,3.58205126077733)
--(axis cs:3.2,6.9019014230051);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_4_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=52.5,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,50);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,50);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,50);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,50);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,50);
\path [draw=black, thick]
(axis cs:-0.2,50)
--(axis cs:-0.2,50);

\path [draw=black, thick]
(axis cs:0.8,50)
--(axis cs:0.8,50);

\path [draw=black, thick]
(axis cs:1.8,50)
--(axis cs:1.8,50);

\path [draw=black, thick]
(axis cs:2.8,50)
--(axis cs:2.8,50);

\path [draw=black, thick]
(axis cs:0.2,50)
--(axis cs:0.2,50);

\path [draw=black, thick]
(axis cs:1.2,50)
--(axis cs:1.2,50);

\path [draw=black, thick]
(axis cs:2.2,50)
--(axis cs:2.2,50);

\path [draw=black, thick]
(axis cs:3.2,50)
--(axis cs:3.2,50);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_4_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=4.34165824752566,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,3.36014486625553);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,3.17791780074691);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,3.07855089915369);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,3.45356708539573);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,2.34042771827586);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,2.34030546252906);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,2.34092109753028);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,2.34055285668242);
\path [draw=black, thick]
(axis cs:-0.2,2.92176708341157)
--(axis cs:-0.2,3.79852264909948);

\path [draw=black, thick]
(axis cs:0.8,2.62632603895128)
--(axis cs:0.8,3.72950956254254);

\path [draw=black, thick]
(axis cs:1.8,2.63435790095709)
--(axis cs:1.8,3.52274389735028);

\path [draw=black, thick]
(axis cs:2.8,2.77222155410035)
--(axis cs:2.8,4.1349126166911);

\path [draw=black, thick]
(axis cs:0.2,2.33986590791938)
--(axis cs:0.2,2.34098952863234);

\path [draw=black, thick]
(axis cs:1.2,2.33990898922657)
--(axis cs:1.2,2.34070193583156);

\path [draw=black, thick]
(axis cs:2.2,2.34043053734084)
--(axis cs:2.2,2.34141165771971);

\path [draw=black, thick]
(axis cs:3.2,2.33997768223665)
--(axis cs:3.2,2.34112803112819);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_4_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=52.5,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,50);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,50);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,50);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,50);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,50);
\path [draw=black, thick]
(axis cs:-0.2,50)
--(axis cs:-0.2,50);

\path [draw=black, thick]
(axis cs:0.8,50)
--(axis cs:0.8,50);

\path [draw=black, thick]
(axis cs:1.8,50)
--(axis cs:1.8,50);

\path [draw=black, thick]
(axis cs:2.8,50)
--(axis cs:2.8,50);

\path [draw=black, thick]
(axis cs:0.2,50)
--(axis cs:0.2,50);

\path [draw=black, thick]
(axis cs:1.2,50)
--(axis cs:1.2,50);

\path [draw=black, thick]
(axis cs:2.2,50)
--(axis cs:2.2,50);

\path [draw=black, thick]
(axis cs:3.2,50)
--(axis cs:3.2,50);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_5_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.64, xmax=4.64,
xtick style={color=black},
xtick={0,1,2,3,4},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=65.9311245073991,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,4.0761480995238);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,3.37226221494105);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,3.06616299606957);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,3.00861064196409);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,3.25716533071819);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,36.9686581028889);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50.6036936711983);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,53.8386393104495);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,48.705006411217);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,49.8579388670593);
\path [draw=black, thick]
(axis cs:-0.2,3.24168107635967)
--(axis cs:-0.2,4.91061512268793);

\path [draw=black, thick]
(axis cs:0.8,2.70759250507401)
--(axis cs:0.8,4.03693192480809);

\path [draw=black, thick]
(axis cs:1.8,2.57161806875553)
--(axis cs:1.8,3.56070792338361);

\path [draw=black, thick]
(axis cs:2.8,2.65595146878654)
--(axis cs:2.8,3.36126981514165);

\path [draw=black, thick]
(axis cs:3.8,2.7324678461571)
--(axis cs:3.8,3.78186281527927);

\path [draw=black, thick]
(axis cs:0.2,27.7352860167264)
--(axis cs:0.2,46.2020301890513);

\path [draw=black, thick]
(axis cs:1.2,40.9939303289329)
--(axis cs:1.2,60.2134570134637);

\path [draw=black, thick]
(axis cs:2.2,44.8857314709951)
--(axis cs:2.2,62.7915471499039);

\path [draw=black, thick]
(axis cs:3.2,38.106340531633)
--(axis cs:3.2,59.3036722908009);

\path [draw=black, thick]
(axis cs:4.2,39.2286912373122)
--(axis cs:4.2,60.4871864968063);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_5_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.64, xmax=4.64,
xtick style={color=black},
xtick={0,1,2,3,4},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=52.5,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,50);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,50);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,50);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,50);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,50);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,50);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,50);
\path [draw=black, thick]
(axis cs:-0.2,50)
--(axis cs:-0.2,50);

\path [draw=black, thick]
(axis cs:0.8,50)
--(axis cs:0.8,50);

\path [draw=black, thick]
(axis cs:1.8,50)
--(axis cs:1.8,50);

\path [draw=black, thick]
(axis cs:2.8,50)
--(axis cs:2.8,50);

\path [draw=black, thick]
(axis cs:3.8,50)
--(axis cs:3.8,50);

\path [draw=black, thick]
(axis cs:0.2,50)
--(axis cs:0.2,50);

\path [draw=black, thick]
(axis cs:1.2,50)
--(axis cs:1.2,50);

\path [draw=black, thick]
(axis cs:2.2,50)
--(axis cs:2.2,50);

\path [draw=black, thick]
(axis cs:3.2,50)
--(axis cs:3.2,50);

\path [draw=black, thick]
(axis cs:4.2,50)
--(axis cs:4.2,50);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_5_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.64, xmax=4.64,
xtick style={color=black},
xtick={0,1,2,3,4},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=9.86883045773891,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,4.0761480995238);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,3.37743897627438);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,3.06856843360803);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,3.00862179283598);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,3.25716533071819);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,5.61513505300763);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,7.09250115008769);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,4.77425575087569);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,6.70525189095644);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,5.57792302442676);
\path [draw=black, thick]
(axis cs:-0.2,3.24168107635967)
--(axis cs:-0.2,4.91061512268793);

\path [draw=black, thick]
(axis cs:0.8,2.71301586347752)
--(axis cs:0.8,4.04186208907124);

\path [draw=black, thick]
(axis cs:1.8,2.57438015244928)
--(axis cs:1.8,3.56275671476679);

\path [draw=black, thick]
(axis cs:2.8,2.65596485237469)
--(axis cs:2.8,3.36127873329727);

\path [draw=black, thick]
(axis cs:3.8,2.7324678461571)
--(axis cs:3.8,3.78186281527927);

\path [draw=black, thick]
(axis cs:0.2,3.99489563015598)
--(axis cs:0.2,7.23537447585928);

\path [draw=black, thick]
(axis cs:1.2,4.78611614994785)
--(axis cs:1.2,9.39888615022754);

\path [draw=black, thick]
(axis cs:2.2,3.50264612481076)
--(axis cs:2.2,6.04586537694061);

\path [draw=black, thick]
(axis cs:3.2,4.7360743109021)
--(axis cs:3.2,8.67442947101077);

\path [draw=black, thick]
(axis cs:4.2,3.68618820918595)
--(axis cs:4.2,7.46965783966757);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_5_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.64, xmax=4.64,
xtick style={color=black},
xtick={0,1,2,3,4},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=52.5,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,50);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,50);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,50);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,50);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,50);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,50);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,50);
\path [draw=black, thick]
(axis cs:-0.2,50)
--(axis cs:-0.2,50);

\path [draw=black, thick]
(axis cs:0.8,50)
--(axis cs:0.8,50);

\path [draw=black, thick]
(axis cs:1.8,50)
--(axis cs:1.8,50);

\path [draw=black, thick]
(axis cs:2.8,50)
--(axis cs:2.8,50);

\path [draw=black, thick]
(axis cs:3.8,50)
--(axis cs:3.8,50);

\path [draw=black, thick]
(axis cs:0.2,50)
--(axis cs:0.2,50);

\path [draw=black, thick]
(axis cs:1.2,50)
--(axis cs:1.2,50);

\path [draw=black, thick]
(axis cs:2.2,50)
--(axis cs:2.2,50);

\path [draw=black, thick]
(axis cs:3.2,50)
--(axis cs:3.2,50);

\path [draw=black, thick]
(axis cs:4.2,50)
--(axis cs:4.2,50);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_5_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.64, xmax=4.64,
xtick style={color=black},
xtick={0,1,2,3,4},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=5.15614587882232,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,4.0761480995238);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,3.37743897627438);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,3.06856843360803);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,3.00862179283598);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,3.25716533071819);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,2.34056050879621);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,2.34091047021395);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,2.34090668659685);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,2.34018736545892);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,2.34009120343651);
\path [draw=black, thick]
(axis cs:-0.2,3.24168107635967)
--(axis cs:-0.2,4.91061512268793);

\path [draw=black, thick]
(axis cs:0.8,2.71301586347752)
--(axis cs:0.8,4.04186208907124);

\path [draw=black, thick]
(axis cs:1.8,2.57438015244928)
--(axis cs:1.8,3.56275671476679);

\path [draw=black, thick]
(axis cs:2.8,2.65596485237469)
--(axis cs:2.8,3.36127873329728);

\path [draw=black, thick]
(axis cs:3.8,2.7324678461571)
--(axis cs:3.8,3.78186281527927);

\path [draw=black, thick]
(axis cs:0.2,2.34000060513563)
--(axis cs:0.2,2.34112041245679);

\path [draw=black, thick]
(axis cs:1.2,2.34034652631956)
--(axis cs:1.2,2.34147441410835);

\path [draw=black, thick]
(axis cs:2.2,2.34035234764732)
--(axis cs:2.2,2.34146102554638);

\path [draw=black, thick]
(axis cs:3.2,2.33967701206763)
--(axis cs:3.2,2.3406977188502);

\path [draw=black, thick]
(axis cs:4.2,2.33961333304135)
--(axis cs:4.2,2.34056907383166);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_5_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.64, xmax=4.64,
xtick style={color=black},
xtick={0,1,2,3,4},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=52.5,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,50);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,50);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,50);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,50);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,50);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,50);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,50);
\path [draw=black, thick]
(axis cs:-0.2,50)
--(axis cs:-0.2,50);

\path [draw=black, thick]
(axis cs:0.8,50)
--(axis cs:0.8,50);

\path [draw=black, thick]
(axis cs:1.8,50)
--(axis cs:1.8,50);

\path [draw=black, thick]
(axis cs:2.8,50)
--(axis cs:2.8,50);

\path [draw=black, thick]
(axis cs:3.8,50)
--(axis cs:3.8,50);

\path [draw=black, thick]
(axis cs:0.2,50)
--(axis cs:0.2,50);

\path [draw=black, thick]
(axis cs:1.2,50)
--(axis cs:1.2,50);

\path [draw=black, thick]
(axis cs:2.2,50)
--(axis cs:2.2,50);

\path [draw=black, thick]
(axis cs:3.2,50)
--(axis cs:3.2,50);

\path [draw=black, thick]
(axis cs:4.2,50)
--(axis cs:4.2,50);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_6_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.69, xmax=5.69,
xtick style={color=black},
xtick={0,1,2,3,4,5},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=67.3021861740163,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,4.08928720434338);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,3.2391762385042);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,3.36926106268876);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,3.97667039535629);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,3.20331952941701);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,3.78662778789223);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,39.3194923562726);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,49.6652988425184);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,51.7969260761264);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,54.126723312796);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,39.1470854960417);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,53.613912760174);
\path [draw=black, thick]
(axis cs:-0.2,3.03942475087042)
--(axis cs:-0.2,5.13914965781634);

\path [draw=black, thick]
(axis cs:0.8,2.71988803181695)
--(axis cs:0.8,3.75846444519146);

\path [draw=black, thick]
(axis cs:1.8,2.74230122667199)
--(axis cs:1.8,3.99622089870552);

\path [draw=black, thick]
(axis cs:2.8,2.79655706751758)
--(axis cs:2.8,5.15678372319501);

\path [draw=black, thick]
(axis cs:3.8,2.47747436075243)
--(axis cs:3.8,3.92916469808159);

\path [draw=black, thick]
(axis cs:4.8,2.63377738288034)
--(axis cs:4.8,4.93947819290412);

\path [draw=black, thick]
(axis cs:0.2,31.6166169866507)
--(axis cs:0.2,47.0223677258944);

\path [draw=black, thick]
(axis cs:1.2,40.252559059371)
--(axis cs:1.2,59.0780386256658);

\path [draw=black, thick]
(axis cs:2.2,42.0158435082305)
--(axis cs:2.2,61.5780086440222);

\path [draw=black, thick]
(axis cs:3.2,44.1561264598623)
--(axis cs:3.2,64.0973201657298);

\path [draw=black, thick]
(axis cs:4.2,30.3398838117393)
--(axis cs:4.2,47.9542871803442);

\path [draw=black, thick]
(axis cs:5.2,44.3712015113374)
--(axis cs:5.2,62.8566240090105);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_6_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.69, xmax=5.69,
xtick style={color=black},
xtick={0,1,2,3,4,5},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=52.5,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,50);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,50);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,50);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,50);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,50);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,50);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,50);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,50);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,50);
\path [draw=black, thick]
(axis cs:-0.2,50)
--(axis cs:-0.2,50);

\path [draw=black, thick]
(axis cs:0.8,50)
--(axis cs:0.8,50);

\path [draw=black, thick]
(axis cs:1.8,50)
--(axis cs:1.8,50);

\path [draw=black, thick]
(axis cs:2.8,50)
--(axis cs:2.8,50);

\path [draw=black, thick]
(axis cs:3.8,50)
--(axis cs:3.8,50);

\path [draw=black, thick]
(axis cs:4.8,50)
--(axis cs:4.8,50);

\path [draw=black, thick]
(axis cs:0.2,50)
--(axis cs:0.2,50);

\path [draw=black, thick]
(axis cs:1.2,50)
--(axis cs:1.2,50);

\path [draw=black, thick]
(axis cs:2.2,50)
--(axis cs:2.2,50);

\path [draw=black, thick]
(axis cs:3.2,50)
--(axis cs:3.2,50);

\path [draw=black, thick]
(axis cs:4.2,50)
--(axis cs:4.2,50);

\path [draw=black, thick]
(axis cs:5.2,50)
--(axis cs:5.2,50);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_6_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.69, xmax=5.69,
xtick style={color=black},
xtick={0,1,2,3,4,5},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=13.7391387391145,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,4.08928720434338);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,3.23896820121537);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,3.38586403692103);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,3.97665199801722);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,3.20331952941701);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,3.78662778789223);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,4.42323741528504);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,6.91564381540632);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,7.43264077821921);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,6.33243072545427);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,9.87607002104304);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,5.7592214011867);
\path [draw=black, thick]
(axis cs:-0.2,3.03942475087042)
--(axis cs:-0.2,5.13914965781634);

\path [draw=black, thick]
(axis cs:0.8,2.71989303316242)
--(axis cs:0.8,3.75804336926831);

\path [draw=black, thick]
(axis cs:1.8,2.76120684917021)
--(axis cs:1.8,4.01052122467186);

\path [draw=black, thick]
(axis cs:2.8,2.79653562494558)
--(axis cs:2.8,5.15676837108886);

\path [draw=black, thick]
(axis cs:3.8,2.47747436075243)
--(axis cs:3.8,3.92916469808159);

\path [draw=black, thick]
(axis cs:4.8,2.63377738288034)
--(axis cs:4.8,4.93947819290412);

\path [draw=black, thick]
(axis cs:0.2,3.36070783004223)
--(axis cs:0.2,5.48576700052785);

\path [draw=black, thick]
(axis cs:1.2,4.60579667509465)
--(axis cs:1.2,9.22549095571799);

\path [draw=black, thick]
(axis cs:2.2,4.95176010904541)
--(axis cs:2.2,9.913521447393);

\path [draw=black, thick]
(axis cs:3.2,4.23528974783402)
--(axis cs:3.2,8.42957170307451);

\path [draw=black, thick]
(axis cs:4.2,6.66724600483422)
--(axis cs:4.2,13.0848940372519);

\path [draw=black, thick]
(axis cs:5.2,3.59555099460805)
--(axis cs:5.2,7.92289180776534);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_6_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.69, xmax=5.69,
xtick style={color=black},
xtick={0,1,2,3,4,5},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=52.5,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,50);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,50);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,50);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,50);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,50);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,50);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,50);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,50);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,50);
\path [draw=black, thick]
(axis cs:-0.2,50)
--(axis cs:-0.2,50);

\path [draw=black, thick]
(axis cs:0.8,50)
--(axis cs:0.8,50);

\path [draw=black, thick]
(axis cs:1.8,50)
--(axis cs:1.8,50);

\path [draw=black, thick]
(axis cs:2.8,50)
--(axis cs:2.8,50);

\path [draw=black, thick]
(axis cs:3.8,50)
--(axis cs:3.8,50);

\path [draw=black, thick]
(axis cs:4.8,50)
--(axis cs:4.8,50);

\path [draw=black, thick]
(axis cs:0.2,50)
--(axis cs:0.2,50);

\path [draw=black, thick]
(axis cs:1.2,50)
--(axis cs:1.2,50);

\path [draw=black, thick]
(axis cs:2.2,50)
--(axis cs:2.2,50);

\path [draw=black, thick]
(axis cs:3.2,50)
--(axis cs:3.2,50);

\path [draw=black, thick]
(axis cs:4.2,50)
--(axis cs:4.2,50);

\path [draw=black, thick]
(axis cs:5.2,50)
--(axis cs:5.2,50);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_6_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.69, xmax=5.69,
xtick style={color=black},
xtick={0,1,2,3,4,5},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=5.4146067896433,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,4.08928720434338);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,3.23896820121537);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,3.38586403692103);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,3.97665199801722);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,3.20331952941701);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,3.78662778789223);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,2.34104934755574);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,2.34062751091981);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,2.34064324094341);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,2.34123707368335);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,2.34035912261722);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,2.34073922302971);
\path [draw=black, thick]
(axis cs:-0.2,3.03942475087042)
--(axis cs:-0.2,5.13914965781634);

\path [draw=black, thick]
(axis cs:0.8,2.71989303316242)
--(axis cs:0.8,3.75804336926831);

\path [draw=black, thick]
(axis cs:1.8,2.76120684917021)
--(axis cs:1.8,4.01052122467186);

\path [draw=black, thick]
(axis cs:2.8,2.79653562494558)
--(axis cs:2.8,5.15676837108886);

\path [draw=black, thick]
(axis cs:3.8,2.47747436075243)
--(axis cs:3.8,3.92916469808159);

\path [draw=black, thick]
(axis cs:4.8,2.63377738288034)
--(axis cs:4.8,4.93947819290412);

\path [draw=black, thick]
(axis cs:0.2,2.3402148370069)
--(axis cs:0.2,2.34188385810458);

\path [draw=black, thick]
(axis cs:1.2,2.34004508156956)
--(axis cs:1.2,2.34120994027006);

\path [draw=black, thick]
(axis cs:2.2,2.34022576215223)
--(axis cs:2.2,2.34106071973459);

\path [draw=black, thick]
(axis cs:3.2,2.34070197085414)
--(axis cs:3.2,2.34177217651257);

\path [draw=black, thick]
(axis cs:4.2,2.3398632201723)
--(axis cs:4.2,2.34085502506213);

\path [draw=black, thick]
(axis cs:5.2,2.33992761937151)
--(axis cs:5.2,2.34155082668791);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_6_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.69, xmax=5.69,
xtick style={color=black},
xtick={0,1,2,3,4,5},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=52.5,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,50);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,50);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,50);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,50);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,50);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,50);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,50);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,50);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,50);
\path [draw=black, thick]
(axis cs:-0.2,50)
--(axis cs:-0.2,50);

\path [draw=black, thick]
(axis cs:0.8,50)
--(axis cs:0.8,50);

\path [draw=black, thick]
(axis cs:1.8,50)
--(axis cs:1.8,50);

\path [draw=black, thick]
(axis cs:2.8,50)
--(axis cs:2.8,50);

\path [draw=black, thick]
(axis cs:3.8,50)
--(axis cs:3.8,50);

\path [draw=black, thick]
(axis cs:4.8,50)
--(axis cs:4.8,50);

\path [draw=black, thick]
(axis cs:0.2,50)
--(axis cs:0.2,50);

\path [draw=black, thick]
(axis cs:1.2,50)
--(axis cs:1.2,50);

\path [draw=black, thick]
(axis cs:2.2,50)
--(axis cs:2.2,50);

\path [draw=black, thick]
(axis cs:3.2,50)
--(axis cs:3.2,50);

\path [draw=black, thick]
(axis cs:4.2,50)
--(axis cs:4.2,50);

\path [draw=black, thick]
(axis cs:5.2,50)
--(axis cs:5.2,50);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_7_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.74, xmax=6.74,
xtick style={color=black},
xtick={0,1,2,3,4,5,6},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=71.4804577568803,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,4.01588299969641);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,3.94562238644543);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,3.93251387947485);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,3.0987437382559);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,4.82596556981851);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,4.75643161148832);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,4.16225624870128);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,46.0214893789795);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,46.9767444781429);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,50.2164182026155);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,50.8885934951773);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,53.4660084439594);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,58.6638168714751);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,48.6742020203774);
\path [draw=black, thick]
(axis cs:-0.2,3.22379032910066)
--(axis cs:-0.2,4.80797567029217);

\path [draw=black, thick]
(axis cs:0.8,3.05936801533163)
--(axis cs:0.8,4.83187675755923);

\path [draw=black, thick]
(axis cs:1.8,2.93400262772663)
--(axis cs:1.8,4.93102513122306);

\path [draw=black, thick]
(axis cs:2.8,2.70959038227014)
--(axis cs:2.8,3.48789709424166);

\path [draw=black, thick]
(axis cs:3.8,3.31305444891085)
--(axis cs:3.8,6.33887669072617);

\path [draw=black, thick]
(axis cs:4.8,3.60177677939245)
--(axis cs:4.8,5.91108644358418);

\path [draw=black, thick]
(axis cs:5.8,3.10713354727829)
--(axis cs:5.8,5.21737895012428);

\path [draw=black, thick]
(axis cs:0.2,36.6737684485439)
--(axis cs:0.2,55.3692103094151);

\path [draw=black, thick]
(axis cs:1.2,37.8999418200345)
--(axis cs:1.2,56.0535471362513);

\path [draw=black, thick]
(axis cs:2.2,38.8487183689525)
--(axis cs:2.2,61.5841180362785);

\path [draw=black, thick]
(axis cs:3.2,40.4072614167264)
--(axis cs:3.2,61.3699255736282);

\path [draw=black, thick]
(axis cs:4.2,42.8562245755058)
--(axis cs:4.2,64.075792312413);

\path [draw=black, thick]
(axis cs:5.2,49.2510073078262)
--(axis cs:5.2,68.0766264351241);

\path [draw=black, thick]
(axis cs:6.2,38.5652628761247)
--(axis cs:6.2,58.7831411646301);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_7_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.74, xmax=6.74,
xtick style={color=black},
xtick={0,1,2,3,4,5,6},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=52.5,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,50);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,50);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,50);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,50);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,50);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,50);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,50);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,50);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,50);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,50);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,50);
\path [draw=black, thick]
(axis cs:-0.2,50)
--(axis cs:-0.2,50);

\path [draw=black, thick]
(axis cs:0.8,50)
--(axis cs:0.8,50);

\path [draw=black, thick]
(axis cs:1.8,50)
--(axis cs:1.8,50);

\path [draw=black, thick]
(axis cs:2.8,50)
--(axis cs:2.8,50);

\path [draw=black, thick]
(axis cs:3.8,50)
--(axis cs:3.8,50);

\path [draw=black, thick]
(axis cs:4.8,50)
--(axis cs:4.8,50);

\path [draw=black, thick]
(axis cs:5.8,50)
--(axis cs:5.8,50);

\path [draw=black, thick]
(axis cs:0.2,50)
--(axis cs:0.2,50);

\path [draw=black, thick]
(axis cs:1.2,50)
--(axis cs:1.2,50);

\path [draw=black, thick]
(axis cs:2.2,50)
--(axis cs:2.2,50);

\path [draw=black, thick]
(axis cs:3.2,50)
--(axis cs:3.2,50);

\path [draw=black, thick]
(axis cs:4.2,50)
--(axis cs:4.2,50);

\path [draw=black, thick]
(axis cs:5.2,50)
--(axis cs:5.2,50);

\path [draw=black, thick]
(axis cs:6.2,50)
--(axis cs:6.2,50);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_7_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.74, xmax=6.74,
xtick style={color=black},
xtick={0,1,2,3,4,5,6},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=14.6691726883051,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,4.01588299969641);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,3.94562238644543);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,3.93251387947485);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,3.0987437382559);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,4.82596556981851);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,4.75643161148832);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,4.16225624870128);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,7.19942890212082);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,7.47515378892816);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,9.51342495844303);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,10.2674576087398);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,7.58338942029469);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,10.7196324132843);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,7.21118814468086);
\path [draw=black, thick]
(axis cs:-0.2,3.22379032910066)
--(axis cs:-0.2,4.80797567029217);

\path [draw=black, thick]
(axis cs:0.8,3.05936801533163)
--(axis cs:0.8,4.83187675755923);

\path [draw=black, thick]
(axis cs:1.8,2.93400262772663)
--(axis cs:1.8,4.93102513122307);

\path [draw=black, thick]
(axis cs:2.8,2.70959038227014)
--(axis cs:2.8,3.48789709424166);

\path [draw=black, thick]
(axis cs:3.8,3.31305444891085)
--(axis cs:3.8,6.33887669072617);

\path [draw=black, thick]
(axis cs:4.8,3.60177677939245)
--(axis cs:4.8,5.91108644358418);

\path [draw=black, thick]
(axis cs:5.8,3.10713354727828)
--(axis cs:5.8,5.21737895012428);

\path [draw=black, thick]
(axis cs:0.2,5.08031631617306)
--(axis cs:0.2,9.31854148806857);

\path [draw=black, thick]
(axis cs:1.2,5.03710753638642)
--(axis cs:1.2,9.9132000414699);

\path [draw=black, thick]
(axis cs:2.2,7.0961300332151)
--(axis cs:2.2,11.930719883671);

\path [draw=black, thick]
(axis cs:3.2,7.05436922479571)
--(axis cs:3.2,13.4805459926838);

\path [draw=black, thick]
(axis cs:4.2,5.24099893150334)
--(axis cs:4.2,9.92577990908605);

\path [draw=black, thick]
(axis cs:5.2,7.46862417104007)
--(axis cs:5.2,13.9706406555286);

\path [draw=black, thick]
(axis cs:6.2,5.0413000949212)
--(axis cs:6.2,9.38107619444052);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_7_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.74, xmax=6.74,
xtick style={color=black},
xtick={0,1,2,3,4,5,6},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=52.5,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,50);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,50);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,50);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,50);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,50);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,50);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,50);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,50);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,50);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,50);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,50);
\path [draw=black, thick]
(axis cs:-0.2,50)
--(axis cs:-0.2,50);

\path [draw=black, thick]
(axis cs:0.8,50)
--(axis cs:0.8,50);

\path [draw=black, thick]
(axis cs:1.8,50)
--(axis cs:1.8,50);

\path [draw=black, thick]
(axis cs:2.8,50)
--(axis cs:2.8,50);

\path [draw=black, thick]
(axis cs:3.8,50)
--(axis cs:3.8,50);

\path [draw=black, thick]
(axis cs:4.8,50)
--(axis cs:4.8,50);

\path [draw=black, thick]
(axis cs:5.8,50)
--(axis cs:5.8,50);

\path [draw=black, thick]
(axis cs:0.2,50)
--(axis cs:0.2,50);

\path [draw=black, thick]
(axis cs:1.2,50)
--(axis cs:1.2,50);

\path [draw=black, thick]
(axis cs:2.2,50)
--(axis cs:2.2,50);

\path [draw=black, thick]
(axis cs:3.2,50)
--(axis cs:3.2,50);

\path [draw=black, thick]
(axis cs:4.2,50)
--(axis cs:4.2,50);

\path [draw=black, thick]
(axis cs:5.2,50)
--(axis cs:5.2,50);

\path [draw=black, thick]
(axis cs:6.2,50)
--(axis cs:6.2,50);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_7_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.74, xmax=6.74,
xtick style={color=black},
xtick={0,1,2,3,4,5,6},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=6.65582052526248,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,4.01588299969641);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,3.94562238644543);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,3.93251387947485);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,3.0987437382559);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,4.82596556981851);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,4.75643161148832);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,4.16225624870128);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,2.34039257237714);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,2.34065669693201);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,2.34074419713799);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,2.34071178302239);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,2.34091393343604);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,2.3408315564087);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,2.34107183629544);
\path [draw=black, thick]
(axis cs:-0.2,3.22379032910066)
--(axis cs:-0.2,4.80797567029217);

\path [draw=black, thick]
(axis cs:0.8,3.05936801533163)
--(axis cs:0.8,4.83187675755923);

\path [draw=black, thick]
(axis cs:1.8,2.93400262772663)
--(axis cs:1.8,4.93102513122307);

\path [draw=black, thick]
(axis cs:2.8,2.70959038227014)
--(axis cs:2.8,3.48789709424166);

\path [draw=black, thick]
(axis cs:3.8,3.31305444891085)
--(axis cs:3.8,6.33887669072617);

\path [draw=black, thick]
(axis cs:4.8,3.60177677939245)
--(axis cs:4.8,5.91108644358418);

\path [draw=black, thick]
(axis cs:5.8,3.10713354727828)
--(axis cs:5.8,5.21737895012428);

\path [draw=black, thick]
(axis cs:0.2,2.3397205187909)
--(axis cs:0.2,2.34106462596338);

\path [draw=black, thick]
(axis cs:1.2,2.34013230563706)
--(axis cs:1.2,2.34118108822696);

\path [draw=black, thick]
(axis cs:2.2,2.34013363666504)
--(axis cs:2.2,2.34135475761093);

\path [draw=black, thick]
(axis cs:3.2,2.3400390727254)
--(axis cs:3.2,2.34138449331939);

\path [draw=black, thick]
(axis cs:4.2,2.34017982221358)
--(axis cs:4.2,2.3416480446585);

\path [draw=black, thick]
(axis cs:5.2,2.34007370498518)
--(axis cs:5.2,2.34158940783222);

\path [draw=black, thick]
(axis cs:6.2,2.34042945226197)
--(axis cs:6.2,2.34171422032891);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_7_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.74, xmax=6.74,
xtick style={color=black},
xtick={0,1,2,3,4,5,6},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=52.5,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,50);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,50);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,50);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,50);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,50);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,50);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,50);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,50);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,50);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,50);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,50);
\path [draw=black, thick]
(axis cs:-0.2,50)
--(axis cs:-0.2,50);

\path [draw=black, thick]
(axis cs:0.8,50)
--(axis cs:0.8,50);

\path [draw=black, thick]
(axis cs:1.8,50)
--(axis cs:1.8,50);

\path [draw=black, thick]
(axis cs:2.8,50)
--(axis cs:2.8,50);

\path [draw=black, thick]
(axis cs:3.8,50)
--(axis cs:3.8,50);

\path [draw=black, thick]
(axis cs:4.8,50)
--(axis cs:4.8,50);

\path [draw=black, thick]
(axis cs:5.8,50)
--(axis cs:5.8,50);

\path [draw=black, thick]
(axis cs:0.2,50)
--(axis cs:0.2,50);

\path [draw=black, thick]
(axis cs:1.2,50)
--(axis cs:1.2,50);

\path [draw=black, thick]
(axis cs:2.2,50)
--(axis cs:2.2,50);

\path [draw=black, thick]
(axis cs:3.2,50)
--(axis cs:3.2,50);

\path [draw=black, thick]
(axis cs:4.2,50)
--(axis cs:4.2,50);

\path [draw=black, thick]
(axis cs:5.2,50)
--(axis cs:5.2,50);

\path [draw=black, thick]
(axis cs:6.2,50)
--(axis cs:6.2,50);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_8_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.79, xmax=7.79,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=70.9496744969663,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,3.33183225653613);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,5.89922949871585);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,4.38015423857199);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,4.40494942093713);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,4.77961039697484);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,5.16600952875581);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,4.99523410196986);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,4.28167834646932);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,48.7860684032875);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,53.1905592162201);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,45.032508121382);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,50.167550028123);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,47.2340997160108);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,58.72014786927);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,49.3952559274807);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,52.0110701662361);
\path [draw=black, thick]
(axis cs:-0.2,2.81757281755699)
--(axis cs:-0.2,3.84609169551526);

\path [draw=black, thick]
(axis cs:0.8,4.3566676872441)
--(axis cs:0.8,7.44179131018759);

\path [draw=black, thick]
(axis cs:1.8,3.36427265820768)
--(axis cs:1.8,5.39603581893631);

\path [draw=black, thick]
(axis cs:2.8,2.96262896147488)
--(axis cs:2.8,5.84726988039939);

\path [draw=black, thick]
(axis cs:3.8,3.7112700643752)
--(axis cs:3.8,5.84795072957448);

\path [draw=black, thick]
(axis cs:4.8,4.06617827764904)
--(axis cs:4.8,6.26584077986258);

\path [draw=black, thick]
(axis cs:5.8,3.88718354492071)
--(axis cs:5.8,6.103284659019);

\path [draw=black, thick]
(axis cs:6.8,3.12295412375042)
--(axis cs:6.8,5.44040256918823);

\path [draw=black, thick]
(axis cs:0.2,39.4643582154349)
--(axis cs:0.2,58.10777859114);

\path [draw=black, thick]
(axis cs:1.2,44.6651223620089)
--(axis cs:1.2,61.7159960704314);

\path [draw=black, thick]
(axis cs:2.2,35.5348324470069)
--(axis cs:2.2,54.5301837957571);

\path [draw=black, thick]
(axis cs:3.2,40.3981918906388)
--(axis cs:3.2,59.9369081656072);

\path [draw=black, thick]
(axis cs:4.2,37.9358388688532)
--(axis cs:4.2,56.5323605631684);

\path [draw=black, thick]
(axis cs:5.2,49.8691771700006)
--(axis cs:5.2,67.5711185685394);

\path [draw=black, thick]
(axis cs:6.2,39.5617317145516)
--(axis cs:6.2,59.2287801404098);

\path [draw=black, thick]
(axis cs:7.2,42.2653780881493)
--(axis cs:7.2,61.756762244323);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_8_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.79, xmax=7.79,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=52.5,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,50);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,50);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,50);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,50);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,50);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,50);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,50);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,50);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,50);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,50);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,50);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,50);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,50);
\path [draw=black, thick]
(axis cs:-0.2,50)
--(axis cs:-0.2,50);

\path [draw=black, thick]
(axis cs:0.8,50)
--(axis cs:0.8,50);

\path [draw=black, thick]
(axis cs:1.8,50)
--(axis cs:1.8,50);

\path [draw=black, thick]
(axis cs:2.8,50)
--(axis cs:2.8,50);

\path [draw=black, thick]
(axis cs:3.8,50)
--(axis cs:3.8,50);

\path [draw=black, thick]
(axis cs:4.8,50)
--(axis cs:4.8,50);

\path [draw=black, thick]
(axis cs:5.8,50)
--(axis cs:5.8,50);

\path [draw=black, thick]
(axis cs:6.8,50)
--(axis cs:6.8,50);

\path [draw=black, thick]
(axis cs:0.2,50)
--(axis cs:0.2,50);

\path [draw=black, thick]
(axis cs:1.2,50)
--(axis cs:1.2,50);

\path [draw=black, thick]
(axis cs:2.2,50)
--(axis cs:2.2,50);

\path [draw=black, thick]
(axis cs:3.2,50)
--(axis cs:3.2,50);

\path [draw=black, thick]
(axis cs:4.2,50)
--(axis cs:4.2,50);

\path [draw=black, thick]
(axis cs:5.2,50)
--(axis cs:5.2,50);

\path [draw=black, thick]
(axis cs:6.2,50)
--(axis cs:6.2,50);

\path [draw=black, thick]
(axis cs:7.2,50)
--(axis cs:7.2,50);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_8_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.79, xmax=7.79,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=16.9302229381944,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,3.33183225653613);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,5.89922949871584);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,4.38015423857199);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,4.40494942093713);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,4.77961039697484);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,5.16600952875581);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,4.99523410196986);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,4.28167834646932);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,6.96084208367946);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,10.7639249902859);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,8.23574150632345);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,12.0993700517035);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,7.42187600060038);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,9.06267686670304);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,12.0389450474937);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,7.06247684131764);
\path [draw=black, thick]
(axis cs:-0.2,2.81757281755699)
--(axis cs:-0.2,3.84609169551527);

\path [draw=black, thick]
(axis cs:0.8,4.3566676872441)
--(axis cs:0.8,7.44179131018759);

\path [draw=black, thick]
(axis cs:1.8,3.36427265820768)
--(axis cs:1.8,5.39603581893631);

\path [draw=black, thick]
(axis cs:2.8,2.96262896147488)
--(axis cs:2.8,5.84726988039939);

\path [draw=black, thick]
(axis cs:3.8,3.7112700643752)
--(axis cs:3.8,5.84795072957449);

\path [draw=black, thick]
(axis cs:4.8,4.06617827764904)
--(axis cs:4.8,6.26584077986258);

\path [draw=black, thick]
(axis cs:5.8,3.88718354492071)
--(axis cs:5.8,6.103284659019);

\path [draw=black, thick]
(axis cs:6.8,3.12295412375042)
--(axis cs:6.8,5.44040256918823);

\path [draw=black, thick]
(axis cs:0.2,4.55291090238767)
--(axis cs:0.2,9.36877326497124);

\path [draw=black, thick]
(axis cs:1.2,7.17490586966223)
--(axis cs:1.2,14.3529441109096);

\path [draw=black, thick]
(axis cs:2.2,5.82522096182471)
--(axis cs:2.2,10.6462620508222);

\path [draw=black, thick]
(axis cs:3.2,8.07471825750746)
--(axis cs:3.2,16.1240218458995);

\path [draw=black, thick]
(axis cs:4.2,4.82447761158659)
--(axis cs:4.2,10.0192743896142);

\path [draw=black, thick]
(axis cs:5.2,5.99439545698558)
--(axis cs:5.2,12.1309582764205);

\path [draw=black, thick]
(axis cs:6.2,7.97115125355367)
--(axis cs:6.2,16.1067388414337);

\path [draw=black, thick]
(axis cs:7.2,5.36635654365453)
--(axis cs:7.2,8.75859713898075);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_8_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.79, xmax=7.79,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=52.5,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,50);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,50);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,50);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,50);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,50);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,50);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,50);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,50);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,50);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,50);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,50);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,50);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,50);
\path [draw=black, thick]
(axis cs:-0.2,50)
--(axis cs:-0.2,50);

\path [draw=black, thick]
(axis cs:0.8,50)
--(axis cs:0.8,50);

\path [draw=black, thick]
(axis cs:1.8,50)
--(axis cs:1.8,50);

\path [draw=black, thick]
(axis cs:2.8,50)
--(axis cs:2.8,50);

\path [draw=black, thick]
(axis cs:3.8,50)
--(axis cs:3.8,50);

\path [draw=black, thick]
(axis cs:4.8,50)
--(axis cs:4.8,50);

\path [draw=black, thick]
(axis cs:5.8,50)
--(axis cs:5.8,50);

\path [draw=black, thick]
(axis cs:6.8,50)
--(axis cs:6.8,50);

\path [draw=black, thick]
(axis cs:0.2,50)
--(axis cs:0.2,50);

\path [draw=black, thick]
(axis cs:1.2,50)
--(axis cs:1.2,50);

\path [draw=black, thick]
(axis cs:2.2,50)
--(axis cs:2.2,50);

\path [draw=black, thick]
(axis cs:3.2,50)
--(axis cs:3.2,50);

\path [draw=black, thick]
(axis cs:4.2,50)
--(axis cs:4.2,50);

\path [draw=black, thick]
(axis cs:5.2,50)
--(axis cs:5.2,50);

\path [draw=black, thick]
(axis cs:6.2,50)
--(axis cs:6.2,50);

\path [draw=black, thick]
(axis cs:7.2,50)
--(axis cs:7.2,50);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_8_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.79, xmax=7.79,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=7.81388087569697,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,3.33183225653613);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,5.89922949871585);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,4.38015423857199);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,4.40494942093713);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,4.77961039697484);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,5.16600952875581);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,4.99523410196986);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,4.28167834646932);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,2.34099797581648);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,2.34086805677895);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,2.34112935641252);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,2.34059836955232);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,2.34136959558429);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,2.3406141120194);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,2.34135590163048);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,2.34055025857173);
\path [draw=black, thick]
(axis cs:-0.2,2.81757281755699)
--(axis cs:-0.2,3.84609169551527);

\path [draw=black, thick]
(axis cs:0.8,4.3566676872441)
--(axis cs:0.8,7.44179131018759);

\path [draw=black, thick]
(axis cs:1.8,3.36427265820768)
--(axis cs:1.8,5.39603581893631);

\path [draw=black, thick]
(axis cs:2.8,2.96262896147488)
--(axis cs:2.8,5.84726988039939);

\path [draw=black, thick]
(axis cs:3.8,3.7112700643752)
--(axis cs:3.8,5.84795072957448);

\path [draw=black, thick]
(axis cs:4.8,4.06617827764904)
--(axis cs:4.8,6.26584077986258);

\path [draw=black, thick]
(axis cs:5.8,3.88718354492071)
--(axis cs:5.8,6.103284659019);

\path [draw=black, thick]
(axis cs:6.8,3.12295412375042)
--(axis cs:6.8,5.44040256918823);

\path [draw=black, thick]
(axis cs:0.2,2.34022114526635)
--(axis cs:0.2,2.34177480636661);

\path [draw=black, thick]
(axis cs:1.2,2.3401682764154)
--(axis cs:1.2,2.3415678371425);

\path [draw=black, thick]
(axis cs:2.2,2.34044028486192)
--(axis cs:2.2,2.34181842796312);

\path [draw=black, thick]
(axis cs:3.2,2.34001395405029)
--(axis cs:3.2,2.34118278505434);

\path [draw=black, thick]
(axis cs:4.2,2.34042486343037)
--(axis cs:4.2,2.34231432773821);

\path [draw=black, thick]
(axis cs:5.2,2.34012994746811)
--(axis cs:5.2,2.34109827657068);

\path [draw=black, thick]
(axis cs:6.2,2.34075151955936)
--(axis cs:6.2,2.34196028370161);

\path [draw=black, thick]
(axis cs:7.2,2.33994761102492)
--(axis cs:7.2,2.34115290611853);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_8_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.79, xmax=7.79,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=52.5,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,50);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,50);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,50);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,50);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,50);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,50);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,50);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,50);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,50);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,50);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,50);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,50);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,50);
\path [draw=black, thick]
(axis cs:-0.2,50)
--(axis cs:-0.2,50);

\path [draw=black, thick]
(axis cs:0.8,50)
--(axis cs:0.8,50);

\path [draw=black, thick]
(axis cs:1.8,50)
--(axis cs:1.8,50);

\path [draw=black, thick]
(axis cs:2.8,50)
--(axis cs:2.8,50);

\path [draw=black, thick]
(axis cs:3.8,50)
--(axis cs:3.8,50);

\path [draw=black, thick]
(axis cs:4.8,50)
--(axis cs:4.8,50);

\path [draw=black, thick]
(axis cs:5.8,50)
--(axis cs:5.8,50);

\path [draw=black, thick]
(axis cs:6.8,50)
--(axis cs:6.8,50);

\path [draw=black, thick]
(axis cs:0.2,50)
--(axis cs:0.2,50);

\path [draw=black, thick]
(axis cs:1.2,50)
--(axis cs:1.2,50);

\path [draw=black, thick]
(axis cs:2.2,50)
--(axis cs:2.2,50);

\path [draw=black, thick]
(axis cs:3.2,50)
--(axis cs:3.2,50);

\path [draw=black, thick]
(axis cs:4.2,50)
--(axis cs:4.2,50);

\path [draw=black, thick]
(axis cs:5.2,50)
--(axis cs:5.2,50);

\path [draw=black, thick]
(axis cs:6.2,50)
--(axis cs:6.2,50);

\path [draw=black, thick]
(axis cs:7.2,50)
--(axis cs:7.2,50);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_9_bars/smartStart_False_cbap_False/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.84, xmax=8.84,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=69.9283395586244,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,3.75103524454283);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,3.97969747484059);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,4.01848692369212);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,5.10004783071683);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,4.93982093323989);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,4.45797200653797);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,4.1365072912642);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,4.76126546276597);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,4.90459758553794);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,44.721580564699);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,53.4898214695947);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,54.3336642297559);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,55.8320467306209);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,50.0945166076221);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,48.6399897550323);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,54.7630367925575);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,53.0132436875716);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,55.1267664107897);
\path [draw=black, thick]
(axis cs:-0.2,2.93401340234363)
--(axis cs:-0.2,4.56805708674202);

\path [draw=black, thick]
(axis cs:0.8,3.19867940512695)
--(axis cs:0.8,4.76071554455423);

\path [draw=black, thick]
(axis cs:1.8,3.00452760420495)
--(axis cs:1.8,5.0324462431793);

\path [draw=black, thick]
(axis cs:2.8,3.85865873443269)
--(axis cs:2.8,6.34143692700098);

\path [draw=black, thick]
(axis cs:3.8,3.76576163207394)
--(axis cs:3.8,6.11388023440585);

\path [draw=black, thick]
(axis cs:4.8,3.45267081076041)
--(axis cs:4.8,5.46327320231553);

\path [draw=black, thick]
(axis cs:5.8,3.32181496389567)
--(axis cs:5.8,4.95119961863274);

\path [draw=black, thick]
(axis cs:6.8,3.43761548450378)
--(axis cs:6.8,6.08491544102817);

\path [draw=black, thick]
(axis cs:7.8,3.95240212622227)
--(axis cs:7.8,5.8567930448536);

\path [draw=black, thick]
(axis cs:0.2,33.621524038375)
--(axis cs:0.2,55.8216370910231);

\path [draw=black, thick]
(axis cs:1.2,44.3117920362829)
--(axis cs:1.2,62.6678509029064);

\path [draw=black, thick]
(axis cs:2.2,44.4879899282951)
--(axis cs:2.2,64.1793385312168);

\path [draw=black, thick]
(axis cs:3.2,45.0656748339804)
--(axis cs:3.2,66.5984186272614);

\path [draw=black, thick]
(axis cs:4.2,39.3083662447146)
--(axis cs:4.2,60.8806669705296);

\path [draw=black, thick]
(axis cs:5.2,39.3488178273672)
--(axis cs:5.2,57.9311616826974);

\path [draw=black, thick]
(axis cs:6.2,44.9721651219596)
--(axis cs:6.2,64.5539084631554);

\path [draw=black, thick]
(axis cs:7.2,44.5127148372892)
--(axis cs:7.2,61.513772537854);

\path [draw=black, thick]
(axis cs:8.2,44.3117943161106)
--(axis cs:8.2,65.9417385054688);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_9_bars/smartStart_False_cbap_False/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.84, xmax=8.84,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=52.5,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,50);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,50);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,50);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,50);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,50);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,50);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,50);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,50);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,50);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,50);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,50);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,50);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,50);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,50);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,50);
\path [draw=black, thick]
(axis cs:-0.2,50)
--(axis cs:-0.2,50);

\path [draw=black, thick]
(axis cs:0.8,50)
--(axis cs:0.8,50);

\path [draw=black, thick]
(axis cs:1.8,50)
--(axis cs:1.8,50);

\path [draw=black, thick]
(axis cs:2.8,50)
--(axis cs:2.8,50);

\path [draw=black, thick]
(axis cs:3.8,50)
--(axis cs:3.8,50);

\path [draw=black, thick]
(axis cs:4.8,50)
--(axis cs:4.8,50);

\path [draw=black, thick]
(axis cs:5.8,50)
--(axis cs:5.8,50);

\path [draw=black, thick]
(axis cs:6.8,50)
--(axis cs:6.8,50);

\path [draw=black, thick]
(axis cs:7.8,50)
--(axis cs:7.8,50);

\path [draw=black, thick]
(axis cs:0.2,50)
--(axis cs:0.2,50);

\path [draw=black, thick]
(axis cs:1.2,50)
--(axis cs:1.2,50);

\path [draw=black, thick]
(axis cs:2.2,50)
--(axis cs:2.2,50);

\path [draw=black, thick]
(axis cs:3.2,50)
--(axis cs:3.2,50);

\path [draw=black, thick]
(axis cs:4.2,50)
--(axis cs:4.2,50);

\path [draw=black, thick]
(axis cs:5.2,50)
--(axis cs:5.2,50);

\path [draw=black, thick]
(axis cs:6.2,50)
--(axis cs:6.2,50);

\path [draw=black, thick]
(axis cs:7.2,50)
--(axis cs:7.2,50);

\path [draw=black, thick]
(axis cs:8.2,50)
--(axis cs:8.2,50);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_9_bars/smartStart_False_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.84, xmax=8.84,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=21.022691623457,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,3.75103524454283);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,3.97969747484059);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,4.01848692369212);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,5.10004783071684);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,4.93982093323989);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,4.45797200653797);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,4.1365072912642);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,4.76126546276597);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,4.90459758553794);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,15.8402642513572);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,13.9150330238834);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,13.762414221297);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,13.9201541763482);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,14.1802545780713);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,12.2092713052427);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,11.9075580469563);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,12.9702688848098);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,11.1642401378934);
\path [draw=black, thick]
(axis cs:-0.2,2.93401340234363)
--(axis cs:-0.2,4.56805708674202);

\path [draw=black, thick]
(axis cs:0.8,3.19867940512695)
--(axis cs:0.8,4.76071554455423);

\path [draw=black, thick]
(axis cs:1.8,3.00452760420495)
--(axis cs:1.8,5.0324462431793);

\path [draw=black, thick]
(axis cs:2.8,3.85865873443269)
--(axis cs:2.8,6.34143692700098);

\path [draw=black, thick]
(axis cs:3.8,3.76576163207394)
--(axis cs:3.8,6.11388023440585);

\path [draw=black, thick]
(axis cs:4.8,3.45267081076041)
--(axis cs:4.8,5.46327320231553);

\path [draw=black, thick]
(axis cs:5.8,3.32181496389567)
--(axis cs:5.8,4.95119961863274);

\path [draw=black, thick]
(axis cs:6.8,3.43761548450378)
--(axis cs:6.8,6.08491544102817);

\path [draw=black, thick]
(axis cs:7.8,3.95240212622227)
--(axis cs:7.8,5.8567930448536);

\path [draw=black, thick]
(axis cs:0.2,11.6589174327554)
--(axis cs:0.2,20.021611069959);

\path [draw=black, thick]
(axis cs:1.2,9.59881810141072)
--(axis cs:1.2,18.231247946356);

\path [draw=black, thick]
(axis cs:2.2,9.85940838163594)
--(axis cs:2.2,17.665420060958);

\path [draw=black, thick]
(axis cs:3.2,10.2705113779996)
--(axis cs:3.2,17.5697969746969);

\path [draw=black, thick]
(axis cs:4.2,10.5778650214877)
--(axis cs:4.2,17.7826441346548);

\path [draw=black, thick]
(axis cs:5.2,8.53122682963133)
--(axis cs:5.2,15.887315780854);

\path [draw=black, thick]
(axis cs:6.2,8.08367405283785)
--(axis cs:6.2,15.7314420410748);

\path [draw=black, thick]
(axis cs:7.2,8.71682742548875)
--(axis cs:7.2,17.2237103441308);

\path [draw=black, thick]
(axis cs:8.2,7.6036074626106)
--(axis cs:8.2,14.7248728131762);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_9_bars/smartStart_False_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.84, xmax=8.84,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=52.5003863751831,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,50);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,50);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,50);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,50);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,50);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,50);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,50);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,50);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,50);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,50);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,50);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,50);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,50);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,49.9996030701754);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,50);
\path [draw=black, thick]
(axis cs:-0.2,50)
--(axis cs:-0.2,50);

\path [draw=black, thick]
(axis cs:0.8,50)
--(axis cs:0.8,50);

\path [draw=black, thick]
(axis cs:1.8,50)
--(axis cs:1.8,50);

\path [draw=black, thick]
(axis cs:2.8,50)
--(axis cs:2.8,50);

\path [draw=black, thick]
(axis cs:3.8,50)
--(axis cs:3.8,50);

\path [draw=black, thick]
(axis cs:4.8,50)
--(axis cs:4.8,50);

\path [draw=black, thick]
(axis cs:5.8,50)
--(axis cs:5.8,50);

\path [draw=black, thick]
(axis cs:6.8,50)
--(axis cs:6.8,50);

\path [draw=black, thick]
(axis cs:7.8,50)
--(axis cs:7.8,50);

\path [draw=black, thick]
(axis cs:0.2,50)
--(axis cs:0.2,50);

\path [draw=black, thick]
(axis cs:1.2,50)
--(axis cs:1.2,50);

\path [draw=black, thick]
(axis cs:2.2,50)
--(axis cs:2.2,50);

\path [draw=black, thick]
(axis cs:3.2,50)
--(axis cs:3.2,50);

\path [draw=black, thick]
(axis cs:4.2,50)
--(axis cs:4.2,50);

\path [draw=black, thick]
(axis cs:5.2,50)
--(axis cs:5.2,50);

\path [draw=black, thick]
(axis cs:6.2,50)
--(axis cs:6.2,50);

\path [draw=black, thick]
(axis cs:7.2,49.998838163986)
--(axis cs:7.2,50.0003679763649);

\path [draw=black, thick]
(axis cs:8.2,50)
--(axis cs:8.2,50);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_9_bars/smartStart_True_cbap_True/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.84, xmax=8.84,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=6.65850877335103,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,3.75103524454283);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,3.97969747484059);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,4.01848692369212);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,5.10004783071683);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,4.93982093323989);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,4.45797200653797);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,4.1365072912642);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,4.76126546276597);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,4.90459758553794);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,2.340821322297);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,2.34114415973591);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,2.34097418251537);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,2.34074712487349);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,2.34062577348438);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,2.34120006577044);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,2.34080401520567);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,2.34093207886646);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,2.34059765217701);
\path [draw=black, thick]
(axis cs:-0.2,2.93401340234363)
--(axis cs:-0.2,4.56805708674202);

\path [draw=black, thick]
(axis cs:0.8,3.19867940512695)
--(axis cs:0.8,4.76071554455423);

\path [draw=black, thick]
(axis cs:1.8,3.00452760420495)
--(axis cs:1.8,5.0324462431793);

\path [draw=black, thick]
(axis cs:2.8,3.85865873443269)
--(axis cs:2.8,6.34143692700098);

\path [draw=black, thick]
(axis cs:3.8,3.76576163207394)
--(axis cs:3.8,6.11388023440585);

\path [draw=black, thick]
(axis cs:4.8,3.45267081076041)
--(axis cs:4.8,5.46327320231553);

\path [draw=black, thick]
(axis cs:5.8,3.32181496389567)
--(axis cs:5.8,4.95119961863274);

\path [draw=black, thick]
(axis cs:6.8,3.43761548450378)
--(axis cs:6.8,6.08491544102817);

\path [draw=black, thick]
(axis cs:7.8,3.95240212622227)
--(axis cs:7.8,5.8567930448536);

\path [draw=black, thick]
(axis cs:0.2,2.33989230065357)
--(axis cs:0.2,2.34175034394044);

\path [draw=black, thick]
(axis cs:1.2,2.34025051972096)
--(axis cs:1.2,2.34203779975085);

\path [draw=black, thick]
(axis cs:2.2,2.34033521701281)
--(axis cs:2.2,2.34161314801792);

\path [draw=black, thick]
(axis cs:3.2,2.33993170172271)
--(axis cs:3.2,2.34156254802426);

\path [draw=black, thick]
(axis cs:4.2,2.340119817262)
--(axis cs:4.2,2.34113172970675);

\path [draw=black, thick]
(axis cs:5.2,2.34052740909611)
--(axis cs:5.2,2.34187272244476);

\path [draw=black, thick]
(axis cs:6.2,2.34018083960749)
--(axis cs:6.2,2.34142719080386);

\path [draw=black, thick]
(axis cs:7.2,2.3402614977492)
--(axis cs:7.2,2.34160265998371);

\path [draw=black, thick]
(axis cs:8.2,2.33985098026533)
--(axis cs:8.2,2.3413443240887);

\end{axis}

\end{tikzpicture}


==> img/50Mbps/numStas_9_bars/smartStart_True_cbap_True/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.84, xmax=8.84,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=52.5,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,50);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,50);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,50);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,50);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,50);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,50);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,50);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,50);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,50);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,50);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,50);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,50);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,50);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,50);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,50);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,50);
\path [draw=black, thick]
(axis cs:-0.2,50)
--(axis cs:-0.2,50);

\path [draw=black, thick]
(axis cs:0.8,50)
--(axis cs:0.8,50);

\path [draw=black, thick]
(axis cs:1.8,50)
--(axis cs:1.8,50);

\path [draw=black, thick]
(axis cs:2.8,50)
--(axis cs:2.8,50);

\path [draw=black, thick]
(axis cs:3.8,50)
--(axis cs:3.8,50);

\path [draw=black, thick]
(axis cs:4.8,50)
--(axis cs:4.8,50);

\path [draw=black, thick]
(axis cs:5.8,50)
--(axis cs:5.8,50);

\path [draw=black, thick]
(axis cs:6.8,50)
--(axis cs:6.8,50);

\path [draw=black, thick]
(axis cs:7.8,50)
--(axis cs:7.8,50);

\path [draw=black, thick]
(axis cs:0.2,50)
--(axis cs:0.2,50);

\path [draw=black, thick]
(axis cs:1.2,50)
--(axis cs:1.2,50);

\path [draw=black, thick]
(axis cs:2.2,50)
--(axis cs:2.2,50);

\path [draw=black, thick]
(axis cs:3.2,50)
--(axis cs:3.2,50);

\path [draw=black, thick]
(axis cs:4.2,50)
--(axis cs:4.2,50);

\path [draw=black, thick]
(axis cs:5.2,50)
--(axis cs:5.2,50);

\path [draw=black, thick]
(axis cs:6.2,50)
--(axis cs:6.2,50);

\path [draw=black, thick]
(axis cs:7.2,50)
--(axis cs:7.2,50);

\path [draw=black, thick]
(axis cs:8.2,50)
--(axis cs:8.2,50);

\end{axis}

\end{tikzpicture}


==> img/bi_interval.tex <==
\begin{tikzpicture}[scale=1, every node/.style={transform shape, font=\scriptsize}]

\def\allocHeight{0.8}
\definecolor{mygray}{rgb}{0.8, 0.8, 0.8}

% time axis
\draw[thick, dashed] (-0.7,0) -- (-0.2,0);
\draw[thick] (-0.2,0) -- (4,0);
\draw[thick, dashed] (4,0) -- (4.5,0);
\draw[->, thick] (4.5,0) -- (7,0) node[below] {t};

% BHI
\draw[fill=mygray] (0,0) rectangle ++(0.8,\allocHeight) node[pos=.5] {BTI};
\draw[fill=mygray] (0.8,0) rectangle ++(0.8,\allocHeight) node[pos=.5] {A-BFT};
\draw[fill=mygray] (1.6,0) rectangle ++(0.8,\allocHeight) node[pos=.5] {ATI};

% DTI
\draw (2.4,0) rectangle ++(1,\allocHeight) node[pos=.5] {CBAP\textsubscript{1}};
\draw (3.4,0) rectangle ++(0.6,\allocHeight) node[pos=.5] {SP\textsubscript{1}};

\draw[dashed] (4,\allocHeight) -- (4.5,\allocHeight);

\draw (4.5,0) rectangle ++(0.8,\allocHeight) node[pos=.5] {SP\textsubscript{N}};
\draw (5.3,0) rectangle ++(1.2,\allocHeight) node[pos=.5] {CBAP\textsubscript{M}};

% text
\draw[|-|] (0, \allocHeight+0.2) -- node[above] {BHI} (2.4, \allocHeight+0.2);
\draw[|-|] (2.4, \allocHeight+0.2) -- node[above] {DTI} (6.5, \allocHeight+0.2);
\draw[|-|] (0, \allocHeight + 0.6) -- node[above] {BI} (6.5, \allocHeight+0.6);

\end{tikzpicture}

==> img/burst/jain_fairness.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
width=\fwidth,
height=\fheight,
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.03)}, anchor=south west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Aggr. Offered Rate / Nominal Rate},
xmajorgrids,
xmin=-0.0395, xmax=1.0495,
xtick style={color=black},
xtick={-0.2,0,0.2,0.4,0.6,0.8,1,1.2},
xticklabels={−0.2,0.0,0.2,0.4,0.6,0.8,1.0,1.2},
y grid style={white!69.0196078431373!black},
ylabel={Jain's Fairness Index},
ymajorgrids,
ymin=0, ymax=1.00057116563914,
ytick style={color=black}
]
\path [draw=color0, thick]
(axis cs:0.01,1)
--(axis cs:0.01,1);

\path [draw=color0, thick]
(axis cs:0.1,1)
--(axis cs:0.1,1);

\path [draw=color0, thick]
(axis cs:0.2,1)
--(axis cs:0.2,1);

\path [draw=color0, thick]
(axis cs:0.3,1)
--(axis cs:0.3,1);

\path [draw=color0, thick]
(axis cs:0.4,1)
--(axis cs:0.4,1);

\path [draw=color0, thick]
(axis cs:0.5,0.99999999992551)
--(axis cs:0.5,1.00000000001189);

\path [draw=color0, thick]
(axis cs:0.6,0.999999999847318)
--(axis cs:0.6,1.00000000001359);

\path [draw=color0, thick]
(axis cs:0.7,0.999999999982744)
--(axis cs:0.7,1.00000000000547);

\path [draw=color0, thick]
(axis cs:0.8,0.999999999936657)
--(axis cs:0.8,1.00000000000918);

\path [draw=color0, thick]
(axis cs:0.9,0.995948674917515)
--(axis cs:0.9,0.997615940071734);

\path [draw=color0, thick]
(axis cs:1,0.988576687502562)
--(axis cs:1,0.993052429381424);

\path [draw=color1, thick]
(axis cs:0.01,1)
--(axis cs:0.01,1);

\path [draw=color1, thick]
(axis cs:0.1,1)
--(axis cs:0.1,1);

\path [draw=color1, thick]
(axis cs:0.2,1)
--(axis cs:0.2,1);

\path [draw=color1, thick]
(axis cs:0.3,1)
--(axis cs:0.3,1);

\path [draw=color1, thick]
(axis cs:0.4,1)
--(axis cs:0.4,1);

\path [draw=color1, thick]
(axis cs:0.5,1)
--(axis cs:0.5,1);

\path [draw=color1, thick]
(axis cs:0.6,1)
--(axis cs:0.6,1);

\path [draw=color1, thick]
(axis cs:0.7,1)
--(axis cs:0.7,1);

\path [draw=color1, thick]
(axis cs:0.8,1)
--(axis cs:0.8,1);

\path [draw=color1, thick]
(axis cs:0.9,1)
--(axis cs:0.9,1);

\path [draw=color1, thick]
(axis cs:1,1)
--(axis cs:1,1);

\path [draw=color1, thick]
(axis cs:0.01,1)
--(axis cs:0.01,1);

\path [draw=color1, thick]
(axis cs:0.1,1)
--(axis cs:0.1,1);

\path [draw=color1, thick]
(axis cs:0.2,1)
--(axis cs:0.2,1);

\path [draw=color1, thick]
(axis cs:0.3,1)
--(axis cs:0.3,1);

\path [draw=color1, thick]
(axis cs:0.4,1)
--(axis cs:0.4,1);

\path [draw=color1, thick]
(axis cs:0.5,0.99999999984546)
--(axis cs:0.5,1.00000000003128);

\path [draw=color1, thick]
(axis cs:0.6,0.999999999968683)
--(axis cs:0.6,1.00000000000992);

\path [draw=color1, thick]
(axis cs:0.7,0.999999999972422)
--(axis cs:0.7,1.000000000004);

\path [draw=color1, thick]
(axis cs:0.8,0.999999999978886)
--(axis cs:0.8,1.00000000000306);

\path [draw=color1, thick]
(axis cs:0.9,0.9756078626726)
--(axis cs:0.9,1.00772547062507);

\path [draw=color1, thick]
(axis cs:1,0.999999999989979)
--(axis cs:1,1.00000000000317);

\path [draw=color1, thick]
(axis cs:0.01,1)
--(axis cs:0.01,1);

\path [draw=color1, thick]
(axis cs:0.1,1)
--(axis cs:0.1,1);

\path [draw=color1, thick]
(axis cs:0.2,1)
--(axis cs:0.2,1);

\path [draw=color1, thick]
(axis cs:0.3,1)
--(axis cs:0.3,1);

\path [draw=color1, thick]
(axis cs:0.4,1)
--(axis cs:0.4,1);

\path [draw=color1, thick]
(axis cs:0.5,1)
--(axis cs:0.5,1);

\path [draw=color1, thick]
(axis cs:0.6,1)
--(axis cs:0.6,1);

\path [draw=color1, thick]
(axis cs:0.7,1)
--(axis cs:0.7,1);

\path [draw=color1, thick]
(axis cs:0.8,1)
--(axis cs:0.8,1);

\path [draw=color1, thick]
(axis cs:0.9,1)
--(axis cs:0.9,1);

\path [draw=color1, thick]
(axis cs:1,1)
--(axis cs:1,1);

\addplot [thick, color0]
table {%
0.01 1
0.1 1
0.2 1
0.3 1
0.4 1
0.5 0.999999999968702
0.6 0.999999999930455
0.7 0.999999999994105
0.8 0.999999999972918
0.9 0.996782307494625
1 0.990814558441993
};
% \addlegendentry{allocationPeriod=1}
\addplot [thick, color1]
table {%
0.01 1
0.1 1
0.2 1
0.3 1
0.4 1
0.5 1
0.6 1
0.7 1
0.8 1
0.9 1
1 1
};
% \addlegendentry{allocationPeriod=1}
\addplot [thick, color1, dashed]
table {%
0.01 1
0.1 1
0.2 1
0.3 1
0.4 1
0.5 0.999999999938372
0.6 0.999999999989301
0.7 0.999999999988209
0.8 0.999999999990973
0.9 0.991666666648835
1 0.999999999996576
};
% \addlegendentry{allocationPeriod=1}
\addplot [thick, color1, densely dotted]
table {%
0.01 1
0.1 1
0.2 1
0.3 1
0.4 1
0.5 1
0.6 1
0.7 1
0.8 1
0.9 1
1 1
};
% \addlegendentry{allocationPeriod=1}
\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOff/normOfferedTraffic_0.01_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=66.9379309397764,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,0.226930747699394);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,0.231270749948552);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,0.434469446693603);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,0.303242961215892);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,49.7309005151156);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,49.1116755539427);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,48.1554647674187);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,54.0411584755545);
\path [draw=black, thick]
(axis cs:-0.2,0.219527322051889)
--(axis cs:-0.2,0.234334173346899);

\path [draw=black, thick]
(axis cs:0.8,0.216723283413551)
--(axis cs:0.8,0.245818216483553);

\path [draw=black, thick]
(axis cs:1.8,0.103754829507518)
--(axis cs:1.8,0.765184063879687);

\path [draw=black, thick]
(axis cs:2.8,0.151793691874586)
--(axis cs:2.8,0.454692230557199);

\path [draw=black, thick]
(axis cs:0.2,40.4708359173118)
--(axis cs:0.2,58.9909651129195);

\path [draw=black, thick]
(axis cs:1.2,38.4253830601494)
--(axis cs:1.2,59.7979680477361);

\path [draw=black, thick]
(axis cs:2.2,38.4885713276912)
--(axis cs:2.2,57.8223582071461);

\path [draw=black, thick]
(axis cs:3.2,44.3319065322743)
--(axis cs:3.2,63.7504104188347);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOff/normOfferedTraffic_0.01_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=2.90792578125,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,2.769453125);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,2.769453125);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,2.769453125);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,2.769453125);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,2.769453125);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,2.769453125);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,2.769453125);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,2.769453125);
\path [draw=black, thick]
(axis cs:-0.2,2.769453125)
--(axis cs:-0.2,2.769453125);

\path [draw=black, thick]
(axis cs:0.8,2.769453125)
--(axis cs:0.8,2.769453125);

\path [draw=black, thick]
(axis cs:1.8,2.769453125)
--(axis cs:1.8,2.769453125);

\path [draw=black, thick]
(axis cs:2.8,2.769453125)
--(axis cs:2.8,2.769453125);

\path [draw=black, thick]
(axis cs:0.2,2.769453125)
--(axis cs:0.2,2.769453125);

\path [draw=black, thick]
(axis cs:1.2,2.769453125)
--(axis cs:1.2,2.769453125);

\path [draw=black, thick]
(axis cs:2.2,2.769453125)
--(axis cs:2.2,2.769453125);

\path [draw=black, thick]
(axis cs:3.2,2.769453125)
--(axis cs:3.2,2.769453125);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOff/normOfferedTraffic_0.1_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=71.7173676929679,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,1.65743850384523);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,1.7046068453761);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,1.75763083584366);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,2.10927853416359);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,52.7742462537395);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50.9982175118827);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,49.4060555488574);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,57.9120623865042);
\path [draw=black, thick]
(axis cs:-0.2,1.46310592610005)
--(axis cs:-0.2,1.8517710815904);

\path [draw=black, thick]
(axis cs:0.8,1.3857396923025)
--(axis cs:0.8,2.02347399844971);

\path [draw=black, thick]
(axis cs:1.8,1.39952052370638)
--(axis cs:1.8,2.11574114798094);

\path [draw=black, thick]
(axis cs:2.8,1.4699406965023)
--(axis cs:2.8,2.74861637182489);

\path [draw=black, thick]
(axis cs:0.2,43.1239381498516)
--(axis cs:0.2,62.4245543576274);

\path [draw=black, thick]
(axis cs:1.2,41.5208002713546)
--(axis cs:1.2,60.4756347524108);

\path [draw=black, thick]
(axis cs:2.2,39.5950150197281)
--(axis cs:2.2,59.2170960779867);

\path [draw=black, thick]
(axis cs:3.2,47.5218698273247)
--(axis cs:3.2,68.3022549456837);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOff/normOfferedTraffic_0.1_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=29.0792578125,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,27.69453125);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,27.69453125);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,27.69453125);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,27.69453125);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,27.69453125);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,27.69453125);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,27.69453125);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,27.69453125);
\path [draw=black, thick]
(axis cs:-0.2,27.69453125)
--(axis cs:-0.2,27.69453125);

\path [draw=black, thick]
(axis cs:0.8,27.69453125)
--(axis cs:0.8,27.69453125);

\path [draw=black, thick]
(axis cs:1.8,27.69453125)
--(axis cs:1.8,27.69453125);

\path [draw=black, thick]
(axis cs:2.8,27.69453125)
--(axis cs:2.8,27.69453125);

\path [draw=black, thick]
(axis cs:0.2,27.69453125)
--(axis cs:0.2,27.69453125);

\path [draw=black, thick]
(axis cs:1.2,27.69453125)
--(axis cs:1.2,27.69453125);

\path [draw=black, thick]
(axis cs:2.2,27.69453125)
--(axis cs:2.2,27.69453125);

\path [draw=black, thick]
(axis cs:3.2,27.69453125)
--(axis cs:3.2,27.69453125);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOff/normOfferedTraffic_0.2_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=72.5944123965473,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,3.82546063341778);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,3.56199215312244);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,3.42685280430678);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,3.94955547020377);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,52.9388835260454);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,48.4454030876268);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,52.8237616590331);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,59.368322032194);
\path [draw=black, thick]
(axis cs:-0.2,3.32614005253829)
--(axis cs:-0.2,4.32478121429728);

\path [draw=black, thick]
(axis cs:0.8,2.96557777425465)
--(axis cs:0.8,4.15840653199023);

\path [draw=black, thick]
(axis cs:1.8,2.94804301294666)
--(axis cs:1.8,3.90566259566691);

\path [draw=black, thick]
(axis cs:2.8,3.11629570420001)
--(axis cs:2.8,4.78281523620753);

\path [draw=black, thick]
(axis cs:0.2,43.5442401411504)
--(axis cs:0.2,62.3335269109405);

\path [draw=black, thick]
(axis cs:1.2,38.44060477165)
--(axis cs:1.2,58.4502014036036);

\path [draw=black, thick]
(axis cs:2.2,42.6709439713997)
--(axis cs:2.2,62.9765793466665);

\path [draw=black, thick]
(axis cs:3.2,49.5991084486288)
--(axis cs:3.2,69.1375356157593);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOff/normOfferedTraffic_0.2_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=58.15859765625,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,55.389140625);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,55.389140625);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,55.389140625);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,55.389140625);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,55.389140625);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,55.389140625);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,55.389140625);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,55.389140625);
\path [draw=black, thick]
(axis cs:-0.2,55.389140625)
--(axis cs:-0.2,55.389140625);

\path [draw=black, thick]
(axis cs:0.8,55.389140625)
--(axis cs:0.8,55.389140625);

\path [draw=black, thick]
(axis cs:1.8,55.389140625)
--(axis cs:1.8,55.389140625);

\path [draw=black, thick]
(axis cs:2.8,55.389140625)
--(axis cs:2.8,55.389140625);

\path [draw=black, thick]
(axis cs:0.2,55.389140625)
--(axis cs:0.2,55.389140625);

\path [draw=black, thick]
(axis cs:1.2,55.389140625)
--(axis cs:1.2,55.389140625);

\path [draw=black, thick]
(axis cs:2.2,55.389140625)
--(axis cs:2.2,55.389140625);

\path [draw=black, thick]
(axis cs:3.2,55.389140625)
--(axis cs:3.2,55.389140625);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOff/normOfferedTraffic_0.3_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=69.4804866881452,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,6.73418922055258);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,5.82504579760884);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,5.54711542763041);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,6.35723947922322);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,52.1559969059432);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,48.2471110996751);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,50.5223383362681);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,57.0826191178597);
\path [draw=black, thick]
(axis cs:-0.2,5.594332603322)
--(axis cs:-0.2,7.87404583778317);

\path [draw=black, thick]
(axis cs:0.8,4.90360289255775)
--(axis cs:0.8,6.74648870265993);

\path [draw=black, thick]
(axis cs:1.8,4.82312316873049)
--(axis cs:1.8,6.27110768653032);

\path [draw=black, thick]
(axis cs:2.8,5.30752594518268)
--(axis cs:2.8,7.40695301326376);

\path [draw=black, thick]
(axis cs:0.2,42.7481386552313)
--(axis cs:0.2,61.5638551566551);

\path [draw=black, thick]
(axis cs:1.2,38.832046282071)
--(axis cs:1.2,57.6621759172792);

\path [draw=black, thick]
(axis cs:2.2,41.5169883496562)
--(axis cs:2.2,59.5276883228799);

\path [draw=black, thick]
(axis cs:3.2,47.9933461517716)
--(axis cs:3.2,66.1718920839478);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOff/normOfferedTraffic_0.3_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=87.23785546875,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,83.083671875);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,83.083671875);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,83.083671875);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,83.083671875);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,83.083671875);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,83.083671875);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,83.083671875);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,83.083671875);
\path [draw=black, thick]
(axis cs:-0.2,83.083671875)
--(axis cs:-0.2,83.083671875);

\path [draw=black, thick]
(axis cs:0.8,83.083671875)
--(axis cs:0.8,83.083671875);

\path [draw=black, thick]
(axis cs:1.8,83.083671875)
--(axis cs:1.8,83.083671875);

\path [draw=black, thick]
(axis cs:2.8,83.083671875)
--(axis cs:2.8,83.083671875);

\path [draw=black, thick]
(axis cs:0.2,83.083671875)
--(axis cs:0.2,83.083671875);

\path [draw=black, thick]
(axis cs:1.2,83.083671875)
--(axis cs:1.2,83.083671875);

\path [draw=black, thick]
(axis cs:2.2,83.083671875)
--(axis cs:2.2,83.083671875);

\path [draw=black, thick]
(axis cs:3.2,83.083671875)
--(axis cs:3.2,83.083671875);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOff/normOfferedTraffic_0.4_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=64.9397280542925,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,9.75323120633818);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,8.1227712881128);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,8.14574503454991);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,9.21475662012734);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,51.9287463620756);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,52.1211662524609);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,49.9326155035448);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,51.7611596140203);
\path [draw=black, thick]
(axis cs:-0.2,8.15120118746335)
--(axis cs:-0.2,11.355261225213);

\path [draw=black, thick]
(axis cs:0.8,6.89809221412741)
--(axis cs:0.8,9.34745036209819);

\path [draw=black, thick]
(axis cs:1.8,6.95783439137244)
--(axis cs:1.8,9.33365567772738);

\path [draw=black, thick]
(axis cs:2.8,7.83207256362724)
--(axis cs:2.8,10.5974406766274);

\path [draw=black, thick]
(axis cs:0.2,42.8594015605118)
--(axis cs:0.2,60.9980911636393);

\path [draw=black, thick]
(axis cs:1.2,42.3949724532147)
--(axis cs:1.2,61.8473600517072);

\path [draw=black, thick]
(axis cs:2.2,39.9263489408098)
--(axis cs:2.2,59.9388820662799);

\path [draw=black, thick]
(axis cs:3.2,43.177142278212)
--(axis cs:3.2,60.3451769498287);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOff/normOfferedTraffic_0.4_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=116.3171953125,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,110.77828125);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,110.77828125);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,110.77828125);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,110.77828125);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,110.77828125);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,110.77828125);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,110.77828125);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,110.77828125);
\path [draw=black, thick]
(axis cs:-0.2,110.77828125)
--(axis cs:-0.2,110.77828125);

\path [draw=black, thick]
(axis cs:0.8,110.77828125)
--(axis cs:0.8,110.77828125);

\path [draw=black, thick]
(axis cs:1.8,110.77828125)
--(axis cs:1.8,110.77828125);

\path [draw=black, thick]
(axis cs:2.8,110.77828125)
--(axis cs:2.8,110.77828125);

\path [draw=black, thick]
(axis cs:0.2,110.77828125)
--(axis cs:0.2,110.77828125);

\path [draw=black, thick]
(axis cs:1.2,110.77828125)
--(axis cs:1.2,110.77828125);

\path [draw=black, thick]
(axis cs:2.2,110.77828125)
--(axis cs:2.2,110.77828125);

\path [draw=black, thick]
(axis cs:3.2,110.77828125)
--(axis cs:3.2,110.77828125);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOff/normOfferedTraffic_0.5_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=66.2598542400621,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,12.9808058136175);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,11.0727569744902);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,11.0348870603131);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,12.7420613773217);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,52.2340508286015);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,54.6919916711082);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,50.5724356563588);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,47.591351574519);
\path [draw=black, thick]
(axis cs:-0.2,10.9768594320539)
--(axis cs:-0.2,14.9847521951811);

\path [draw=black, thick]
(axis cs:0.8,9.37322605767419)
--(axis cs:0.8,12.7722878913063);

\path [draw=black, thick]
(axis cs:1.8,9.42777964322606)
--(axis cs:1.8,12.6419944774001);

\path [draw=black, thick]
(axis cs:2.8,10.7014208815343)
--(axis cs:2.8,14.7827018731091);

\path [draw=black, thick]
(axis cs:0.2,43.2787286423068)
--(axis cs:0.2,61.1893730148961);

\path [draw=black, thick]
(axis cs:1.2,46.2793602564431)
--(axis cs:1.2,63.1046230857734);

\path [draw=black, thick]
(axis cs:2.2,41.6795228788531)
--(axis cs:2.2,59.4653484338646);

\path [draw=black, thick]
(axis cs:3.2,39.171028095273)
--(axis cs:3.2,56.0116750537651);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOff/normOfferedTraffic_0.5_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=145.396687618447,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,138.472571600877);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,138.47261129386);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,138.47261129386);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,138.4728125);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,138.4728125);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,138.4728125);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,138.4728125);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,138.4728125);
\path [draw=black, thick]
(axis cs:-0.2,138.472107374662)
--(axis cs:-0.2,138.473035827092);

\path [draw=black, thick]
(axis cs:0.8,138.472223558264)
--(axis cs:0.8,138.472999029456);

\path [draw=black, thick]
(axis cs:1.8,138.472223558264)
--(axis cs:1.8,138.472999029456);

\path [draw=black, thick]
(axis cs:2.8,138.4728125)
--(axis cs:2.8,138.4728125);

\path [draw=black, thick]
(axis cs:0.2,138.4728125)
--(axis cs:0.2,138.4728125);

\path [draw=black, thick]
(axis cs:1.2,138.4728125)
--(axis cs:1.2,138.4728125);

\path [draw=black, thick]
(axis cs:2.2,138.4728125)
--(axis cs:2.2,138.4728125);

\path [draw=black, thick]
(axis cs:3.2,138.4728125)
--(axis cs:3.2,138.4728125);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOff/normOfferedTraffic_0.6_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=64.9793663067473,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,16.8725044790687);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,14.4188879819959);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,14.6945817792411);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,16.5528725310247);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,52.4914742956354);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,54.1756759015722);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,51.7866841389757);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,45.4649990064289);
\path [draw=black, thick]
(axis cs:-0.2,14.3406430502828)
--(axis cs:-0.2,19.4043659078545);

\path [draw=black, thick]
(axis cs:0.8,12.1007250322733)
--(axis cs:0.8,16.7370509317184);

\path [draw=black, thick]
(axis cs:1.8,12.6202875692265)
--(axis cs:1.8,16.7688759892557);

\path [draw=black, thick]
(axis cs:2.8,14.0075196267888)
--(axis cs:2.8,19.0982254352606);

\path [draw=black, thick]
(axis cs:0.2,44.1036313859649)
--(axis cs:0.2,60.8793172053058);

\path [draw=black, thick]
(axis cs:1.2,46.4662410348137)
--(axis cs:1.2,61.8851107683307);

\path [draw=black, thick]
(axis cs:2.2,42.1817510202714)
--(axis cs:2.2,61.39161725768);

\path [draw=black, thick]
(axis cs:3.2,37.4193690087241)
--(axis cs:3.2,53.5106290041336);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOff/normOfferedTraffic_0.6_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=174.476053282807,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,166.166826480263);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,166.166826480263);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,166.167421875);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,166.167421875);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,166.167421875);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,166.167421875);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,166.167421875);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,166.167421875);
\path [draw=black, thick]
(axis cs:-0.2,166.165983167376)
--(axis cs:-0.2,166.16766979315);

\path [draw=black, thick]
(axis cs:0.8,166.165983167376)
--(axis cs:0.8,166.16766979315);

\path [draw=black, thick]
(axis cs:1.8,166.167421875)
--(axis cs:1.8,166.167421875);

\path [draw=black, thick]
(axis cs:2.8,166.167421875)
--(axis cs:2.8,166.167421875);

\path [draw=black, thick]
(axis cs:0.2,166.167421875)
--(axis cs:0.2,166.167421875);

\path [draw=black, thick]
(axis cs:1.2,166.167421875)
--(axis cs:1.2,166.167421875);

\path [draw=black, thick]
(axis cs:2.2,166.167421875)
--(axis cs:2.2,166.167421875);

\path [draw=black, thick]
(axis cs:3.2,166.167421875)
--(axis cs:3.2,166.167421875);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOff/normOfferedTraffic_0.7_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=65.9308471258414,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,21.3788352673242);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,18.6178937506921);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,18.9079802093298);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,21.0433216848955);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,53.1910504519526);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,53.3777531042151);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,53.6932384996039);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,44.7884861562176);
\path [draw=black, thick]
(axis cs:-0.2,18.3450527155845)
--(axis cs:-0.2,24.4126178190639);

\path [draw=black, thick]
(axis cs:0.8,15.6661001267331)
--(axis cs:0.8,21.569687374651);

\path [draw=black, thick]
(axis cs:1.8,16.2804211283154)
--(axis cs:1.8,21.5355392903442);

\path [draw=black, thick]
(axis cs:2.8,18.1502568551799)
--(axis cs:2.8,23.9363865146112);

\path [draw=black, thick]
(axis cs:0.2,44.8599388287941)
--(axis cs:0.2,61.522162075111);

\path [draw=black, thick]
(axis cs:1.2,45.1050808722623)
--(axis cs:1.2,61.6504253361678);

\path [draw=black, thick]
(axis cs:2.2,44.595194022216)
--(axis cs:2.2,62.7912829769919);

\path [draw=black, thick]
(axis cs:3.2,37.2571028456999)
--(axis cs:3.2,52.3198694667352);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOff/normOfferedTraffic_0.7_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=203.555243968841,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,193.861953125);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,193.861953125);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,193.861754660088);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,193.861953125);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,193.861953125);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,193.861953125);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,193.861953125);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,193.861953125);
\path [draw=black, thick]
(axis cs:-0.2,193.861953125)
--(axis cs:-0.2,193.861953125);

\path [draw=black, thick]
(axis cs:0.8,193.861953125)
--(axis cs:0.8,193.861953125);

\path [draw=black, thick]
(axis cs:1.8,193.861372206993)
--(axis cs:1.8,193.862137113182);

\path [draw=black, thick]
(axis cs:2.8,193.861953125)
--(axis cs:2.8,193.861953125);

\path [draw=black, thick]
(axis cs:0.2,193.861953125)
--(axis cs:0.2,193.861953125);

\path [draw=black, thick]
(axis cs:1.2,193.861953125)
--(axis cs:1.2,193.861953125);

\path [draw=black, thick]
(axis cs:2.2,193.861953125)
--(axis cs:2.2,193.861953125);

\path [draw=black, thick]
(axis cs:3.2,193.861953125)
--(axis cs:3.2,193.861953125);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOff/normOfferedTraffic_0.8_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=68.2709030667485,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,26.707506722635);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,23.5269182922783);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,23.7140766643399);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,26.8203574579155);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,53.716084399232);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,55.5052291164005);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,52.9586861262405);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,47.811678475411);
\path [draw=black, thick]
(axis cs:-0.2,23.3207231437205)
--(axis cs:-0.2,30.0942903015495);

\path [draw=black, thick]
(axis cs:0.8,20.2056664272123)
--(axis cs:0.8,26.8481701573443);

\path [draw=black, thick]
(axis cs:1.8,20.5486489612017)
--(axis cs:1.8,26.8795043674782);

\path [draw=black, thick]
(axis cs:2.8,23.3995181578491)
--(axis cs:2.8,30.2411967579819);

\path [draw=black, thick]
(axis cs:0.2,45.4493286987719)
--(axis cs:0.2,61.9828400996922);

\path [draw=black, thick]
(axis cs:1.2,45.9905505501834)
--(axis cs:1.2,65.0199076826176);

\path [draw=black, thick]
(axis cs:2.2,44.605504119526)
--(axis cs:2.2,61.311868132955);

\path [draw=black, thick]
(axis cs:3.2,39.7289895430791)
--(axis cs:3.2,55.894367407743);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOff/normOfferedTraffic_0.8_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=232.634512043853,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,221.5565625);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,221.555768640351);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,221.5565625);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,221.5565625);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,221.5565625);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,221.5565625);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,221.5565625);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,221.5565625);
\path [draw=black, thick]
(axis cs:-0.2,221.5565625)
--(axis cs:-0.2,221.5565625);

\path [draw=black, thick]
(axis cs:0.8,221.554859143699)
--(axis cs:0.8,221.556678137003);

\path [draw=black, thick]
(axis cs:1.8,221.5565625)
--(axis cs:1.8,221.5565625);

\path [draw=black, thick]
(axis cs:2.8,221.5565625)
--(axis cs:2.8,221.5565625);

\path [draw=black, thick]
(axis cs:0.2,221.5565625)
--(axis cs:0.2,221.5565625);

\path [draw=black, thick]
(axis cs:1.2,221.5565625)
--(axis cs:1.2,221.5565625);

\path [draw=black, thick]
(axis cs:2.2,221.5565625)
--(axis cs:2.2,221.5565625);

\path [draw=black, thick]
(axis cs:3.2,221.5565625)
--(axis cs:3.2,221.5565625);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOff/normOfferedTraffic_0.9_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=272.335250159695,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,230.425238775339);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,194.879050977726);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,206.141767447393);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,227.007895489905);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,53.922189482733);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,58.4216142490951);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,51.5581799313198);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,50.6042242340301);
\path [draw=black, thick]
(axis cs:-0.2,201.483572636682)
--(axis cs:-0.2,259.366904913996);

\path [draw=black, thick]
(axis cs:0.8,168.375544225616)
--(axis cs:0.8,221.382557729836);

\path [draw=black, thick]
(axis cs:1.8,178.098709545473)
--(axis cs:1.8,234.184825349313);

\path [draw=black, thick]
(axis cs:2.8,203.134430924661)
--(axis cs:2.8,250.881360055149);

\path [draw=black, thick]
(axis cs:0.2,45.7342134235717)
--(axis cs:0.2,62.1101655418943);

\path [draw=black, thick]
(axis cs:1.2,49.0097912395315)
--(axis cs:1.2,67.8334372586586);

\path [draw=black, thick]
(axis cs:2.2,43.8587489703051)
--(axis cs:2.2,59.2576108923345);

\path [draw=black, thick]
(axis cs:3.2,42.9755786278041)
--(axis cs:3.2,58.232869840256);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOff/normOfferedTraffic_0.9_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=261.7136484375,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,231.119546491228);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,233.985994462719);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,233.495803179825);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,229.611809594298);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,249.25109375);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,249.25109375);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,249.25109375);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,249.25109375);
\path [draw=black, thick]
(axis cs:-0.2,225.716147363026)
--(axis cs:-0.2,236.52294561943);

\path [draw=black, thick]
(axis cs:0.8,229.35514241387)
--(axis cs:0.8,238.616846511568);

\path [draw=black, thick]
(axis cs:1.8,228.629623108826)
--(axis cs:1.8,238.361983250823);

\path [draw=black, thick]
(axis cs:2.8,225.201983320085)
--(axis cs:2.8,234.021635868512);

\path [draw=black, thick]
(axis cs:0.2,249.25109375)
--(axis cs:0.2,249.25109375);

\path [draw=black, thick]
(axis cs:1.2,249.25109375)
--(axis cs:1.2,249.25109375);

\path [draw=black, thick]
(axis cs:2.2,249.25109375)
--(axis cs:2.2,249.25109375);

\path [draw=black, thick]
(axis cs:3.2,249.25109375)
--(axis cs:3.2,249.25109375);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOff/normOfferedTraffic_1_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.57, xmax=3.17,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=376.717715403737,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,341.014901008925);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,307.182894508386);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,325.831965743127);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,325.653222209939);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,nan);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,nan);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,nan);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,nan);
\path [draw=black, thick]
(axis cs:-0.2,323.251025442863)
--(axis cs:-0.2,358.778776574987);

\path [draw=black, thick]
(axis cs:0.8,288.408525930967)
--(axis cs:0.8,325.957263085804);

\path [draw=black, thick]
(axis cs:1.8,309.549447802428)
--(axis cs:1.8,342.114483683825);

\path [draw=black, thick]
(axis cs:2.8,304.725280514964)
--(axis cs:2.8,346.581163904914);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOff/normOfferedTraffic_1_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=299.779039059142,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,231.041826041667);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,240.246513322368);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,222.918387198465);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,224.270502220395);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,267.7141796875);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,203.093515625);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,193.8619921875);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,166.167421875);
\path [draw=black, thick]
(axis cs:-0.2,222.972606385796)
--(axis cs:-0.2,239.111045697537);

\path [draw=black, thick]
(axis cs:0.8,234.905676341071)
--(axis cs:0.8,245.587350303666);

\path [draw=black, thick]
(axis cs:1.8,214.919291939344)
--(axis cs:1.8,230.917482457586);

\path [draw=black, thick]
(axis cs:2.8,215.616609385908)
--(axis cs:2.8,232.924395054881);

\path [draw=black, thick]
(axis cs:0.2,249.924512652008)
--(axis cs:0.2,285.503846722992);

\path [draw=black, thick]
(axis cs:1.2,159.268189704491)
--(axis cs:1.2,246.918841545509);

\path [draw=black, thick]
(axis cs:2.2,148.446949919788)
--(axis cs:2.2,239.277034455212);

\path [draw=black, thick]
(axis cs:3.2,117.616699483104)
--(axis cs:3.2,214.718144266896);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOn/normOfferedTraffic_0.01_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=1.39457911434091,
ytick style={color=black},
ytick={0,0.2,0.4,0.6,0.8,1,1.2,1.4},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0,1.2,1.4}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,0.226930747699394);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,0.231270749948552);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,0.434469446693603);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,0.303242961215892);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,0.337156071169965);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,0.735178439533635);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,0.533218830447951);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,0.589716807320017);
\path [draw=black, thick]
(axis cs:-0.2,0.219527322051889)
--(axis cs:-0.2,0.234334173346899);

\path [draw=black, thick]
(axis cs:0.8,0.216723283413551)
--(axis cs:0.8,0.245818216483553);

\path [draw=black, thick]
(axis cs:1.8,0.103754829507518)
--(axis cs:1.8,0.765184063879688);

\path [draw=black, thick]
(axis cs:2.8,0.151793691874586)
--(axis cs:2.8,0.454692230557199);

\path [draw=black, thick]
(axis cs:0.2,0.230751065166986)
--(axis cs:0.2,0.443561077172944);

\path [draw=black, thick]
(axis cs:1.2,0.142186293980689)
--(axis cs:1.2,1.32817058508658);

\path [draw=black, thick]
(axis cs:2.2,0.113064036675267)
--(axis cs:2.2,0.953373624220634);

\path [draw=black, thick]
(axis cs:3.2,0.142739213049647)
--(axis cs:3.2,1.03669440159039);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOn/normOfferedTraffic_0.01_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=2.90792578125,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,2.769453125);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,2.769453125);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,2.769453125);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,2.769453125);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,2.769453125);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,2.769453125);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,2.769453125);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,2.769453125);
\path [draw=black, thick]
(axis cs:-0.2,2.769453125)
--(axis cs:-0.2,2.769453125);

\path [draw=black, thick]
(axis cs:0.8,2.769453125)
--(axis cs:0.8,2.769453125);

\path [draw=black, thick]
(axis cs:1.8,2.769453125)
--(axis cs:1.8,2.769453125);

\path [draw=black, thick]
(axis cs:2.8,2.769453125)
--(axis cs:2.8,2.769453125);

\path [draw=black, thick]
(axis cs:0.2,2.769453125)
--(axis cs:0.2,2.769453125);

\path [draw=black, thick]
(axis cs:1.2,2.769453125)
--(axis cs:1.2,2.769453125);

\path [draw=black, thick]
(axis cs:2.2,2.769453125)
--(axis cs:2.2,2.769453125);

\path [draw=black, thick]
(axis cs:3.2,2.769453125)
--(axis cs:3.2,2.769453125);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOn/normOfferedTraffic_0.1_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=4.23490008335835,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,1.65743850384523);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,1.7046068453761);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,1.75763083584366);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,2.10927853416359);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,1.81463089324544);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,2.88011407179739);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,2.24214759433219);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,2.61851120225749);
\path [draw=black, thick]
(axis cs:-0.2,1.46310592610005)
--(axis cs:-0.2,1.8517710815904);

\path [draw=black, thick]
(axis cs:0.8,1.3857396923025)
--(axis cs:0.8,2.02347399844971);

\path [draw=black, thick]
(axis cs:1.8,1.39952052370638)
--(axis cs:1.8,2.11574114798094);

\path [draw=black, thick]
(axis cs:2.8,1.4699406965023)
--(axis cs:2.8,2.74861637182489);

\path [draw=black, thick]
(axis cs:0.2,1.54667274494171)
--(axis cs:0.2,2.08258904154918);

\path [draw=black, thick]
(axis cs:1.2,1.72698996896778)
--(axis cs:1.2,4.033238174627);

\path [draw=black, thick]
(axis cs:2.2,1.57961415107176)
--(axis cs:2.2,2.90468103759262);

\path [draw=black, thick]
(axis cs:3.2,1.43196205810519)
--(axis cs:3.2,3.80506034640979);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOn/normOfferedTraffic_0.1_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=29.0792578125,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,27.69453125);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,27.69453125);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,27.69453125);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,27.69453125);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,27.69453125);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,27.69453125);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,27.69453125);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,27.69453125);
\path [draw=black, thick]
(axis cs:-0.2,27.69453125)
--(axis cs:-0.2,27.69453125);

\path [draw=black, thick]
(axis cs:0.8,27.69453125)
--(axis cs:0.8,27.69453125);

\path [draw=black, thick]
(axis cs:1.8,27.69453125)
--(axis cs:1.8,27.69453125);

\path [draw=black, thick]
(axis cs:2.8,27.69453125)
--(axis cs:2.8,27.69453125);

\path [draw=black, thick]
(axis cs:0.2,27.69453125)
--(axis cs:0.2,27.69453125);

\path [draw=black, thick]
(axis cs:1.2,27.69453125)
--(axis cs:1.2,27.69453125);

\path [draw=black, thick]
(axis cs:2.2,27.69453125)
--(axis cs:2.2,27.69453125);

\path [draw=black, thick]
(axis cs:3.2,27.69453125)
--(axis cs:3.2,27.69453125);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOn/normOfferedTraffic_0.2_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=8.41171666666743,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,3.82546063341778);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,3.56199215312244);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,3.42685280430678);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,3.94955547020377);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,4.7509161420593);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,5.76022010833814);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,5.96253454945793);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,6.19073641134869);
\path [draw=black, thick]
(axis cs:-0.2,3.32614005253829)
--(axis cs:-0.2,4.32478121429728);

\path [draw=black, thick]
(axis cs:0.8,2.96557777425465)
--(axis cs:0.8,4.15840653199023);

\path [draw=black, thick]
(axis cs:1.8,2.94804301294666)
--(axis cs:1.8,3.90566259566691);

\path [draw=black, thick]
(axis cs:2.8,3.11629570420001)
--(axis cs:2.8,4.78281523620753);

\path [draw=black, thick]
(axis cs:0.2,3.29924044470752)
--(axis cs:0.2,6.20259183941108);

\path [draw=black, thick]
(axis cs:1.2,3.9107576147803)
--(axis cs:1.2,7.60968260189599);

\path [draw=black, thick]
(axis cs:2.2,4.37132734644055)
--(axis cs:2.2,7.55374175247531);

\path [draw=black, thick]
(axis cs:3.2,4.37031409253792)
--(axis cs:3.2,8.01115873015946);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOn/normOfferedTraffic_0.2_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=58.15859765625,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,55.389140625);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,55.389140625);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,55.389140625);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,55.389140625);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,55.389140625);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,55.389140625);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,55.389140625);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,55.389140625);
\path [draw=black, thick]
(axis cs:-0.2,55.389140625)
--(axis cs:-0.2,55.389140625);

\path [draw=black, thick]
(axis cs:0.8,55.389140625)
--(axis cs:0.8,55.389140625);

\path [draw=black, thick]
(axis cs:1.8,55.389140625)
--(axis cs:1.8,55.389140625);

\path [draw=black, thick]
(axis cs:2.8,55.389140625)
--(axis cs:2.8,55.389140625);

\path [draw=black, thick]
(axis cs:0.2,55.389140625)
--(axis cs:0.2,55.389140625);

\path [draw=black, thick]
(axis cs:1.2,55.389140625)
--(axis cs:1.2,55.389140625);

\path [draw=black, thick]
(axis cs:2.2,55.389140625)
--(axis cs:2.2,55.389140625);

\path [draw=black, thick]
(axis cs:3.2,55.389140625)
--(axis cs:3.2,55.389140625);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOn/normOfferedTraffic_0.3_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=16.841718678864,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,6.73418922055258);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,5.82504579760884);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,5.54711542763041);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,6.35723947922322);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,8.48517495311468);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,10.3207298854883);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,9.9785989889281);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,12.9971815130019);
\path [draw=black, thick]
(axis cs:-0.2,5.594332603322)
--(axis cs:-0.2,7.87404583778316);

\path [draw=black, thick]
(axis cs:0.8,4.90360289255775)
--(axis cs:0.8,6.74648870265993);

\path [draw=black, thick]
(axis cs:1.8,4.82312316873049)
--(axis cs:1.8,6.27110768653032);

\path [draw=black, thick]
(axis cs:2.8,5.30752594518268)
--(axis cs:2.8,7.40695301326376);

\path [draw=black, thick]
(axis cs:0.2,6.10512445679834)
--(axis cs:0.2,10.865225449431);

\path [draw=black, thick]
(axis cs:1.2,7.80144150816557)
--(axis cs:1.2,12.8400182628111);

\path [draw=black, thick]
(axis cs:2.2,7.65037852827076)
--(axis cs:2.2,12.3068194495854);

\path [draw=black, thick]
(axis cs:3.2,9.95463095089523)
--(axis cs:3.2,16.0397320751086);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOn/normOfferedTraffic_0.3_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=87.23785546875,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,83.083671875);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,83.083671875);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,83.083671875);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,83.083671875);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,83.083671875);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,83.083671875);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,83.083671875);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,83.083671875);
\path [draw=black, thick]
(axis cs:-0.2,83.083671875)
--(axis cs:-0.2,83.083671875);

\path [draw=black, thick]
(axis cs:0.8,83.083671875)
--(axis cs:0.8,83.083671875);

\path [draw=black, thick]
(axis cs:1.8,83.083671875)
--(axis cs:1.8,83.083671875);

\path [draw=black, thick]
(axis cs:2.8,83.083671875)
--(axis cs:2.8,83.083671875);

\path [draw=black, thick]
(axis cs:0.2,83.083671875)
--(axis cs:0.2,83.083671875);

\path [draw=black, thick]
(axis cs:1.2,83.083671875)
--(axis cs:1.2,83.083671875);

\path [draw=black, thick]
(axis cs:2.2,83.083671875)
--(axis cs:2.2,83.083671875);

\path [draw=black, thick]
(axis cs:3.2,83.083671875)
--(axis cs:3.2,83.083671875);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOn/normOfferedTraffic_0.4_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=24.4989399228889,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,9.75323120633818);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,8.1227712881128);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,8.14574503454991);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,9.21475662012733);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,13.1442020794729);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,16.2563968007493);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,14.216209073949);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,18.9721491384889);
\path [draw=black, thick]
(axis cs:-0.2,8.15120118746336)
--(axis cs:-0.2,11.355261225213);

\path [draw=black, thick]
(axis cs:0.8,6.89809221412742)
--(axis cs:0.8,9.34745036209819);

\path [draw=black, thick]
(axis cs:1.8,6.95783439137244)
--(axis cs:1.8,9.33365567772738);

\path [draw=black, thick]
(axis cs:2.8,7.83207256362724)
--(axis cs:2.8,10.5974406766274);

\path [draw=black, thick]
(axis cs:0.2,10.1343963314165)
--(axis cs:0.2,16.1540078275293);

\path [draw=black, thick]
(axis cs:1.2,12.9412834934473)
--(axis cs:1.2,19.5715101080512);

\path [draw=black, thick]
(axis cs:2.2,11.2611872276712)
--(axis cs:2.2,17.1712309202267);

\path [draw=black, thick]
(axis cs:3.2,14.6119745408931)
--(axis cs:3.2,23.3323237360846);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOn/normOfferedTraffic_0.4_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=116.3171953125,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,110.77828125);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,110.77828125);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,110.77828125);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,110.77828125);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,110.77828125);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,110.77828125);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,110.77828125);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,110.77828125);
\path [draw=black, thick]
(axis cs:-0.2,110.77828125)
--(axis cs:-0.2,110.77828125);

\path [draw=black, thick]
(axis cs:0.8,110.77828125)
--(axis cs:0.8,110.77828125);

\path [draw=black, thick]
(axis cs:1.8,110.77828125)
--(axis cs:1.8,110.77828125);

\path [draw=black, thick]
(axis cs:2.8,110.77828125)
--(axis cs:2.8,110.77828125);

\path [draw=black, thick]
(axis cs:0.2,110.77828125)
--(axis cs:0.2,110.77828125);

\path [draw=black, thick]
(axis cs:1.2,110.77828125)
--(axis cs:1.2,110.77828125);

\path [draw=black, thick]
(axis cs:2.2,110.77828125)
--(axis cs:2.2,110.77828125);

\path [draw=black, thick]
(axis cs:3.2,110.77828125)
--(axis cs:3.2,110.77828125);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOn/normOfferedTraffic_0.5_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=32.0498759888953,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,12.9808058136175);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,11.0727569744902);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,11.0348870603131);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,12.7420613773217);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,19.8100280234967);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,23.4086187647668);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,20.1055430678027);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,25.2216418046237);
\path [draw=black, thick]
(axis cs:-0.2,10.9768594320539)
--(axis cs:-0.2,14.9847521951811);

\path [draw=black, thick]
(axis cs:0.8,9.37322605767418)
--(axis cs:0.8,12.7722878913063);

\path [draw=black, thick]
(axis cs:1.8,9.42777964322607)
--(axis cs:1.8,12.6419944774001);

\path [draw=black, thick]
(axis cs:2.8,10.7014208815343)
--(axis cs:2.8,14.7827018731091);

\path [draw=black, thick]
(axis cs:0.2,15.3605654527691)
--(axis cs:0.2,24.2594905942243);

\path [draw=black, thick]
(axis cs:1.2,19.3217525860412)
--(axis cs:1.2,27.4954849434925);

\path [draw=black, thick]
(axis cs:2.2,16.0096203216754)
--(axis cs:2.2,24.2014658139299);

\path [draw=black, thick]
(axis cs:3.2,19.919592191252)
--(axis cs:3.2,30.5236914179955);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOn/normOfferedTraffic_0.5_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=145.396839500183,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,138.472571600877);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,138.47261129386);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,138.47261129386);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,138.4728125);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,138.472614035088);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,138.4728125);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,138.472614035088);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,138.472415570175);
\path [draw=black, thick]
(axis cs:-0.2,138.472107374662)
--(axis cs:-0.2,138.473035827092);

\path [draw=black, thick]
(axis cs:0.8,138.472223558264)
--(axis cs:0.8,138.472999029456);

\path [draw=black, thick]
(axis cs:1.8,138.472223558264)
--(axis cs:1.8,138.472999029456);

\path [draw=black, thick]
(axis cs:2.8,138.4728125)
--(axis cs:2.8,138.4728125);

\path [draw=black, thick]
(axis cs:0.2,138.472231581993)
--(axis cs:0.2,138.472996488182);

\path [draw=black, thick]
(axis cs:1.2,138.4728125)
--(axis cs:1.2,138.4728125);

\path [draw=black, thick]
(axis cs:2.2,138.472231581993)
--(axis cs:2.2,138.472996488182);

\path [draw=black, thick]
(axis cs:3.2,138.471650663986)
--(axis cs:3.2,138.473180476365);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOn/normOfferedTraffic_0.6_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=39.285451519319,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,16.8725044790687);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,14.4188879819959);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,14.6945817792411);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,16.5528725310247);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,27.8391538628913);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,31.6136920959056);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,29.8174743570176);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,31.0938015354393);
\path [draw=black, thick]
(axis cs:-0.2,14.3406430502828)
--(axis cs:-0.2,19.4043659078545);

\path [draw=black, thick]
(axis cs:0.8,12.1007250322733)
--(axis cs:0.8,16.7370509317184);

\path [draw=black, thick]
(axis cs:1.8,12.6202875692265)
--(axis cs:1.8,16.7688759892557);

\path [draw=black, thick]
(axis cs:2.8,14.0075196267888)
--(axis cs:2.8,19.0982254352606);

\path [draw=black, thick]
(axis cs:0.2,22.5441664279859)
--(axis cs:0.2,33.1341412977967);

\path [draw=black, thick]
(axis cs:1.2,26.3656458696111)
--(axis cs:1.2,36.8617383222);

\path [draw=black, thick]
(axis cs:2.2,23.8443375541892)
--(axis cs:2.2,35.7906111598461);

\path [draw=black, thick]
(axis cs:3.2,24.7728873381938)
--(axis cs:3.2,37.4147157326848);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOn/normOfferedTraffic_0.6_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=174.476053282807,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,166.166826480263);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,166.166826480263);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,166.167421875);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,166.167421875);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,166.167421875);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,166.167223410088);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,166.167223410088);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,166.167421875);
\path [draw=black, thick]
(axis cs:-0.2,166.165983167376)
--(axis cs:-0.2,166.16766979315);

\path [draw=black, thick]
(axis cs:0.8,166.165983167376)
--(axis cs:0.8,166.16766979315);

\path [draw=black, thick]
(axis cs:1.8,166.167421875)
--(axis cs:1.8,166.167421875);

\path [draw=black, thick]
(axis cs:2.8,166.167421875)
--(axis cs:2.8,166.167421875);

\path [draw=black, thick]
(axis cs:0.2,166.167421875)
--(axis cs:0.2,166.167421875);

\path [draw=black, thick]
(axis cs:1.2,166.166840956993)
--(axis cs:1.2,166.167605863183);

\path [draw=black, thick]
(axis cs:2.2,166.166840956993)
--(axis cs:2.2,166.167605863183);

\path [draw=black, thick]
(axis cs:3.2,166.167421875)
--(axis cs:3.2,166.167421875);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOn/normOfferedTraffic_0.7_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=48.5370024627756,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,21.3788352673242);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,18.6178937506921);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,18.9079802093298);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,21.0433216848955);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,37.7067672707495);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,39.4899223493209);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,39.5937026160515);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,36.4487607494698);
\path [draw=black, thick]
(axis cs:-0.2,18.3450527155845)
--(axis cs:-0.2,24.4126178190639);

\path [draw=black, thick]
(axis cs:0.8,15.6661001267331)
--(axis cs:0.8,21.569687374651);

\path [draw=black, thick]
(axis cs:1.8,16.2804211283154)
--(axis cs:1.8,21.5355392903442);

\path [draw=black, thick]
(axis cs:2.8,18.1502568551799)
--(axis cs:2.8,23.9363865146112);

\path [draw=black, thick]
(axis cs:0.2,31.5003136040234)
--(axis cs:0.2,43.9132209374757);

\path [draw=black, thick]
(axis cs:1.2,32.7791649893883)
--(axis cs:1.2,46.2006797092535);

\path [draw=black, thick]
(axis cs:2.2,32.9616886008881)
--(axis cs:2.2,46.2257166312149);

\path [draw=black, thick]
(axis cs:3.2,29.8682822995415)
--(axis cs:3.2,43.0292391993981);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOn/normOfferedTraffic_0.7_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=203.555243968841,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,193.861953125);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,193.861953125);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,193.861754660088);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,193.861953125);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,193.861556195175);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,193.861953125);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,193.861953125);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,193.861953125);
\path [draw=black, thick]
(axis cs:-0.2,193.861953125)
--(axis cs:-0.2,193.861953125);

\path [draw=black, thick]
(axis cs:0.8,193.861953125)
--(axis cs:0.8,193.861953125);

\path [draw=black, thick]
(axis cs:1.8,193.861372206993)
--(axis cs:1.8,193.862137113182);

\path [draw=black, thick]
(axis cs:2.8,193.861953125)
--(axis cs:2.8,193.861953125);

\path [draw=black, thick]
(axis cs:0.2,193.86102473198)
--(axis cs:0.2,193.86208765837);

\path [draw=black, thick]
(axis cs:1.2,193.861953125)
--(axis cs:1.2,193.861953125);

\path [draw=black, thick]
(axis cs:2.2,193.861953125)
--(axis cs:2.2,193.861953125);

\path [draw=black, thick]
(axis cs:3.2,193.861953125)
--(axis cs:3.2,193.861953125);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOn/normOfferedTraffic_0.8_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=61.2341596965448,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,26.707506722635);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,23.5269182922783);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,23.7140766643399);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,26.8203574579155);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,45.2940427976077);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,50.320781047184);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,45.5690751183586);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,42.7568752531177);
\path [draw=black, thick]
(axis cs:-0.2,23.3207231437206)
--(axis cs:-0.2,30.0942903015495);

\path [draw=black, thick]
(axis cs:0.8,20.2056664272123)
--(axis cs:0.8,26.8481701573443);

\path [draw=black, thick]
(axis cs:1.8,20.5486489612017)
--(axis cs:1.8,26.8795043674782);

\path [draw=black, thick]
(axis cs:2.8,23.3995181578491)
--(axis cs:2.8,30.2411967579819);

\path [draw=black, thick]
(axis cs:0.2,38.1671691069671)
--(axis cs:0.2,52.4209164882482);

\path [draw=black, thick]
(axis cs:1.2,42.3233147643253)
--(axis cs:1.2,58.3182473300427);

\path [draw=black, thick]
(axis cs:2.2,38.0435789371653)
--(axis cs:2.2,53.0945712995519);

\path [draw=black, thick]
(axis cs:3.2,35.503078705929)
--(axis cs:3.2,50.0106718003065);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOn/normOfferedTraffic_0.8_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=232.634583812592,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,221.5565625);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,221.555768640351);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,221.5565625);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,221.5565625);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,221.5565625);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,221.556364035088);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,221.556364035088);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,221.5565625);
\path [draw=black, thick]
(axis cs:-0.2,221.5565625)
--(axis cs:-0.2,221.5565625);

\path [draw=black, thick]
(axis cs:0.8,221.554859143699)
--(axis cs:0.8,221.556678137003);

\path [draw=black, thick]
(axis cs:1.8,221.5565625)
--(axis cs:1.8,221.5565625);

\path [draw=black, thick]
(axis cs:2.8,221.5565625)
--(axis cs:2.8,221.5565625);

\path [draw=black, thick]
(axis cs:0.2,221.5565625)
--(axis cs:0.2,221.5565625);

\path [draw=black, thick]
(axis cs:1.2,221.555981581993)
--(axis cs:1.2,221.556746488182);

\path [draw=black, thick]
(axis cs:2.2,221.555981581993)
--(axis cs:2.2,221.556746488182);

\path [draw=black, thick]
(axis cs:3.2,221.5565625)
--(axis cs:3.2,221.5565625);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOn/normOfferedTraffic_0.9_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.57, xmax=3.17,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=272.335250159695,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,230.425238775339);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,194.879050977726);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,206.141767447393);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,227.007895489905);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,52.5330530552601);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,55.534656490149);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,49.0275388465062);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,nan);
\path [draw=black, thick]
(axis cs:-0.2,201.483572636682)
--(axis cs:-0.2,259.366904913996);

\path [draw=black, thick]
(axis cs:0.8,168.375544225616)
--(axis cs:0.8,221.382557729836);

\path [draw=black, thick]
(axis cs:1.8,178.098709545473)
--(axis cs:1.8,234.184825349314);

\path [draw=black, thick]
(axis cs:2.8,203.134430924661)
--(axis cs:2.8,250.881360055149);

\path [draw=black, thick]
(axis cs:0.2,44.5740260124155)
--(axis cs:0.2,60.4920800981047);

\path [draw=black, thick]
(axis cs:1.2,46.0257306155279)
--(axis cs:1.2,65.0435823647701);

\path [draw=black, thick]
(axis cs:2.2,41.1757294917701)
--(axis cs:2.2,56.8793482012423);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOn/normOfferedTraffic_0.9_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=269.800870639336,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,231.119546491228);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,233.985994462719);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,233.495803179825);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,229.611809594298);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,249.25109375);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,249.25109375);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,249.250696820176);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,240.942525493421);
\path [draw=black, thick]
(axis cs:-0.2,225.716147363026)
--(axis cs:-0.2,236.52294561943);

\path [draw=black, thick]
(axis cs:0.8,229.35514241387)
--(axis cs:0.8,238.616846511568);

\path [draw=black, thick]
(axis cs:1.8,228.629623108826)
--(axis cs:1.8,238.361983250823);

\path [draw=black, thick]
(axis cs:2.8,225.201983320085)
--(axis cs:2.8,234.021635868512);

\path [draw=black, thick]
(axis cs:0.2,249.25109375)
--(axis cs:0.2,249.25109375);

\path [draw=black, thick]
(axis cs:1.2,249.25109375)
--(axis cs:1.2,249.25109375);

\path [draw=black, thick]
(axis cs:2.2,249.249931913986)
--(axis cs:2.2,249.251461726365);

\path [draw=black, thick]
(axis cs:3.2,224.931840854142)
--(axis cs:3.2,256.953210132701);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOn/normOfferedTraffic_1_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.57, xmax=3.17,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=377.247362908746,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,341.55100341048);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,304.304962535876);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,327.917436313379);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,326.826158209181);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,nan);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,nan);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,nan);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,nan);
\path [draw=black, thick]
(axis cs:-0.2,323.818804050725)
--(axis cs:-0.2,359.283202770234);

\path [draw=black, thick]
(axis cs:0.8,285.911082184394)
--(axis cs:0.8,322.698842887359);

\path [draw=black, thick]
(axis cs:1.8,313.324972103013)
--(axis cs:1.8,342.509900523744);

\path [draw=black, thick]
(axis cs:2.8,305.618650177077)
--(axis cs:2.8,348.033666241284);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOff_cbapOn/normOfferedTraffic_1_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=299.778816827856,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,230.754642927632);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,239.833700794956);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,223.1037578125);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,224.788255235746);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,267.713981222588);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,203.093317160088);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,193.8619921875);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,166.167421875);
\path [draw=black, thick]
(axis cs:-0.2,222.691308829882)
--(axis cs:-0.2,238.817977025381);

\path [draw=black, thick]
(axis cs:0.8,234.453711286262)
--(axis cs:0.8,245.21369030365);

\path [draw=black, thick]
(axis cs:1.8,215.025005356039)
--(axis cs:1.8,231.182510268962);

\path [draw=black, thick]
(axis cs:2.8,216.29702363257)
--(axis cs:2.8,233.279486838921);

\path [draw=black, thick]
(axis cs:0.2,249.924327371027)
--(axis cs:0.2,285.503635074148);

\path [draw=black, thick]
(axis cs:1.2,159.268034064456)
--(axis cs:1.2,246.91860025572);

\path [draw=black, thick]
(axis cs:2.2,148.446949919788)
--(axis cs:2.2,239.277034455212);

\path [draw=black, thick]
(axis cs:3.2,117.616699483104)
--(axis cs:3.2,214.718144266896);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOn/normOfferedTraffic_0.01_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=0.803443267073672,
ytick style={color=black},
ytick={0,0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9},
yticklabels={0.0,0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,0.226930747699394);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,0.231270749948552);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,0.434469446693603);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,0.303242961215892);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,0.193731219069189);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,0.191625911370724);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,0.202227877622634);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,0.195987678460853);
\path [draw=black, thick]
(axis cs:-0.2,0.219527322051889)
--(axis cs:-0.2,0.234334173346899);

\path [draw=black, thick]
(axis cs:0.8,0.216723283413551)
--(axis cs:0.8,0.245818216483553);

\path [draw=black, thick]
(axis cs:1.8,0.103754829507518)
--(axis cs:1.8,0.765184063879688);

\path [draw=black, thick]
(axis cs:2.8,0.151793691874586)
--(axis cs:2.8,0.454692230557199);

\path [draw=black, thick]
(axis cs:0.2,0.184066064648084)
--(axis cs:0.2,0.203396373490293);

\path [draw=black, thick]
(axis cs:1.2,0.184814309591235)
--(axis cs:1.2,0.198437513150212);

\path [draw=black, thick]
(axis cs:2.2,0.193798763914865)
--(axis cs:2.2,0.210656991330403);

\path [draw=black, thick]
(axis cs:3.2,0.186126684096989)
--(axis cs:3.2,0.205848672824717);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOn/normOfferedTraffic_0.01_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=2.90792578125,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,2.769453125);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,2.769453125);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,2.769453125);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,2.769453125);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,2.769453125);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,2.769453125);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,2.769453125);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,2.769453125);
\path [draw=black, thick]
(axis cs:-0.2,2.769453125)
--(axis cs:-0.2,2.769453125);

\path [draw=black, thick]
(axis cs:0.8,2.769453125)
--(axis cs:0.8,2.769453125);

\path [draw=black, thick]
(axis cs:1.8,2.769453125)
--(axis cs:1.8,2.769453125);

\path [draw=black, thick]
(axis cs:2.8,2.769453125)
--(axis cs:2.8,2.769453125);

\path [draw=black, thick]
(axis cs:0.2,2.769453125)
--(axis cs:0.2,2.769453125);

\path [draw=black, thick]
(axis cs:1.2,2.769453125)
--(axis cs:1.2,2.769453125);

\path [draw=black, thick]
(axis cs:2.2,2.769453125)
--(axis cs:2.2,2.769453125);

\path [draw=black, thick]
(axis cs:3.2,2.769453125)
--(axis cs:3.2,2.769453125);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOn/normOfferedTraffic_0.1_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=2.88604719041613,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,1.65743850384523);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,1.7046068453761);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,1.75763083584366);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,2.1092785341636);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,1.30972825326854);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,1.30950797724991);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,1.31061720843278);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,1.30995877310843);
\path [draw=black, thick]
(axis cs:-0.2,1.46310592610005)
--(axis cs:-0.2,1.8517710815904);

\path [draw=black, thick]
(axis cs:0.8,1.38573969230249)
--(axis cs:0.8,2.02347399844971);

\path [draw=black, thick]
(axis cs:1.8,1.39952052370638)
--(axis cs:1.8,2.11574114798094);

\path [draw=black, thick]
(axis cs:2.8,1.4699406965023)
--(axis cs:2.8,2.74861637182489);

\path [draw=black, thick]
(axis cs:0.2,1.3087164993104)
--(axis cs:0.2,1.31074000722668);

\path [draw=black, thick]
(axis cs:1.2,1.3087944336675)
--(axis cs:1.2,1.31022152083233);

\path [draw=black, thick]
(axis cs:2.2,1.30973427971106)
--(axis cs:2.2,1.31150013715451);

\path [draw=black, thick]
(axis cs:3.2,1.30892465312426)
--(axis cs:3.2,1.31099289309261);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOn/normOfferedTraffic_0.1_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=29.0792578125,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,27.69453125);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,27.69453125);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,27.69453125);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,27.69453125);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,27.69453125);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,27.69453125);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,27.69453125);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,27.69453125);
\path [draw=black, thick]
(axis cs:-0.2,27.69453125)
--(axis cs:-0.2,27.69453125);

\path [draw=black, thick]
(axis cs:0.8,27.69453125)
--(axis cs:0.8,27.69453125);

\path [draw=black, thick]
(axis cs:1.8,27.69453125)
--(axis cs:1.8,27.69453125);

\path [draw=black, thick]
(axis cs:2.8,27.69453125)
--(axis cs:2.8,27.69453125);

\path [draw=black, thick]
(axis cs:0.2,27.69453125)
--(axis cs:0.2,27.69453125);

\path [draw=black, thick]
(axis cs:1.2,27.69453125)
--(axis cs:1.2,27.69453125);

\path [draw=black, thick]
(axis cs:2.2,27.69453125)
--(axis cs:2.2,27.69453125);

\path [draw=black, thick]
(axis cs:3.2,27.69453125)
--(axis cs:3.2,27.69453125);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOn/normOfferedTraffic_0.2_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=5.02195599801791,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,3.82546063341778);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,3.56199215312244);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,3.42685280430678);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,3.94955547020377);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,2.59165537932201);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,2.59154508236487);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,2.59210049716757);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,2.59176766097227);
\path [draw=black, thick]
(axis cs:-0.2,3.32614005253829)
--(axis cs:-0.2,4.32478121429728);

\path [draw=black, thick]
(axis cs:0.8,2.96557777425465)
--(axis cs:0.8,4.15840653199023);

\path [draw=black, thick]
(axis cs:1.8,2.94804301294666)
--(axis cs:1.8,3.90566259566691);

\path [draw=black, thick]
(axis cs:2.8,3.11629570420001)
--(axis cs:2.8,4.78281523620753);

\path [draw=black, thick]
(axis cs:0.2,2.59114846288785)
--(axis cs:0.2,2.59216229575618);

\path [draw=black, thick]
(axis cs:1.2,2.59118729188134)
--(axis cs:1.2,2.5919028728484);

\path [draw=black, thick]
(axis cs:2.2,2.59165780656256)
--(axis cs:2.2,2.59254318777258);

\path [draw=black, thick]
(axis cs:3.2,2.59124847808939)
--(axis cs:3.2,2.59228684385515);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOn/normOfferedTraffic_0.2_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=58.15859765625,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,55.389140625);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,55.389140625);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,55.389140625);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,55.389140625);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,55.389140625);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,55.389140625);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,55.389140625);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,55.389140625);
\path [draw=black, thick]
(axis cs:-0.2,55.389140625)
--(axis cs:-0.2,55.389140625);

\path [draw=black, thick]
(axis cs:0.8,55.389140625)
--(axis cs:0.8,55.389140625);

\path [draw=black, thick]
(axis cs:1.8,55.389140625)
--(axis cs:1.8,55.389140625);

\path [draw=black, thick]
(axis cs:2.8,55.389140625)
--(axis cs:2.8,55.389140625);

\path [draw=black, thick]
(axis cs:0.2,55.389140625)
--(axis cs:0.2,55.389140625);

\path [draw=black, thick]
(axis cs:1.2,55.389140625)
--(axis cs:1.2,55.389140625);

\path [draw=black, thick]
(axis cs:2.2,55.389140625)
--(axis cs:2.2,55.389140625);

\path [draw=black, thick]
(axis cs:3.2,55.389140625)
--(axis cs:3.2,55.389140625);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOn/normOfferedTraffic_0.3_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=8.26774812967232,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,6.73418922055258);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,5.82504579760884);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,5.54711542763041);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,6.35723947922322);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,3.87536472921494);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,3.87529116252043);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,3.87566161699947);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,3.87543752076502);
\path [draw=black, thick]
(axis cs:-0.2,5.594332603322)
--(axis cs:-0.2,7.87404583778317);

\path [draw=black, thick]
(axis cs:0.8,4.90360289255775)
--(axis cs:0.8,6.74648870265993);

\path [draw=black, thick]
(axis cs:1.8,4.82312316873049)
--(axis cs:1.8,6.27110768653032);

\path [draw=black, thick]
(axis cs:2.8,5.30752594518268)
--(axis cs:2.8,7.40695301326376);

\path [draw=black, thick]
(axis cs:0.2,3.87502641162278)
--(axis cs:0.2,3.8757030468071);

\path [draw=black, thick]
(axis cs:1.2,3.87505217927212)
--(axis cs:1.2,3.87553014576874);

\path [draw=black, thick]
(axis cs:2.2,3.87536595044222)
--(axis cs:2.2,3.87595728355672);

\path [draw=black, thick]
(axis cs:3.2,3.87509030475)
--(axis cs:3.2,3.87578473678003);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOn/normOfferedTraffic_0.3_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=87.23785546875,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,83.083671875);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,83.083671875);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,83.083671875);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,83.083671875);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,83.083671875);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,83.083671875);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,83.083671875);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,83.083671875);
\path [draw=black, thick]
(axis cs:-0.2,83.083671875)
--(axis cs:-0.2,83.083671875);

\path [draw=black, thick]
(axis cs:0.8,83.083671875)
--(axis cs:0.8,83.083671875);

\path [draw=black, thick]
(axis cs:1.8,83.083671875)
--(axis cs:1.8,83.083671875);

\path [draw=black, thick]
(axis cs:2.8,83.083671875)
--(axis cs:2.8,83.083671875);

\path [draw=black, thick]
(axis cs:0.2,83.083671875)
--(axis cs:0.2,83.083671875);

\path [draw=black, thick]
(axis cs:1.2,83.083671875)
--(axis cs:1.2,83.083671875);

\path [draw=black, thick]
(axis cs:2.2,83.083671875)
--(axis cs:2.2,83.083671875);

\path [draw=black, thick]
(axis cs:3.2,83.083671875)
--(axis cs:3.2,83.083671875);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOn/normOfferedTraffic_0.4_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=11.9230242864736,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,9.75323120633817);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,8.12866454512199);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,8.14635947705229);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,9.20954462304285);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,5.15953792546835);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,5.15948273716673);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,5.15976064480309);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,5.15959095740812);
\path [draw=black, thick]
(axis cs:-0.2,8.15120118746335)
--(axis cs:-0.2,11.355261225213);

\path [draw=black, thick]
(axis cs:0.8,6.90124508770484)
--(axis cs:0.8,9.35608400253913);

\path [draw=black, thick]
(axis cs:1.8,6.95847051225992)
--(axis cs:1.8,9.33424844184466);

\path [draw=black, thick]
(axis cs:2.8,7.82754457974607)
--(axis cs:2.8,10.5915446663396);

\path [draw=black, thick]
(axis cs:0.2,5.15928396533576)
--(axis cs:0.2,5.15979188560093);

\path [draw=black, thick]
(axis cs:1.2,5.15930319671632)
--(axis cs:1.2,5.15966227761715);

\path [draw=black, thick]
(axis cs:2.2,5.15953854040539)
--(axis cs:2.2,5.15998274920079);

\path [draw=black, thick]
(axis cs:3.2,5.15932978069513)
--(axis cs:3.2,5.1598521341211);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOn/normOfferedTraffic_0.4_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=116.3171953125,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,110.77828125);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,110.77828125);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,110.77828125);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,110.77828125);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,110.77828125);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,110.77828125);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,110.77828125);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,110.77828125);
\path [draw=black, thick]
(axis cs:-0.2,110.77828125)
--(axis cs:-0.2,110.77828125);

\path [draw=black, thick]
(axis cs:0.8,110.77828125)
--(axis cs:0.8,110.77828125);

\path [draw=black, thick]
(axis cs:1.8,110.77828125)
--(axis cs:1.8,110.77828125);

\path [draw=black, thick]
(axis cs:2.8,110.77828125)
--(axis cs:2.8,110.77828125);

\path [draw=black, thick]
(axis cs:0.2,110.77828125)
--(axis cs:0.2,110.77828125);

\path [draw=black, thick]
(axis cs:1.2,110.77828125)
--(axis cs:1.2,110.77828125);

\path [draw=black, thick]
(axis cs:2.2,110.77828125)
--(axis cs:2.2,110.77828125);

\path [draw=black, thick]
(axis cs:3.2,110.77828125)
--(axis cs:3.2,110.77828125);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOn/normOfferedTraffic_0.5_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=15.7339898049402,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,12.9808058136175);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,11.0727569744902);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,11.0348870603131);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,12.7420613773217);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,6.44358798127095);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,6.44356798865972);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,6.44381983776769);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,6.44366688521853);
\path [draw=black, thick]
(axis cs:-0.2,10.9768594320539)
--(axis cs:-0.2,14.9847521951811);

\path [draw=black, thick]
(axis cs:0.8,9.37322605767419)
--(axis cs:0.8,12.7722878913063);

\path [draw=black, thick]
(axis cs:1.8,9.42777964322607)
--(axis cs:1.8,12.6419944774001);

\path [draw=black, thick]
(axis cs:2.8,10.7014208815343)
--(axis cs:2.8,14.7827018731091);

\path [draw=black, thick]
(axis cs:0.2,6.44339285999363)
--(axis cs:0.2,6.44378310254827);

\path [draw=black, thick]
(axis cs:1.2,6.44342823099979)
--(axis cs:1.2,6.44370774631965);

\path [draw=black, thick]
(axis cs:2.2,6.4436448302762)
--(axis cs:2.2,6.44399484525919);

\path [draw=black, thick]
(axis cs:3.2,6.44345623999395)
--(axis cs:3.2,6.44387753044312);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOn/normOfferedTraffic_0.5_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=145.396687618447,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,138.472571600877);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,138.47261129386);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,138.47261129386);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,138.4728125);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,138.4728125);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,138.4728125);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,138.4728125);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,138.4728125);
\path [draw=black, thick]
(axis cs:-0.2,138.472107374662)
--(axis cs:-0.2,138.473035827092);

\path [draw=black, thick]
(axis cs:0.8,138.472223558264)
--(axis cs:0.8,138.472999029456);

\path [draw=black, thick]
(axis cs:1.8,138.472223558264)
--(axis cs:1.8,138.472999029456);

\path [draw=black, thick]
(axis cs:2.8,138.4728125)
--(axis cs:2.8,138.4728125);

\path [draw=black, thick]
(axis cs:0.2,138.4728125)
--(axis cs:0.2,138.4728125);

\path [draw=black, thick]
(axis cs:1.2,138.4728125)
--(axis cs:1.2,138.4728125);

\path [draw=black, thick]
(axis cs:2.2,138.4728125)
--(axis cs:2.2,138.4728125);

\path [draw=black, thick]
(axis cs:3.2,138.4728125)
--(axis cs:3.2,138.4728125);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOn/normOfferedTraffic_0.6_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=20.3745842032472,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,16.8725044790687);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,14.4188879819959);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,14.6945817792411);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,16.5528725310247);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,7.72285465606067);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,7.7228178299618);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,7.72300327234946);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,7.72288794580125);
\path [draw=black, thick]
(axis cs:-0.2,14.3406430502828)
--(axis cs:-0.2,19.4043659078545);

\path [draw=black, thick]
(axis cs:0.8,12.1007250322733)
--(axis cs:0.8,16.7370509317184);

\path [draw=black, thick]
(axis cs:1.8,12.6202875692265)
--(axis cs:1.8,16.7688759892557);

\path [draw=black, thick]
(axis cs:2.8,14.0075196267888)
--(axis cs:2.8,19.0982254352606);

\path [draw=black, thick]
(axis cs:0.2,7.72268497362875)
--(axis cs:0.2,7.72302433849259);

\path [draw=black, thick]
(axis cs:1.2,7.72269767276457)
--(axis cs:1.2,7.72293798715903);

\path [draw=black, thick]
(axis cs:2.2,7.72285465968948)
--(axis cs:2.2,7.72315188500944);

\path [draw=black, thick]
(axis cs:3.2,7.72271272072836)
--(axis cs:3.2,7.72306317087413);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOn/normOfferedTraffic_0.6_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=174.476053282807,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,166.166826480263);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,166.166826480263);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,166.167421875);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,166.167421875);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,166.167421875);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,166.167421875);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,166.167421875);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,166.167421875);
\path [draw=black, thick]
(axis cs:-0.2,166.165983167376)
--(axis cs:-0.2,166.16766979315);

\path [draw=black, thick]
(axis cs:0.8,166.165983167376)
--(axis cs:0.8,166.16766979315);

\path [draw=black, thick]
(axis cs:1.8,166.167421875)
--(axis cs:1.8,166.167421875);

\path [draw=black, thick]
(axis cs:2.8,166.167421875)
--(axis cs:2.8,166.167421875);

\path [draw=black, thick]
(axis cs:0.2,166.167421875)
--(axis cs:0.2,166.167421875);

\path [draw=black, thick]
(axis cs:1.2,166.167421875)
--(axis cs:1.2,166.167421875);

\path [draw=black, thick]
(axis cs:2.2,166.167421875)
--(axis cs:2.2,166.167421875);

\path [draw=black, thick]
(axis cs:3.2,166.167421875)
--(axis cs:3.2,166.167421875);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOn/normOfferedTraffic_0.7_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=25.7365255681673,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,21.5179666943838);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,18.6178970820806);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,18.9749435888885);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,20.8604382207211);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,9.00718019917084);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,9.00714706035128);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,9.00728692962033);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,9.00718990313625);
\path [draw=black, thick]
(axis cs:-0.2,18.5249566571797)
--(axis cs:-0.2,24.5109767315879);

\path [draw=black, thick]
(axis cs:0.8,15.6661047995992)
--(axis cs:0.8,21.5696893645621);

\path [draw=black, thick]
(axis cs:1.8,16.3549654707694)
--(axis cs:1.8,21.5949217070076);

\path [draw=black, thick]
(axis cs:2.8,17.922014132649)
--(axis cs:2.8,23.7988623087932);

\path [draw=black, thick]
(axis cs:0.2,9.0070352819876)
--(axis cs:0.2,9.00732511635407);

\path [draw=black, thick]
(axis cs:1.2,9.00704448777573)
--(axis cs:1.2,9.00724963292682);

\path [draw=black, thick]
(axis cs:2.2,9.00716101957801)
--(axis cs:2.2,9.00741283966264);

\path [draw=black, thick]
(axis cs:3.2,9.00703736519896)
--(axis cs:3.2,9.00734244107353);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOn/normOfferedTraffic_0.7_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=203.555243968841,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,193.861953125);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,193.861953125);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,193.861754660088);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,193.861953125);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,193.861953125);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,193.861953125);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,193.861953125);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,193.861953125);
\path [draw=black, thick]
(axis cs:-0.2,193.861953125)
--(axis cs:-0.2,193.861953125);

\path [draw=black, thick]
(axis cs:0.8,193.861953125)
--(axis cs:0.8,193.861953125);

\path [draw=black, thick]
(axis cs:1.8,193.861372206993)
--(axis cs:1.8,193.862137113182);

\path [draw=black, thick]
(axis cs:2.8,193.861953125)
--(axis cs:2.8,193.861953125);

\path [draw=black, thick]
(axis cs:0.2,193.861953125)
--(axis cs:0.2,193.861953125);

\path [draw=black, thick]
(axis cs:1.2,193.861953125)
--(axis cs:1.2,193.861953125);

\path [draw=black, thick]
(axis cs:2.2,193.861953125)
--(axis cs:2.2,193.861953125);

\path [draw=black, thick]
(axis cs:3.2,193.861953125)
--(axis cs:3.2,193.861953125);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOn/normOfferedTraffic_0.8_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=31.753256595881,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,26.707506722635);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,23.5269182922783);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,23.7140766643399);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,26.8203574579155);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,10.2915923226099);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,10.2915647044067);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,10.2917037792687);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,10.2916157123998);
\path [draw=black, thick]
(axis cs:-0.2,23.3207231437205)
--(axis cs:-0.2,30.0942903015495);

\path [draw=black, thick]
(axis cs:0.8,20.2056664272123)
--(axis cs:0.8,26.8481701573443);

\path [draw=black, thick]
(axis cs:1.8,20.5486489612017)
--(axis cs:1.8,26.8795043674782);

\path [draw=black, thick]
(axis cs:2.8,23.3995181578491)
--(axis cs:2.8,30.2411967579819);

\path [draw=black, thick]
(axis cs:0.2,10.2914648966036)
--(axis cs:0.2,10.2917197486161);

\path [draw=black, thick]
(axis cs:1.2,10.291474318366)
--(axis cs:1.2,10.2916550904473);

\path [draw=black, thick]
(axis cs:2.2,10.2915920141517)
--(axis cs:2.2,10.2918155443858);

\path [draw=black, thick]
(axis cs:3.2,10.2914835768582)
--(axis cs:3.2,10.2917478479415);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOn/normOfferedTraffic_0.8_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=232.634512043853,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,221.5565625);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,221.555768640351);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,221.5565625);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,221.5565625);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,221.5565625);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,221.5565625);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,221.5565625);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,221.5565625);
\path [draw=black, thick]
(axis cs:-0.2,221.5565625)
--(axis cs:-0.2,221.5565625);

\path [draw=black, thick]
(axis cs:0.8,221.554859143699)
--(axis cs:0.8,221.556678137003);

\path [draw=black, thick]
(axis cs:1.8,221.5565625)
--(axis cs:1.8,221.5565625);

\path [draw=black, thick]
(axis cs:2.8,221.5565625)
--(axis cs:2.8,221.5565625);

\path [draw=black, thick]
(axis cs:0.2,221.5565625)
--(axis cs:0.2,221.5565625);

\path [draw=black, thick]
(axis cs:1.2,221.5565625)
--(axis cs:1.2,221.5565625);

\path [draw=black, thick]
(axis cs:2.2,221.5565625)
--(axis cs:2.2,221.5565625);

\path [draw=black, thick]
(axis cs:3.2,221.5565625)
--(axis cs:3.2,221.5565625);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOn/normOfferedTraffic_0.9_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=272.335250159695,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,230.425238775339);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,194.879050977726);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,206.141767447393);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,227.007895489905);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,11.5760229976691);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,11.5759984485613);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,11.5761214333038);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,11.576033367766);
\path [draw=black, thick]
(axis cs:-0.2,201.483572636682)
--(axis cs:-0.2,259.366904913996);

\path [draw=black, thick]
(axis cs:0.8,168.375544225616)
--(axis cs:0.8,221.382557729836);

\path [draw=black, thick]
(axis cs:1.8,178.098709545473)
--(axis cs:1.8,234.184825349314);

\path [draw=black, thick]
(axis cs:2.8,203.134430924661)
--(axis cs:2.8,250.881360055149);

\path [draw=black, thick]
(axis cs:0.2,11.5759096544124)
--(axis cs:0.2,11.5761363409258);

\path [draw=black, thick]
(axis cs:1.2,11.5759179832253)
--(axis cs:1.2,11.5760789138973);

\path [draw=black, thick]
(axis cs:2.2,11.5760216659923)
--(axis cs:2.2,11.5762212006153);

\path [draw=black, thick]
(axis cs:3.2,11.5759139311609)
--(axis cs:3.2,11.5761528043711);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOn/normOfferedTraffic_0.9_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=261.7136484375,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,231.119546491228);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,233.985994462719);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,233.495803179825);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,229.611809594298);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,249.25109375);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,249.25109375);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,249.25109375);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,249.25109375);
\path [draw=black, thick]
(axis cs:-0.2,225.716147363026)
--(axis cs:-0.2,236.52294561943);

\path [draw=black, thick]
(axis cs:0.8,229.35514241387)
--(axis cs:0.8,238.616846511568);

\path [draw=black, thick]
(axis cs:1.8,228.629623108826)
--(axis cs:1.8,238.361983250823);

\path [draw=black, thick]
(axis cs:2.8,225.201983320085)
--(axis cs:2.8,234.021635868512);

\path [draw=black, thick]
(axis cs:0.2,249.25109375)
--(axis cs:0.2,249.25109375);

\path [draw=black, thick]
(axis cs:1.2,249.25109375)
--(axis cs:1.2,249.25109375);

\path [draw=black, thick]
(axis cs:2.2,249.25109375)
--(axis cs:2.2,249.25109375);

\path [draw=black, thick]
(axis cs:3.2,249.25109375)
--(axis cs:3.2,249.25109375);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOn/normOfferedTraffic_1_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.57, xmax=3.17,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=377.247362908746,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,341.55100341048);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,304.304962535876);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,327.917436313378);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,326.82615820918);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,nan);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,nan);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,nan);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,nan);
\path [draw=black, thick]
(axis cs:-0.2,323.818804050725)
--(axis cs:-0.2,359.283202770234);

\path [draw=black, thick]
(axis cs:0.8,285.911082184394)
--(axis cs:0.8,322.698842887358);

\path [draw=black, thick]
(axis cs:1.8,313.324972103013)
--(axis cs:1.8,342.509900523744);

\path [draw=black, thick]
(axis cs:2.8,305.618650177077)
--(axis cs:2.8,348.033666241284);

\end{axis}

\end{tikzpicture}


==> img/burst_smartOn/normOfferedTraffic_1_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=299.779039059142,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,230.754642927632);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,239.833700794956);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,223.1037578125);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,224.788255235746);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,267.7141796875);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,203.093515625);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,193.8619921875);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,166.167421875);
\path [draw=black, thick]
(axis cs:-0.2,222.691308829882)
--(axis cs:-0.2,238.817977025381);

\path [draw=black, thick]
(axis cs:0.8,234.453711286262)
--(axis cs:0.8,245.21369030365);

\path [draw=black, thick]
(axis cs:1.8,215.025005356039)
--(axis cs:1.8,231.182510268962);

\path [draw=black, thick]
(axis cs:2.8,216.29702363257)
--(axis cs:2.8,233.279486838921);

\path [draw=black, thick]
(axis cs:0.2,249.924512652008)
--(axis cs:0.2,285.503846722992);

\path [draw=black, thick]
(axis cs:1.2,159.268189704491)
--(axis cs:1.2,246.918841545509);

\path [draw=black, thick]
(axis cs:2.2,148.446949919788)
--(axis cs:2.2,239.277034455212);

\path [draw=black, thick]
(axis cs:3.2,117.616699483104)
--(axis cs:3.2,214.718144266896);

\end{axis}

\end{tikzpicture}


==> img/burst_stdev/avg_delay_variation.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
width=\fwidth,
height=\fheight,
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={$\rho$},
x label style={at={(axis description cs:0.5,-0.25)},anchor=north},
xmajorgrids,
minor x tick num=10,
xminorgrids,
extra x ticks={0.2}, % 0.2 not showing for some reason
extra x tick labels={}, % remove label
extra tick style={tickwidth=\pgfkeysvalueof{/pgfplots/minor tick length}}, % make it a minor tick
xmin=0.000767270499010925, xmax=0.260664264112613,
xmode=log,
% xtick style={color=black},
% xtick={1e-05,0.0001,0.001,0.01,0.1,1,10},
% xticklabels={\(\displaystyle {10^{-5}}\),\(\displaystyle {10^{-4}}\),\(\displaystyle {10^{-3}}\),\(\displaystyle {10^{-2}}\),\(\displaystyle {10^{-1}}\),\(\displaystyle {10^{0}}\),\(\displaystyle {10^{1}}\)},
y grid style={white!69.0196078431373!black},
ylabel={Jitter [$\mu$s]},
scaled y ticks={real:0.001}, % scale from ms to us
ytick scale label code/.code={}, % remove scale label
ymajorgrids,
ymin=0, ymax=0.1,
ytick style={color=black},
% ytick={0.01,0.02,0.03,0.04,0.05,0.06,0.07},
% yticklabels={0.01,0.02,0.03,0.04,0.05,0.06,0.07}
]
\path [draw=color0, thick]
(axis cs:0,0.0480938331496938)
--(axis cs:0,0.0608996200195079);

\path [draw=color0, thick]
(axis cs:0.001,0.0480938331496938)
--(axis cs:0.001,0.0608996200195079);

\path [draw=color0, thick]
(axis cs:0.002,0.0480938331496938)
--(axis cs:0.002,0.0608996200195079);

\path [draw=color0, thick]
(axis cs:0.005,0.047858593675683)
--(axis cs:0.005,0.0606239250600787);

\path [draw=color0, thick]
(axis cs:0.01,0.0460666069322293)
--(axis cs:0.01,0.056052837359408);

\path [draw=color0, thick]
(axis cs:0.02,0.047064721632887)
--(axis cs:0.02,0.0540727712794589);

\path [draw=color0, thick]
(axis cs:0.05,0.0518147377382793)
--(axis cs:0.05,0.0556381043002595);

\path [draw=color0, thick]
(axis cs:0.1,0.0543073596001402)
--(axis cs:0.1,0.0564906265783786);

\path [draw=color0, thick]
(axis cs:0.2,0.0615642668354013)
--(axis cs:0.2,0.0647003291118153);

\path [draw=color1, thick]
(axis cs:0,0.0208746968853917)
--(axis cs:0,0.0208760167016207);

\path [draw=color1, thick]
(axis cs:0.001,0.0208746981618041)
--(axis cs:0.001,0.0208760173828842);

\path [draw=color1, thick]
(axis cs:0.002,0.0208746968853917)
--(axis cs:0.002,0.0208760167016207);

\path [draw=color1, thick]
(axis cs:0.005,0.0208746968853917)
--(axis cs:0.005,0.0208760167016207);

\path [draw=color1, thick]
(axis cs:0.01,0.042905324613088)
--(axis cs:0.01,0.0581309319705074);

\path [draw=color1, thick]
(axis cs:0.02,0.0476753738887511)
--(axis cs:0.02,0.0628589334805186);

\path [draw=color1, thick]
(axis cs:0.05,0.0473488243613714)
--(axis cs:0.05,0.0526390536867597);

\path [draw=color1, thick]
(axis cs:0.1,0.0520585879418591)
--(axis cs:0.1,0.0557171562609355);

\path [draw=color1, thick]
(axis cs:0.2,0.0602964677686005)
--(axis cs:0.2,0.0631387995696304);

\path [draw=color1, thick]
(axis cs:0,0.0454937305113569)
--(axis cs:0,0.0568445867396051);

\path [draw=color1, thick]
(axis cs:0.001,0.0454937305113569)
--(axis cs:0.001,0.0568445867396051);

\path [draw=color1, thick]
(axis cs:0.002,0.0454937305113569)
--(axis cs:0.002,0.0568445867396051);

\path [draw=color1, thick]
(axis cs:0.005,0.0454937305113569)
--(axis cs:0.005,0.0568445867396051);

\path [draw=color1, thick]
(axis cs:0.01,0.0466929394806505)
--(axis cs:0.01,0.058873333276692);

\path [draw=color1, thick]
(axis cs:0.02,0.0483606652674733)
--(axis cs:0.02,0.0591622194821304);

\path [draw=color1, thick]
(axis cs:0.05,0.0483232764282395)
--(axis cs:0.05,0.0558814355780224);

\path [draw=color1, thick]
(axis cs:0.1,0.0533944915396663)
--(axis cs:0.1,0.0569706186340269);

\path [draw=color1, thick]
(axis cs:0.2,0.058725793876429)
--(axis cs:0.2,0.0613003546247875);

\path [draw=color1, thick]
(axis cs:0,0.0324397517227887)
--(axis cs:0,0.0403265278774272);

\path [draw=color1, thick]
(axis cs:0.001,0.0324397517227887)
--(axis cs:0.001,0.0403265278774272);

\path [draw=color1, thick]
(axis cs:0.002,0.0324397517227887)
--(axis cs:0.002,0.0403265278774272);

\path [draw=color1, thick]
(axis cs:0.005,0.0324397517227887)
--(axis cs:0.005,0.0403265278774272);

\path [draw=color1, thick]
(axis cs:0.01,0.03631986636456)
--(axis cs:0.01,0.0460803674035446);

\path [draw=color1, thick]
(axis cs:0.02,0.0393074319519112)
--(axis cs:0.02,0.0507262571162962);

\path [draw=color1, thick]
(axis cs:0.05,0.0511829972255439)
--(axis cs:0.05,0.062347785487211);

\path [draw=color1, thick]
(axis cs:0.1,0.0675475557007828)
--(axis cs:0.1,0.0769118451425987);

\path [draw=color1, thick]
(axis cs:0.2,0.0920368360026034)
--(axis cs:0.2,0.103671292462776);

\addplot [thick, color0]
table {%
0.0000001 0.0544967265846009
0.001 0.0544967265846009
0.002 0.0544967265846009
0.005 0.0542412593678809
0.01 0.0510597221458186
0.02 0.050568746456173
0.05 0.0537264210192694
0.1 0.0553989930892594
0.2 0.0631322979736083
};
% \addlegendentry{allocationPeriod=1}
\addplot [thick, color1]
table {%
0.0000001 0.0208753567935062
0.001 0.0208753577723441
0.002 0.0208753567935062
0.005 0.0208753567935062
0.01 0.0505181282917977
0.02 0.0552671536846349
0.05 0.0499939390240655
0.1 0.0538878721013973
0.2 0.0617176336691154
};
% \addlegendentry{allocationPeriod=1}
\addplot [thick, color1, dashed]
table {%
0.0000001 0.051169158625481
0.001 0.051169158625481
0.002 0.051169158625481
0.005 0.051169158625481
0.01 0.0527831363786713
0.02 0.0537614423748018
0.05 0.052102356003131
0.1 0.0551825550868466
0.2 0.0600130742506082
};
% \addlegendentry{allocationPeriod=1}
\addplot [thick, color1, densely dotted]
table {%
0.0000001 0.036383139800108
0.001 0.036383139800108
0.002 0.0363831398001079
0.005 0.0363831398001079
0.01 0.0412001168840523
0.02 0.0450168445341037
0.05 0.0567653913563774
0.1 0.0722297004216907
0.2 0.0978540642326897
};
% \addlegendentry{allocationPeriod=1}
\end{axis}

\end{tikzpicture}


==> img/burst_stdev/jain_fairness.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
width=\fwidth,
height=\fheight,
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.03)}, anchor=south west, draw=white!80!black},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Period Deviation Ratio},
xmajorgrids,
xmin=0.000767270499010925, xmax=0.260664264112613,
xmode=log,
xtick style={color=black},
xtick={1e-05,0.0001,0.001,0.01,0.1,1,10},
xticklabels={\(\displaystyle {10^{-5}}\),\(\displaystyle {10^{-4}}\),\(\displaystyle {10^{-3}}\),\(\displaystyle {10^{-2}}\),\(\displaystyle {10^{-1}}\),\(\displaystyle {10^{0}}\),\(\displaystyle {10^{1}}\)},
y grid style={white!69.0196078431373!black},
ylabel={Jain's Fairness Index},
ymajorgrids,
ymin=0, ymax=1.00002056899214,
ytick style={color=black},
% ytick={0.9995,0.9996,0.9997,0.9998,0.9999,1,1.0001},
% yticklabels={0.9995,0.9996,0.9997,0.9998,0.9999,1.0000,1.0001}
]
\path [draw=color0, thick]
(axis cs:0,0.999999999984968)
--(axis cs:0,1.00000000000476);

\path [draw=color0, thick]
(axis cs:0.001,0.999999999984968)
--(axis cs:0.001,1.00000000000476);

\path [draw=color0, thick]
(axis cs:0.002,0.999999999984968)
--(axis cs:0.002,1.00000000000476);

\path [draw=color0, thick]
(axis cs:0.005,0.999999999984968)
--(axis cs:0.005,1.00000000000476);

\path [draw=color0, thick]
(axis cs:0.01,0.999992448486675)
--(axis cs:0.01,0.999998777041637);

\path [draw=color0, thick]
(axis cs:0.02,0.999986961744015)
--(axis cs:0.02,0.99999456619864);

\path [draw=color0, thick]
(axis cs:0.05,0.999967550824848)
--(axis cs:0.05,0.99998158236222);

\path [draw=color0, thick]
(axis cs:0.1,0.999905153060082)
--(axis cs:0.1,0.999946215928686);

\path [draw=color0, thick]
(axis cs:0.2,0.999588620257085)
--(axis cs:0.2,0.999783894822035);

\path [draw=color1, thick]
(axis cs:0,1)
--(axis cs:0,1);

\path [draw=color1, thick]
(axis cs:0.001,1)
--(axis cs:0.001,1);

\path [draw=color1, thick]
(axis cs:0.002,1)
--(axis cs:0.002,1);

\path [draw=color1, thick]
(axis cs:0.005,1)
--(axis cs:0.005,1);

\path [draw=color1, thick]
(axis cs:0.01,0.999994730565844)
--(axis cs:0.01,0.999999758425917);

\path [draw=color1, thick]
(axis cs:0.02,0.999989238786654)
--(axis cs:0.02,0.999996502360262);

\path [draw=color1, thick]
(axis cs:0.05,0.999960122911879)
--(axis cs:0.05,0.999980281910482);

\path [draw=color1, thick]
(axis cs:0.1,0.99988080919698)
--(axis cs:0.1,0.999932627441667);

\path [draw=color1, thick]
(axis cs:0.2,0.999598939328295)
--(axis cs:0.2,0.999774668005986);

\path [draw=color1, thick]
(axis cs:0,0.999999999975977)
--(axis cs:0,1.00000000000348);

\path [draw=color1, thick]
(axis cs:0.001,0.999999999975977)
--(axis cs:0.001,1.00000000000348);

\path [draw=color1, thick]
(axis cs:0.002,0.999999999975977)
--(axis cs:0.002,1.00000000000348);

\path [draw=color1, thick]
(axis cs:0.005,0.999999999975977)
--(axis cs:0.005,1.00000000000348);

\path [draw=color1, thick]
(axis cs:0.01,0.999988803096994)
--(axis cs:0.01,0.999997805876177);

\path [draw=color1, thick]
(axis cs:0.02,0.999984244283786)
--(axis cs:0.02,0.999995395195181);

\path [draw=color1, thick]
(axis cs:0.05,0.999964042878346)
--(axis cs:0.05,0.999983251066703);

\path [draw=color1, thick]
(axis cs:0.1,0.999908676392983)
--(axis cs:0.1,0.999947765905284);

\path [draw=color1, thick]
(axis cs:0.2,0.999645103346205)
--(axis cs:0.2,0.999786305281619);

\path [draw=color1, thick]
(axis cs:0,1)
--(axis cs:0,1);

\path [draw=color1, thick]
(axis cs:0.001,1)
--(axis cs:0.001,1);

\path [draw=color1, thick]
(axis cs:0.002,1)
--(axis cs:0.002,1);

\path [draw=color1, thick]
(axis cs:0.005,1)
--(axis cs:0.005,1);

\path [draw=color1, thick]
(axis cs:0.01,0.999988799700474)
--(axis cs:0.01,0.999997804479659);

\path [draw=color1, thick]
(axis cs:0.02,0.999985173196923)
--(axis cs:0.02,0.999996083034849);

\path [draw=color1, thick]
(axis cs:0.05,0.999970982495211)
--(axis cs:0.05,0.999987567981949);

\path [draw=color1, thick]
(axis cs:0.1,0.999937543312412)
--(axis cs:0.1,0.999963598195592);

\path [draw=color1, thick]
(axis cs:0.2,0.999812843949966)
--(axis cs:0.2,0.999897545798736);

\addplot [thick, color0]
table {%
0 0.999999999994864
0.001 0.999999999994864
0.002 0.999999999994864
0.005 0.999999999994864
0.01 0.999995612764156
0.02 0.999990763971328
0.05 0.999974566593534
0.1 0.999925684494384
0.2 0.99968625753956
};
% \addlegendentry{allocationPeriod=1}
\addplot [thick, color1]
table {%
0 1
0.001 1
0.002 1
0.005 1
0.01 0.99999724449588
0.02 0.999992870573458
0.05 0.99997020241118
0.1 0.999906718319324
0.2 0.99968680366714
};
% \addlegendentry{allocationPeriod=1}
\addplot [thick, color1, dashed]
table {%
0 0.999999999989729
0.001 0.999999999989729
0.002 0.999999999989729
0.005 0.999999999989729
0.01 0.999993304486585
0.02 0.999989819739484
0.05 0.999973646972525
0.1 0.999928221149133
0.2 0.999715704313912
};
% \addlegendentry{allocationPeriod=1}
\addplot [thick, color1, densely dotted]
table {%
0 1
0.001 1
0.002 1
0.005 1
0.01 0.999993302090067
0.02 0.999990628115886
0.05 0.99997927523858
0.1 0.999950570754002
0.2 0.999855194874351
};
% \addlegendentry{allocationPeriod=1}
\end{axis}

\end{tikzpicture}


==> img/burst_stdev/norm_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
width=\fwidth,
height=\fheight,
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Period Deviation Ratio},
xmajorgrids,
xmin=0.000767270499010925, xmax=0.260664264112613,
xmode=log,
xtick style={color=black},
xtick={1e-05,0.0001,0.001,0.01,0.1,1,10},
xticklabels={\(\displaystyle {10^{-5}}\),\(\displaystyle {10^{-4}}\),\(\displaystyle {10^{-3}}\),\(\displaystyle {10^{-2}}\),\(\displaystyle {10^{-1}}\),\(\displaystyle {10^{0}}\),\(\displaystyle {10^{1}}\)},
y grid style={white!69.0196078431373!black},
ylabel={Aggr. Throughput / Aggr. Offered Rate},
ymajorgrids,
ymin=0, ymax=1.00331980369313,
ytick style={color=black}
]
\path [draw=color0, thick]
(axis cs:0,0.999998946041368)
--(axis cs:0,0.999999866686492);

\path [draw=color0, thick]
(axis cs:0.001,0.999998946041368)
--(axis cs:0.001,0.999999866686492);

\path [draw=color0, thick]
(axis cs:0.002,0.999998946041368)
--(axis cs:0.002,0.999999866686492);

\path [draw=color0, thick]
(axis cs:0.005,0.999998946041368)
--(axis cs:0.005,0.999999866686492);

\path [draw=color0, thick]
(axis cs:0.01,0.999396858863535)
--(axis cs:0.01,1.00042651533007);

\path [draw=color0, thick]
(axis cs:0.02,0.999138430550389)
--(axis cs:0.02,1.00050854961531);

\path [draw=color0, thick]
(axis cs:0.05,0.998340516347971)
--(axis cs:0.05,1.000946404112);

\path [draw=color0, thick]
(axis cs:0.1,0.997375103898071)
--(axis cs:0.1,1.00156916663695);

\path [draw=color0, thick]
(axis cs:0.2,0.993451519669674)
--(axis cs:0.2,1.00180854164606);

\path [draw=color1, thick]
(axis cs:0,0.999999645237345)
--(axis cs:0,0.999999645237345);

\path [draw=color1, thick]
(axis cs:0.001,0.999999645237345)
--(axis cs:0.001,0.999999645237345);

\path [draw=color1, thick]
(axis cs:0.002,0.999999645237345)
--(axis cs:0.002,0.999999645237345);

\path [draw=color1, thick]
(axis cs:0.005,0.999999645237345)
--(axis cs:0.005,0.999999645237345);

\path [draw=color1, thick]
(axis cs:0.01,1.0000304065073)
--(axis cs:0.01,1.0006706381044);

\path [draw=color1, thick]
(axis cs:0.02,1.00003362368966)
--(axis cs:0.02,1.00119278103113);

\path [draw=color1, thick]
(axis cs:0.05,0.999124172832092)
--(axis cs:0.05,1.00174609960506);

\path [draw=color1, thick]
(axis cs:0.1,0.99767244939967)
--(axis cs:0.1,1.00196402033575);

\path [draw=color1, thick]
(axis cs:0.2,0.995173994245915)
--(axis cs:0.2,1.0028498854063);

\path [draw=color1, thick]
(axis cs:0,0.99999852781861)
--(axis cs:0,0.99999980716242);

\path [draw=color1, thick]
(axis cs:0.001,0.99999852781861)
--(axis cs:0.001,0.99999980716242);

\path [draw=color1, thick]
(axis cs:0.002,0.99999852781861)
--(axis cs:0.002,0.99999980716242);

\path [draw=color1, thick]
(axis cs:0.005,0.99999852781861)
--(axis cs:0.005,0.99999980716242);

\path [draw=color1, thick]
(axis cs:0.01,0.999454739560171)
--(axis cs:0.01,1.00036290167147);

\path [draw=color1, thick]
(axis cs:0.02,0.999062073276144)
--(axis cs:0.02,1.0002254303781);

\path [draw=color1, thick]
(axis cs:0.05,0.998320065982255)
--(axis cs:0.05,1.00062086032496);

\path [draw=color1, thick]
(axis cs:0.1,0.996633931521091)
--(axis cs:0.1,1.00054592098797);

\path [draw=color1, thick]
(axis cs:0.2,0.995174570240211)
--(axis cs:0.2,1.00270082569706);

\path [draw=color1, thick]
(axis cs:0,0.999999645237345)
--(axis cs:0,0.999999645237345);

\path [draw=color1, thick]
(axis cs:0.001,0.999999645237345)
--(axis cs:0.001,0.999999645237345);

\path [draw=color1, thick]
(axis cs:0.002,0.999999645237345)
--(axis cs:0.002,0.999999645237345);

\path [draw=color1, thick]
(axis cs:0.005,0.999999645237345)
--(axis cs:0.005,0.999999645237345);

\path [draw=color1, thick]
(axis cs:0.01,0.999458126920989)
--(axis cs:0.01,1.00036572501945);

\path [draw=color1, thick]
(axis cs:0.02,0.999169147312914)
--(axis cs:0.02,1.00029349832941);

\path [draw=color1, thick]
(axis cs:0.05,0.997995396611765)
--(axis cs:0.05,1.00019728907616);

\path [draw=color1, thick]
(axis cs:0.1,0.994784724836955)
--(axis cs:0.1,0.99823703622458);

\path [draw=color1, thick]
(axis cs:0.2,0.98807346628061)
--(axis cs:0.2,0.993547613511908);

\addplot [thick, color0]
table {%
0 0.99999940636393
0.001 0.99999940636393
0.002 0.99999940636393
0.005 0.99999940636393
0.01 0.999911687096804
0.02 0.999823490082847
0.05 0.999643460229987
0.1 0.999472135267512
0.2 0.997630030657865
};
% \addlegendentry{allocationPeriod=1}
\addplot [thick, color1]
table {%
0 0.999999645237345
0.001 0.999999645237345
0.002 0.999999645237345
0.005 0.999999645237345
0.01 1.00035052230585
0.02 1.0006132023604
0.05 1.00043513621858
0.1 0.999818234867711
0.2 0.999011939826106
};
% \addlegendentry{allocationPeriod=1}
\addplot [thick, color1, dashed]
table {%
0 0.999999167490515
0.001 0.999999167490515
0.002 0.999999167490515
0.005 0.999999167490515
0.01 0.999908820615821
0.02 0.99964375182712
0.05 0.999470463153605
0.1 0.99858992625453
0.2 0.998937697968636
};
% \addlegendentry{allocationPeriod=1}
\addplot [thick, color1, densely dotted]
table {%
0 0.999999645237345
0.001 0.999999645237345
0.002 0.999999645237345
0.005 0.999999645237345
0.01 0.999911925970219
0.02 0.999731322821162
0.05 0.999096342843961
0.1 0.996510880530768
0.2 0.990810539896259
};
% \addlegendentry{allocationPeriod=1}
\end{axis}

\end{tikzpicture}


==> img/numStas/numStas_10_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.89, xmax=9.89,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9,STA 10},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=22.9790343911967,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,13.4542862893513);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,12.7113473135891);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,17.0912434300401);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,14.139233784555);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,13.5574561873567);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,13.4551304187765);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,16.5291773712155);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,19.2352324874943);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,14.2659944792679);
\draw[draw=none,fill=color0] (axis cs:8.6,0) rectangle (axis cs:9,15.9939976640255);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,3.87531488703518);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,3.87581665440138);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,3.87609924573255);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,3.87539744810156);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,3.87583874011225);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,3.87569991356822);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,3.8753143012702);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,3.87594347485677);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,3.87529461204866);
\draw[draw=none,fill=color1] (axis cs:9,0) rectangle (axis cs:9.4,3.87534779375696);
\path [draw=black, thick]
(axis cs:-0.2,10.8861209803823)
--(axis cs:-0.2,16.0224515983202);

\path [draw=black, thick]
(axis cs:0.8,9.91443535223782)
--(axis cs:0.8,15.5082592749403);

\path [draw=black, thick]
(axis cs:1.8,14.2664343536)
--(axis cs:1.8,19.9160525064803);

\path [draw=black, thick]
(axis cs:2.8,11.1627985484228)
--(axis cs:2.8,17.1156690206872);

\path [draw=black, thick]
(axis cs:3.8,10.9990656087078)
--(axis cs:3.8,16.1158467660056);

\path [draw=black, thick]
(axis cs:4.8,10.5398218441001)
--(axis cs:4.8,16.370438993453);

\path [draw=black, thick]
(axis cs:5.8,13.5889246283198)
--(axis cs:5.8,19.4694301141111);

\path [draw=black, thick]
(axis cs:6.8,16.5856703167059)
--(axis cs:6.8,21.8847946582826);

\path [draw=black, thick]
(axis cs:7.8,11.8796887776168)
--(axis cs:7.8,16.6523001809191);

\path [draw=black, thick]
(axis cs:8.8,13.381118118074)
--(axis cs:8.8,18.6068772099769);

\path [draw=black, thick]
(axis cs:0.2,3.8750170104838)
--(axis cs:0.2,3.87561276358657);

\path [draw=black, thick]
(axis cs:1.2,3.87539045049123)
--(axis cs:1.2,3.87624285831152);

\path [draw=black, thick]
(axis cs:2.2,3.87570165969552)
--(axis cs:2.2,3.87649683176957);

\path [draw=black, thick]
(axis cs:3.2,3.87506879400796)
--(axis cs:3.2,3.87572610219517);

\path [draw=black, thick]
(axis cs:4.2,3.8754452263195)
--(axis cs:4.2,3.87623225390499);

\path [draw=black, thick]
(axis cs:5.2,3.87528117694828)
--(axis cs:5.2,3.87611865018816);

\path [draw=black, thick]
(axis cs:6.2,3.87504070452436)
--(axis cs:6.2,3.87558789801603);

\path [draw=black, thick]
(axis cs:7.2,3.8755241116)
--(axis cs:7.2,3.87636283811354);

\path [draw=black, thick]
(axis cs:8.2,3.87503223898113)
--(axis cs:8.2,3.8755569851162);

\path [draw=black, thick]
(axis cs:9.2,3.87505563425553)
--(axis cs:9.2,3.87563995325838);

\end{axis}

\end{tikzpicture}


==> img/numStas/numStas_10_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.89, xmax=9.89,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8,STA 9,STA 10},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=87.2442186713408,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,83.0804217105263);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,83.0729594298246);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,83.0817490953948);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,83.0834734100877);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,83.0832749451754);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,83.0834734100877);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,83.0832749451754);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,83.0832749451754);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8,83.083671875);
\draw[draw=none,fill=color0] (axis cs:8.6,0) rectangle (axis cs:9,83.0834734100877);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,83.083671875);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,83.083671875);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,83.083671875);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,83.083671875);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,83.083671875);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,83.083671875);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,83.083671875);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,83.083671875);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.4,83.083671875);
\draw[draw=none,fill=color1] (axis cs:9,0) rectangle (axis cs:9.4,83.083671875);
\path [draw=black, thick]
(axis cs:-0.2,83.0763367656008)
--(axis cs:-0.2,83.0845066554519);

\path [draw=black, thick]
(axis cs:0.8,83.0561867917055)
--(axis cs:0.8,83.0897320679437);

\path [draw=black, thick]
(axis cs:1.8,83.0787871221833)
--(axis cs:1.8,83.0847110686062);

\path [draw=black, thick]
(axis cs:2.8,83.083090956993)
--(axis cs:2.8,83.0838558631825);

\path [draw=black, thick]
(axis cs:3.8,83.082510038986)
--(axis cs:3.8,83.0840398513649);

\path [draw=black, thick]
(axis cs:4.8,83.083090956993)
--(axis cs:4.8,83.0838558631825);

\path [draw=black, thick]
(axis cs:5.8,83.0827434819805)
--(axis cs:5.8,83.0838064083704);

\path [draw=black, thick]
(axis cs:6.8,83.0827434819805)
--(axis cs:6.8,83.0838064083704);

\path [draw=black, thick]
(axis cs:7.8,83.083671875)
--(axis cs:7.8,83.083671875);

\path [draw=black, thick]
(axis cs:8.8,83.083090956993)
--(axis cs:8.8,83.0838558631825);

\path [draw=black, thick]
(axis cs:0.2,83.083671875)
--(axis cs:0.2,83.083671875);

\path [draw=black, thick]
(axis cs:1.2,83.083671875)
--(axis cs:1.2,83.083671875);

\path [draw=black, thick]
(axis cs:2.2,83.083671875)
--(axis cs:2.2,83.083671875);

\path [draw=black, thick]
(axis cs:3.2,83.083671875)
--(axis cs:3.2,83.083671875);

\path [draw=black, thick]
(axis cs:4.2,83.083671875)
--(axis cs:4.2,83.083671875);

\path [draw=black, thick]
(axis cs:5.2,83.083671875)
--(axis cs:5.2,83.083671875);

\path [draw=black, thick]
(axis cs:6.2,83.083671875)
--(axis cs:6.2,83.083671875);

\path [draw=black, thick]
(axis cs:7.2,83.083671875)
--(axis cs:7.2,83.083671875);

\path [draw=black, thick]
(axis cs:8.2,83.083671875)
--(axis cs:8.2,83.083671875);

\path [draw=black, thick]
(axis cs:9.2,83.083671875)
--(axis cs:9.2,83.083671875);

\end{axis}

\end{tikzpicture}


==> img/numStas/numStas_2_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.49, xmax=1.49,
xtick style={color=black},
xtick={0,1},
xticklabels={STA 1,STA 2},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=41.7736306269767,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,36.0665385499118);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,35.2622687342842);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,21.215361827387);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,20.573133555923);
\path [draw=black, thick]
(axis cs:-0.2,32.3486669788934)
--(axis cs:-0.2,39.7844101209302);

\path [draw=black, thick]
(axis cs:0.8,31.8926866462131)
--(axis cs:0.8,38.6318508223552);

\path [draw=black, thick]
(axis cs:0.2,19.5741791857631)
--(axis cs:0.2,22.856544469011);

\path [draw=black, thick]
(axis cs:1.2,19.4013119551047)
--(axis cs:1.2,21.7449551567413);

\end{axis}

\end{tikzpicture}


==> img/numStas/numStas_2_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.49, xmax=1.49,
xtick style={color=black},
xtick={0,1},
xticklabels={STA 1,STA 2},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=436.18944140625,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,415.418515625);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,415.418515625);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,415.418515625);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,415.418515625);
\path [draw=black, thick]
(axis cs:-0.2,415.418515625)
--(axis cs:-0.2,415.418515625);

\path [draw=black, thick]
(axis cs:0.8,415.418515625)
--(axis cs:0.8,415.418515625);

\path [draw=black, thick]
(axis cs:0.2,415.418515625)
--(axis cs:0.2,415.418515625);

\path [draw=black, thick]
(axis cs:1.2,415.418515625)
--(axis cs:1.2,415.418515625);

\end{axis}

\end{tikzpicture}


==> img/numStas/numStas_4_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=28.4689353037846,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,23.8913401896154);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,21.1396490213861);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,21.2846592290431);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,23.7976083273969);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,9.65203001437322);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,9.65200056267937);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,9.6521488703147);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,9.65205537545273);
\path [draw=black, thick]
(axis cs:-0.2,20.6694086613407)
--(axis cs:-0.2,27.1132717178901);

\path [draw=black, thick]
(axis cs:0.8,17.9735220899474)
--(axis cs:0.8,24.3057759528249);

\path [draw=black, thick]
(axis cs:1.8,18.3784425384837)
--(axis cs:1.8,24.1908759196024);

\path [draw=black, thick]
(axis cs:2.8,20.6736352465532)
--(axis cs:2.8,26.9215814082406);

\path [draw=black, thick]
(axis cs:0.2,9.65189417473701)
--(axis cs:0.2,9.65216585400943);

\path [draw=black, thick]
(axis cs:1.2,9.65190424926408)
--(axis cs:1.2,9.65209687609465);

\path [draw=black, thick]
(axis cs:2.2,9.65202976860706)
--(axis cs:2.2,9.65226797202235);

\path [draw=black, thick]
(axis cs:3.2,9.65191466100834)
--(axis cs:3.2,9.65219608989712);

\end{axis}

\end{tikzpicture}


==> img/numStas/numStas_4_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.59, xmax=3.59,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={STA 1,STA 2,STA 3,STA 4},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=218.094872875092,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,207.70921875);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,207.709020285088);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,207.70921875);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,207.70921875);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,207.70921875);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,207.70921875);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,207.70921875);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,207.70921875);
\path [draw=black, thick]
(axis cs:-0.2,207.70921875)
--(axis cs:-0.2,207.70921875);

\path [draw=black, thick]
(axis cs:0.8,207.708637831993)
--(axis cs:0.8,207.709402738183);

\path [draw=black, thick]
(axis cs:1.8,207.70921875)
--(axis cs:1.8,207.70921875);

\path [draw=black, thick]
(axis cs:2.8,207.70921875)
--(axis cs:2.8,207.70921875);

\path [draw=black, thick]
(axis cs:0.2,207.70921875)
--(axis cs:0.2,207.70921875);

\path [draw=black, thick]
(axis cs:1.2,207.70921875)
--(axis cs:1.2,207.70921875);

\path [draw=black, thick]
(axis cs:2.2,207.70921875)
--(axis cs:2.2,207.70921875);

\path [draw=black, thick]
(axis cs:3.2,207.70921875)
--(axis cs:3.2,207.70921875);

\end{axis}

\end{tikzpicture}


==> img/numStas/numStas_6_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.69, xmax=5.69,
xtick style={color=black},
xtick={0,1,2,3,4,5},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=22.4579575716219,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,18.4659431599722);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,18.073409476012);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,18.6561850518291);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,17.372427888493);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,17.519592924389);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,16.1068996745568);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,6.4438440549825);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,6.44370216092175);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,6.44370220655683);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,6.44391749535109);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,6.4435947055908);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,6.44372961018584);
\path [draw=black, thick]
(axis cs:-0.2,15.6082613555023)
--(axis cs:-0.2,21.3236249644421);

\path [draw=black, thick]
(axis cs:0.8,15.1221107865462)
--(axis cs:0.8,21.0247081654778);

\path [draw=black, thick]
(axis cs:1.8,15.923839083066)
--(axis cs:1.8,21.3885310205923);

\path [draw=black, thick]
(axis cs:2.8,14.0328102692187)
--(axis cs:2.8,20.7120455077673);

\path [draw=black, thick]
(axis cs:3.8,14.8061048144495)
--(axis cs:3.8,20.2330810343284);

\path [draw=black, thick]
(axis cs:4.8,13.0138415155787)
--(axis cs:4.8,19.1999578335348);

\path [draw=black, thick]
(axis cs:0.2,6.44354082240857)
--(axis cs:0.2,6.44414728755643);

\path [draw=black, thick]
(axis cs:1.2,6.44349176894519)
--(axis cs:1.2,6.44391255289832);

\path [draw=black, thick]
(axis cs:2.2,6.4435507265639)
--(axis cs:2.2,6.44385368654977);

\path [draw=black, thick]
(axis cs:3.2,6.44372321616007)
--(axis cs:3.2,6.44411177454212);

\path [draw=black, thick]
(axis cs:4.2,6.44341335520847)
--(axis cs:4.2,6.44377605597312);

\path [draw=black, thick]
(axis cs:5.2,6.4434344504153)
--(axis cs:5.2,6.44402476995639);

\end{axis}

\end{tikzpicture}


==> img/numStas/numStas_6_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.69, xmax=5.69,
xtick style={color=black},
xtick={0,1,2,3,4,5},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=145.396735645078,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,138.472415570175);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,138.472614035088);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,138.472415570175);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,138.472018640351);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,138.472415570175);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,138.47261129386);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,138.4728125);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,138.4728125);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,138.4728125);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,138.4728125);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,138.4728125);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,138.4728125);
\path [draw=black, thick]
(axis cs:-0.2,138.47188410698)
--(axis cs:-0.2,138.47294703337);

\path [draw=black, thick]
(axis cs:0.8,138.472231581993)
--(axis cs:0.8,138.472996488182);

\path [draw=black, thick]
(axis cs:1.8,138.47188410698)
--(axis cs:1.8,138.47294703337);

\path [draw=black, thick]
(axis cs:2.8,138.470955713961)
--(axis cs:2.8,138.473081566741);

\path [draw=black, thick]
(axis cs:3.8,138.47188410698)
--(axis cs:3.8,138.47294703337);

\path [draw=black, thick]
(axis cs:4.8,138.472228986467)
--(axis cs:4.8,138.472993601253);

\path [draw=black, thick]
(axis cs:0.2,138.4728125)
--(axis cs:0.2,138.4728125);

\path [draw=black, thick]
(axis cs:1.2,138.4728125)
--(axis cs:1.2,138.4728125);

\path [draw=black, thick]
(axis cs:2.2,138.4728125)
--(axis cs:2.2,138.4728125);

\path [draw=black, thick]
(axis cs:3.2,138.4728125)
--(axis cs:3.2,138.4728125);

\path [draw=black, thick]
(axis cs:4.2,138.4728125)
--(axis cs:4.2,138.4728125);

\path [draw=black, thick]
(axis cs:5.2,138.4728125)
--(axis cs:5.2,138.4728125);

\end{axis}

\end{tikzpicture}


==> img/numStas/numStas_8_bars/user_delay.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.79, xmax=7.79,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8},
y grid style={white!69.0196078431373!black},
ylabel={Avg delay [ms]},
ymajorgrids,
ymin=0, ymax=21.5142476740206,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,13.5426693181028);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,16.7907754597271);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,16.5970667939873);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,13.7013158506802);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,17.2238631960489);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,16.1841668689186);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,14.5885169159377);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,16.06681989342);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,4.84000259958798);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,4.83994594387132);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,4.84007173626596);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,4.83980628339931);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,4.84018540228928);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,4.83981454222602);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,4.84017489098725);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,4.83978575293964);
\path [draw=black, thick]
(axis cs:-0.2,10.6723751353477)
--(axis cs:-0.2,16.4129635008579);

\path [draw=black, thick]
(axis cs:0.8,13.7673660708638)
--(axis cs:0.8,19.8141848485903);

\path [draw=black, thick]
(axis cs:1.8,13.8265848845185)
--(axis cs:1.8,19.367548703456);

\path [draw=black, thick]
(axis cs:2.8,10.6327668189454)
--(axis cs:2.8,16.769864882415);

\path [draw=black, thick]
(axis cs:3.8,13.9579667025543)
--(axis cs:3.8,20.4897596895435);

\path [draw=black, thick]
(axis cs:4.8,13.3296166543158)
--(axis cs:4.8,19.0387170835214);

\path [draw=black, thick]
(axis cs:5.8,11.9314117260566)
--(axis cs:5.8,17.2456221058187);

\path [draw=black, thick]
(axis cs:6.8,13.12293747539)
--(axis cs:6.8,19.01070231145);

\path [draw=black, thick]
(axis cs:0.2,4.83962743076079)
--(axis cs:0.2,4.84037776841517);

\path [draw=black, thick]
(axis cs:1.2,4.83960817363789)
--(axis cs:1.2,4.84028371410475);

\path [draw=black, thick]
(axis cs:2.2,4.83973941785247)
--(axis cs:2.2,4.84040405467945);

\path [draw=black, thick]
(axis cs:3.2,4.83952273191796)
--(axis cs:3.2,4.84008983488066);

\path [draw=black, thick]
(axis cs:4.2,4.83972940095755)
--(axis cs:4.2,4.84064140362102);

\path [draw=black, thick]
(axis cs:5.2,4.83957952968978)
--(axis cs:5.2,4.84004955476227);

\path [draw=black, thick]
(axis cs:6.2,4.83988301019979)
--(axis cs:6.2,4.84046677177471);

\path [draw=black, thick]
(axis cs:7.2,4.83949411040923)
--(axis cs:7.2,4.84007739547006);

\end{axis}

\end{tikzpicture}


==> img/numStas/numStas_8_bars/user_thr.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Node ID},
xmajorgrids,
xmin=-0.79, xmax=7.79,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7},
xticklabels={STA 1,STA 2,STA 3,STA 4,STA 5,STA 6,STA 7,STA 8},
y grid style={white!69.0196078431373!black},
ylabel={Throughput [Mbps]},
ymajorgrids,
ymin=0, ymax=109.047919406525,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,103.854609375);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{allocationPeriod=0}

\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,103.854013980263);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,103.854013980263);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3,103.854013980263);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4,103.853815515351);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5,103.854609375);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6,103.854609375);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7,103.854212445176);
\draw[draw=none,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,103.854609375);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
% \addlegendentry{allocationPeriod=1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,103.854609375);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,103.854609375);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.4,103.854609375);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.4,103.854609375);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.4,103.854609375);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.4,103.854609375);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.4,103.854609375);
\path [draw=black, thick]
(axis cs:-0.2,103.854609375)
--(axis cs:-0.2,103.854609375);

\path [draw=black, thick]
(axis cs:0.8,103.852866620979)
--(axis cs:0.8,103.855161339547);

\path [draw=black, thick]
(axis cs:1.8,103.853374802452)
--(axis cs:1.8,103.854653158074);

\path [draw=black, thick]
(axis cs:2.8,103.853170667377)
--(axis cs:2.8,103.85485729315);

\path [draw=black, thick]
(axis cs:3.8,103.8530912531)
--(axis cs:3.8,103.854539777602);

\path [draw=black, thick]
(axis cs:4.8,103.854609375)
--(axis cs:4.8,103.854609375);

\path [draw=black, thick]
(axis cs:5.8,103.854609375)
--(axis cs:5.8,103.854609375);

\path [draw=black, thick]
(axis cs:6.8,103.853680981981)
--(axis cs:6.8,103.85474390837);

\path [draw=black, thick]
(axis cs:0.2,103.854609375)
--(axis cs:0.2,103.854609375);

\path [draw=black, thick]
(axis cs:1.2,103.854609375)
--(axis cs:1.2,103.854609375);

\path [draw=black, thick]
(axis cs:2.2,103.854609375)
--(axis cs:2.2,103.854609375);

\path [draw=black, thick]
(axis cs:3.2,103.854609375)
--(axis cs:3.2,103.854609375);

\path [draw=black, thick]
(axis cs:4.2,103.854609375)
--(axis cs:4.2,103.854609375);

\path [draw=black, thick]
(axis cs:5.2,103.854609375)
--(axis cs:5.2,103.854609375);

\path [draw=black, thick]
(axis cs:6.2,103.854609375)
--(axis cs:6.2,103.854609375);

\path [draw=black, thick]
(axis cs:7.2,103.854609375)
--(axis cs:7.2,103.854609375);

\end{axis}

\end{tikzpicture}


==> img/scenario.tex <==
\begin{tikzpicture}[scale=1, every node/.style={transform shape, font=\scriptsize}]
  \def\radius{2.5}
  \def\nodeRadius{0.5}

  \draw (0, 0) circle [radius=0.5] node (P0) {PCP/AP};

  \foreach \x in {1,...,10}
  {
    \draw (\x*360/10:\radius) circle [radius=\nodeRadius] node {STA \x};
    \draw[->, dashed] (\x*360/10:\radius-\nodeRadius*1.1) -- (\x*360/10:\nodeRadius*1.1);
  }

  % \foreach \x in {5,...,10}
  % {
  %   \draw[gray] (\x*360/10:\radius) circle [radius=\nodeRadius] node {STA \x};
  %   \draw[->, dashed, gray] (\x*360/10:\radius-\nodeRadius*1.1) -- (\x*360/10:\nodeRadius*1.1);
  % }
  
\end{tikzpicture}
